Ember: No-Code Context Enrichment via Similarity-Based Keyless Joins

Structured data, or data that adheres to a pre-defined schema, can suffer from fragmented context: information describing a single entity can be scattered across multiple datasets or tables tailored for specific business needs, with no explicit linking keys (e.g., primary key-foreign key relationships or heuristic functions). Context enrichment, or rebuilding fragmented context, using keyless joins is an implicit or explicit step in machine learning (ML) pipelines over structured data sources. This process is tedious, domain-specific, and lacks support in now-prevalent no-code ML systems that let users create ML pipelines using just input data and high-level configuration files. In response, we propose Ember, a system that abstracts and automates keyless joins to generalize context enrichment. Our key insight is that Ember can enable a general keyless join operator by constructing an index populated with task-specific embeddings. Ember learns these embeddings by leveraging Transformer-based representation learning techniques. We describe our core architectural principles and operators when developing Ember, and empirically demonstrate that Ember allows users to develop no-code pipelines for five domains, including search, recommendation and question answering, and can exceed alternatives by up to 39% recall, with as little as a single line configuration change.

==> context enrichment 8/abstract.tex <==
\begin{abstract}
Structured data, or data that adheres to a pre-defined schema, can suffer from fragmented context: information describing a single entity can be scattered across multiple datasets or tables tailored for specific business needs, with no explicit linking keys (e.g., primary key-foreign key relationships or heuristic functions).
Context enrichment, or rebuilding fragmented context, using \emph{keyless joins} is an implicit or explicit step in machine learning (ML) pipelines over structured data sources.
This process is tedious, domain-specific, and lacks support in now-prevalent no-code ML systems that let users create ML pipelines using just input data and high-level configuration files.
In response, we propose \sys, a system that abstracts and automates keyless joins to generalize context enrichment.
Our key insight is that \sys can enable a general keyless join operator by constructing an index populated with task-specific embeddings. 
\sys learns these embeddings by leveraging Transformer-based representation learning techniques.
We describe our core architectural principles and operators when developing \sys, and empirically demonstrate that \sys allows users to develop no-code pipelines for five domains, including search, recommendation and question answering, and can exceed alternatives by up to 39\% recall, with as little as a single line configuration change.

\end{abstract}




==> context enrichment 8/application.tex <==

\section{Context Enrichment}
\label{sec:applications}

In this section, we define context enrichment, and provide example workloads that can be framed as a form of context enrichment.

\subsection{Problem Statement}
\label{subsec:problem}

Structured data, or data that adheres to a fixed schema formatted in rows and columns, suffers from context fragmentation.
We broadly define structured data to include semi-structured and textual data sources that may be stored and keyed in data management systems, such as content from Wikipedia articles or web search results. 
Unlike unstructured data, structured data follows a scattered format that is efficient to store, query, and manipulate for specific business needs.
This may be in the form of an e-commerce company storing datasets cataloging products and user reviews as in Figure~\ref{fig:example}.
To use this fragmented data for ML tasks, practitioners implicitly or explicitly join these dataset to construct discriminative features. 

We refer to this joining process as \emph{context enrichment}, which we define as follows:
Given a base dataset in tabular form, $D_0$, context enrichment aligns $D_0$ with context derived from auxiliary data sources, $D = \{D_1, ... , D_M\}$, to solve a task $T$. 
We focus on a text-based, two-dataset case ($|D| = 1$), but propose means for multi-dataset extension Sections~\ref{sec:preprocessing}-\ref{sec:joining}, and defer their evaluation to future work.
We explore context enrichment in regimes with abundant and limited labeled relevant pairs $Y$ to learn source alignment.

%Each dataset $D_i$ consists of $\mathbf{d_i}$ columns, each of which we denote as $C_{ir}, r \in \{1, ...,\mathbf{d_i}\}$. 
%Data points in each dataset are represented as $d_{ij}$ for the $j^{th}$ row in dataset $i$, and $d_{ij} \in \mathbf{D_i}$, where each domain $\mathbf{D_i} \in  \{\mathbb{R} \cup \mathbb{N}\}^{\mathbf{d_i}}$ (each column is either numeric or textual, e.g., categorical or free form text). We briefly describe how to extend our methods beyond these formats in Section~\ref{sec:representation}. 

We represent each dataset $D_i$ as an $\mathbf{n_i}\times\mathbf{d_i}$ matrix of $\mathbf{n_i}$ data points (or records) and  $\mathbf{d_i}$ columns. 
%, where $j \in \{1, ...,\mathbf{n_i}\}$, .
We denote $C_{ir}$ as the $r^{th}$ column in dataset $i$.
We denote $d_{ij}$ as the $j^{th}$ row in dataset $i$.
%, where $r \in \{1, ...,\mathbf{d_i}\}$. 
Columns are numeric or textual, and we refer to the domain of $d_{ij}$ as $\mathbf{D_i}$.


\eat{Each dataset $D_i$ consists of $\mathbf{d_i}$ columns, each of which we denote as $C_{ir}$, where $r \in \{1, ...,\mathbf{d_i}\}$. 
Columns are either numeric or textual, meaning $C_{ir} \in X^{{n_i}}$, where $X \in \{\mathbb{R} \cup \mathbb{N}\}$ and $n_i$ is the number of records in dataset $D_i$.
Data points in each dataset are represented as $d_{ij}$ for the $j^{th}$ row in dataset $i$, where $j \in \{1, ...,n_i\}$ and $d_{ij} \in X^{\mathbf{d_i}}$. We describe how to extend beyond these formats in Section~\ref{sec:representation}. }

%Each dataset $D_i$ consists of $\mathbf{d_i}$ columns, each of which we denote as $C_{ir} \in \{\mathbb{R} \cup \mathbb{N}\}$, where $r \in \{1, ...,\mathbf{d_i}\}$; each column is either numeric or textual (e.g., categorical or free form text).
%Data points in each dataset are represented as $d_{ij}$ for the $j^{th}$ row in dataset $i$, and $d_{ij} \in \mathbf{D_i}$, where each domain $\mathbf{D_i} = \{C_{ir}\}_{r=0}^{\mathbf{d_i}}$. We briefly describe how to extend our methods beyond these formats in Section~\ref{sec:representation}. 

Our goal is to \emph{enrich}, or identify all context for, each $d_{0j}$ in $D_0$: auxiliary records $d_{lm}$ ($l \neq 0$) that are related to $d_{0j}$, as per task $T$.

\subsection{Motivating Applications}
\label{subsec:target}

Context enrichment is a key component for applications across a broad array of domains. 
Thus, a context enrichment system would reduce the developer time and effort needed to construct domain-specific pipelines.
We now describe a subset of these domains, which we evaluate in Section~\ref{sec:eval}. 
Additional applicable domains include entity linkage or disambiguation~\citep{link2,link1}, nearest neighbor machine translation~\citep{knnmt}, and nearest neighbor language modeling~\citep{knnlm}.

\minihead{Entity Matching and Deduplication}
Entity matching identifies data points that refer to the same real-world entity across two different collections of entity mentions~\citep{matchsurvey}. 
An entity denotes any distinct real-world object such as a person or organization, while its entity mention is a reference to this entity in a structured dataset or a text span.   
Entity deduplication identifies entities that are found multiple times in a single data source, thus is a special case of entity matching where both collections of entity mentions are the same.

\vspace{4pt}
\noindent
We frame entity matching as a context enrichment problem where $D_0$ and $D_1$ represent the two collections of entity mentions. 
Context enrichment aligns entities $d_{1m}$ in the auxiliary dataset $D_1$ with each entity $d_{0j}$ in the base dataset $D_0$. In entity deduplication, $D_0 = D_1$. 
The downstream task $T$ is a binary classifier over the retrieved relevant records, as the aim is to identify matching entities. 

\eat{
\minihead{Entity Linking or Disambiguation}
Entity linking, or named entity disambiguation, joins entity mentions (as defined above) in the form of a text span to a canonical entity in a database or knowledge graph~\citep{link1,link2}. Entity linkage differs from entity matching in that it has access to relationship information across entities.

\vspace{3pt}
\noindent
We frame entity linkage as a context enrichment problem where $D_0$ and $D_1$ represent the collection of entity mentions and a database or linearized representation of the knowledge graph, respectively. 
Context enrichment aligns entities $d_{1m}$ in the auxiliary dataset $D_1$ that map to each entity $d_{0j}$ in the base dataset $D_0$.
The downstream task $T$ is a binary classifier over the retrieved relevant records, as the aim is to identify matching entities. \\
}

\minihead{Fuzzy Joining}
A fuzzy join identifies data point pairs that are similar to one another across two database tables, where similar records may be identified with respect to a similarity function (e.g., cosine similarity, Jaccard similarity, edit distance) and threshold~\citep{fj1,surajit} defined over a subset of key columns. 
Though related to entity matching, fuzzy joins can be viewed as a primitive used to efficiently mine and block pairs that are similar across the two data sources. 

\vspace{4pt}
\noindent
We frame fuzzy joining as a context enrichment problem where $D_0$ and $D_1$ represent the two database tables.
We let $C_0$ and $C_1$ denote the set of key columns used for joining.
Records $d_{0j}$ and $d_{1m}$ are joined if their values in columns $C_0$ and $C_1$ are similar, to some threshold quantity. 
This is equivalent to a generic context enrichment task with a limited number of features used. 
The downstream task $T$ is a top-k query, as the aim is to identify similar entities. 

\minihead{Recommendation}
A recommender system predicts the rating that a user would give an item, typically for use in content recommendation or filtering~\citep{recsys}. 
We also consider the broader problem of uncovering the global rating for an item, as in the e-commerce example in Figure~\ref{fig:example}, as being a form of recommendation problem---namely, the global score may be predicted by aggregating the predicted per-user results obtained via classic recommender systems.  

\vspace{4pt}
\noindent
We frame such recommendation workloads as a context enrichment problem where $D_0$ represents all information regarding the entity to be ranked (e.g., a base product table, or new candidate products), and $D_1$ represents the information of the rankers, or other auxiliary data (e.g., catalogs of previously ranked products).
Context enrichment aligns rankers $d_{1m}$ in the auxiliary dataset $D_1$ with those that are related to each entity to be ranked $d_{0j}$ in the base dataset $D_0$. 
The downstream task $T$ is to return the top-1 query, or to perform aggregation or train an ML model over the returned top-k entries.

\minihead{Search}
An enterprise search engine returns information relevant to a user query issued over internal databases, documentation, files, or web pages~\citep{enterprise1, enterprise2}. 
A general web retrieval system displays information relevant to a given search query~\citep{search1,search2}. 
Both rely on information retrieval techniques and relevance-based ranking over an underlying document corpus as building blocks to develop complex, personalized pipelines, or for retrospective analyses~\citep{marco}.

\vspace{4pt}
\noindent
We frame retrieval and ranking in search as a context enrichment problem where $D_0$ represents the set of user queries, and $D_1$ represents the underlying document corpus.
Context enrichment aligns documents $d_{1m}$ in the auxiliary dataset $D_1$ that map to each query $d_{0j}$ in the base dataset $D_0$.
The downstream task $T$ is to return the top-k documents for each query, sorted by their query relatedness.


\minihead{Question Answering}
Question answering systems answer natural language questions given a corresponding passage (e.g., in reading comprehension tasks) or existing knowledge source (e.g., in open domain question answering)~\citep{squad,qa}.
Multi-hop question answering generalizes this setting, where the system must traverse a series of passages to uncover the answer~\citep{multihop}. 
For instance, the question "what color is the ocean?" may be provided the statements "the sky is blue" and "the ocean is the same color as the sky." 

\vspace{4pt}
\noindent
We frame the retriever component~\citep{retriever} of a classic retriever-reader model in open domain question answering as a context enrichment problem. 
Our task is to identify the candidate text spans in the provided passages that contain the question's answer (the retriever component), and a downstream reader task can formulate the answer to the question.
We let dataset $D_0$ represent the set of questions, and $D_1$ represent the provided passages or knowledge source, split into spans (e.g., based on sentences, or fixed word windows).
Context enrichment aligns spans $d_{1m}$ in the auxiliary dataset $D_1$ that contain the answer to each question $d_{0j}$ in the base dataset $D_0$. 
Multi-hop question answering requires an extra round of context enrichment for each hop required.
Each round selects a different passage's spans as the base table $D_0$; to identify context relevant to the question, the user can traverse the related spans extracted from each passage.
The downstream task $T$ is to learn a reader model to answer questions using the enriched data sources.

\eat{
\minihead{Machine Translation}


\red{Do the nearest neighbor MT or LM warrant adding?} 
}



==> context enrichment 8/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We demonstrate how seemingly unrelated tasks spanning data integration, search, and recommendation can all be viewed as instantiations of context enrichment.
We propose keyless joins as a unifying abstraction that can power a system for general context enrichment, which allows us to view context enrichment as a data management problem. 
Consequently, we developed and applied \sys, a first-of-its kind system that performs no-code context enrichment via keyless joins. 
We evaluate how developing a keyless join enrichment layer empowers a single system to generalize to five downstream applications, with no ML code written by the user.
%By proposing a unifying framework for context enrichment, decrease 

%data management problem requiring a new class of join: a keyless join.
%We evaluate how 

%%We call for the development of a system optimized for a new class of join: a keyless join.

==> context enrichment 8/ember.tex <==
\input{tables/types}

\section{\sys}
\label{sec:ember}

We develop \sys,\footnote{https://github.com/sahaana/ember} an open-source system for no-code context enrichment.
\sys implements a keyless join abstraction layer that meets the specification in Section~\ref{subsec:keyless_spec}.
\sys first represents input records using transformer-based embeddings directly optimized for the condition in Section~\ref{subsec:keyless}.
\sys then populates a reusable index with these embeddings based on the \texttt{join type}, and configures index retrieval based on the \texttt{join sizes}. 
We now provide an overview of \sys's usage, API and architecture; data types and operators are in Table~\ref{table:types}, with an architecture overview in Figure~\ref{fig:pipeline}.

\subsection{Usage}
\label{subsec:api}

As input, \sys requires the join specification parameters: a base data source $D_0$ ("left"), auxiliary data sources $D=\{D_1,...,D_M\}$ ("right"), labeled examples of related data points that represent similar entities, \texttt{join type}, and \texttt{join sizes}.
Labeled examples are provided in one of two supervision forms: pairs of related records, one from each table, or a triple where a record from $D_0$ is linked to a related and unrelated record from each $D_i$.
That is, unrelated examples are optional, but related ones are required.
Recall that we focus on the $M = 1$ case, but describe extensions in Sections~\ref{sec:preprocessing}-\ref{sec:joining}.

As output, \sys retrieves the data points enriched based on the \texttt{join type} and \texttt{join sizes} as a list of tuples.
Users configure \sys using a json configuration file that exposes the join specification and lower-level \sys-specific parameters (see Section~\ref{subsec:extensibility}).


%As output, \sys's default pipeline retrieves a list of the most related data points in the auxiliary source $D_1$ for each data point in $D_0$, where relatedness is learned using the provided labeled examples. 

\subsection{API and Architecture}
\label{subsec:arch}

Keyless joins learn a representation that quantifies data point relatedness, and retrieve these points regardless of the input schema. 
We propose a modular system with three architectural elements to enable this: data preprocessing, representation learning, and data joining.
\sys consists of dataflow operators that transform inputs into the formats required for each step (see Table~\ref{table:types}). 

\sys represents input data records $d_{ij}$ as {\records} in key-value pairs.
Supervision is represented via \labelers.
An \sys pipeline consists of {\preparers}, {\encoders}, \samplers, \losses, and \retrievers. 
\sys uses \preparers to transform \records into \sentences.
\sys uses \encoders to transform \sentences into \embeddings that are optimized per a provided \loss; \samplers mine negative examples if the provided supervision only provides examples of related records.
The trained \embeddings are stored in an index, and are retrieved using a \retriever.
We provide an API over these operators in the form of a customizable, high-level configuration, as described in Section~\ref{subsec:easy}.
To enable functionality beyond that described, users must implement additional \preparers, \encoders, \samplers, or \retrievers. 
Users configure \sys using pre-defined or custom operators, or use the following pre-configured default:  
%First, the system must represent records in a comparable format regardless of input schema. 
%Second, these representations must be automatically tuned to cluster related records. 
%Finally, related records must be efficiently retrieved. 
%\sys implements these elements via a three-step architecture consisting of 

\minihead{Preprocessing (Figure~\ref{fig:pipeline}A, \S\ref{sec:preprocessing})} \sys ingests any text or numeric data source with a pre-defined schema, and converts its records to a common representation. 
By default, \sys converts \records to \texttt{sentence}s using \texttt{sentence preparer} modules, which are fed as input to the pipeline's \texttt{encoders}. 
\sys optionally pretrains the \texttt{encoders} in this step using self-supervision.

\minihead{Representation Learning (Figure~\ref{fig:pipeline}B, \S\ref{sec:representation})} \sys learns a mapping for each input data source's \records such that the transformed data is clustered by relatedness. 
To learn this mapping, \sys's \texttt{encoders} are fine-tuned with the input supervision (in the form of a \texttt{labeler}) and \texttt{loss}.
\sys applies the learned mapping to each of the \sentences to generate \embeddings passed to the final step.
%\sys currently only supports a contrastive triplet loss, and thus converts pairwise binary supervision into triplets using a negative \texttt{sampler}.


\minihead{Joining (Figure~\ref{fig:pipeline}C \S\ref{sec:joining})} \sys populates an index with the learned \embeddings using Faiss~\citep{faiss}. 
A keyless join can be completed by issuing a similarity search query given an input \record (transformed to an \embedding) against this index.
The dataset that is indexed is determined by the \texttt{join type}. 
\sys uses a k-NN \texttt{retriever} module to retrieve as many records specified by the \texttt{join sizes}. 
%Users can specify how many records should be returned and to what similarity sensitivity by configuring a \texttt{retriever} to enable both one-to-one and one-to-many join semantics. 




==> context enrichment 8/evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

In this section, we demonstrate that \sys and its operators are:

\begin{enumerate}
    \item \textbf{General}: \sys enables context enrichment across five domains while meeting or exceeding similarity-join baseline recall and query runtime performance (Section~\ref{subsec:general}). 
    \item \textbf{Extensible}: \sys provides a modular architecture, where each component affects performance (Section~\ref{subsec:micros}). \sys enables task-specific pipelines for various similarity-based queries, and provides task performance that can be fine-tuned by state-of-the-art systems (Section~\ref{subsec:extensibility}). 
    \item \textbf{Low Effort}: \sys requires no more than five configuration changes (Table~\ref{table:datasets}) from its default, and does not always require large amounts of hand-labeled examples (Section~\ref{subsec:easy}).
\end{enumerate}


\input{tables/datasets}

\subsection{Evaluation Metric and Applications}

\minihead{Context Enrichment Evaluation Metric} Context enrichment identifies related records across a base and auxiliary dataset. 
We can view related records between the two datasets as forming edges in a bipartite graph: each record in each dataset represents a vertex in the graph. 
Under this framing, a context enrichment system must retrieve all of the outgoing edges (i.e., related records) for each record in the base dataset.
This is equivalent to maximizing record-level recall, or the fraction of records for which we recover \emph{all} related records. 
We choose to define recall at the record-level, rather than the edge-level, as we view context enrichment systems as being repeatedly queried for new incoming data once instantiated. 

A na\"ive means to optimize for recall is to return \textit{all} auxiliary records as being related to each record in the base dataset. 
A precision metric greatly drops when we retrieve multiple records.
Thus, our evaluation metric is \textbf{recall@k}, for small k (i.e., \texttt{join size}).
% and the k required to reach a fixed recall threshold given a set of ground-truth related pairs, which we denote as k-to-thresh.} 

\minihead{Applications} We evaluate \sys against workloads from five application domains: fuzzy joining, entity matching, search, question answering, and recommendation (summarized in in Table~\ref{table:datasets}). 
We make all our datasets publicly available post-\sys processing. 

\subsubsection{Fuzzy Join (FJ)}
We build two workloads using a dataset and generation procedure from a 2019 scalable fuzzy join VLDB paper~\citep{surajit}. 
The first dataset consists of the Title, Year, and Genre columns from IMDb~\citep{imdb}.
The second dataset is generated by perturbing each row in the first by applying a combination of token insertion, token deletion, and token replacement. 
The task $T$, is to join each perturbed row with the row that generated it.
%The candidate key columns are all of the columns selected for perturbation.
We generate two dataset versions: 5 perturbations per row (IMDb) and 15 perturbations per row (IMDb-hard), up to 25\% of the record length. 
As we focus on generalizablity more than scalability, to form a dataset, we randomly sample 10,000 movies and generate 5 perturbed rows for each. 
We hold out 20\% of records as the test set; no records from the same unperturbed record are in both the train and test sets.
%Supervision is provided as a list of related pairs. 

\subsubsection{Entity Matching (EM)}
We use all 13 benchmark datasets~\citep{dmdata} released with DeepMatcher~\citep{deepmatcher}, spanning structured (EM-S), textual (EM-T), and dirty (EM-D) entity matching. 
The base and auxiliary datasets always share the same schema. 
In EM-T, all data records are raw text entries or descriptions. 
In EM-S, each data record is drawn from a table following a pre-defined schema, where text-based column values are restricted in length. 
In EM-D, records are similar to EM-S, but some column values are injected into the incorrect column.
The task $T$ is to label a record pair (one from each dataset) as representing the same entity or not. %; the evaluation criteria the F1 score. 
Train, validation, and test supervision are lists of unrelated, and related pairs---we only use the related pairs for training \sys, as we identified mislabeled entries (false negatives) when using \sys to explore results.


\subsubsection{Search (S)}
We use the MS MARCO passage retrieval benchmark~\citep{marco}.
MS MARCO consists of a collection of passages from web pages that were gathered by sampling and anonymizing Bing logs from real queries~\citep{marco}. 
The task $T$ is to rank the passage(s) that are relevant to a given query as highly as possible. %; the evaluation criteria is MRR@10. %, which we compute over the provided dev set.
Supervision is a set of 397M triples, with 1 relevant and up to 999 irrelevant passages for most queries.
Irrelevant passages are retrieved via BM25.
We report results over the publicly available labeled development set. 
%Results over the full test set were only available upon benchmark submission; we instead report results over the smaller dev set.% similar to a test set by only using it for final evaluation. %, where only very few (often a single) passages are marked as relevant for a given query.


\subsubsection{Question Answering (QA)}
We modify the Stanford Question Answering Dataset (SQuAD)~\citep{squad}.
SQuAD consists of Wikipedia passages and questions corresponding to each passage. 
The task $T$ is to identify the beginning of the text span containing the answer to each question. 
As described in Section~\ref{sec:applications}, a retriever module, used in retriever-reader models for QA~\citep{retriever}, performs context enrichment.
We modify SQuAD by splitting each each passage at the sentence-level, and combining these sentences to form a new dataset. 
The modified task is to recover the sentence containing the answer.%, rather than the exact text span.

\subsubsection{Recommendation (R)}
We construct a workload using IMDb and Wikipedia to mimic the e-commerce example from Figure~\ref{fig:example}.
%We construct similarity-based aggregation for recommendation workload similar to the e-commerce example in the introduction using the IMDb and Wikipedia datasets. 
For the first dataset, we denormalize four IMDb tables using KFK joins: movie information (title.basics), principal cast/crew for each movie (title.principals) and their information (name.basics), and movie ratings (title.ratings)~\citep{imdb}.
%We replace null values with a `\textbackslash~N' character. 
For the second dataset, we extract the summary paragraphs of the Wikipedia entry for each IMDb movie by querying latest Wikipedia snapshot; we extract 47813 overlapping records~\citep{wiki}.
We remove the IMDb ID that provides a KFK relationship to induce a need for keyless joins.
We construct this workload to enable two applications. 
In Application A, we show that \sys can join datasets with dramatically different schema. %This is performed over dataset IMDb-wiki-join.  
In Application B, we show how to estimate the rating for movies in the test set given ratings for the train set by performing similarity-based analyses enabled by \sys. 
% where the objective is to predict the review of a new movie
Supervision is provided as exact matches and movie ratings with an 80-20 train-test set split.

%This is performed over dataset IMDb-wiki-rec (same as IMDb-wiki-join, but with an additional ratings column in the train dataset). 
%The second goal is analogous to the initial e-commerce example where the objective is to predict the review of a new movie.

\input{tables/baselines}

%We provide detailed explanations about each dataset in their respective case studies.

\eat{\minihead{Evaluation Metrics} We evaluate all EM workloads with respect to F1 score, as is standard in existing work~\citep{deepmatcher,ditto}.
For the remainder of the workloads, we report MRR@k and Retrieval@k for k = 1, 10. 
MRR@k refers to the average of the multiplicative inverse of the rank of the first relevant item in the top k ranked items, and is an information retrieval standard~\citep{marco}.
We define Retrieval@k to be the percentage of the test set whose true match is present in the top-k returned nearest neighbors by the \retriever. 
We report Retrieval@k as a modification of Recall@k, to reflect that we are only looking for a single match in these join scenarios.
MRR@1 is equivalent to Retrieval@1.}

\subsection{Experimental Setup}
\label{sec:setup}

\minihead{Baselines} We first evaluate all workloads compared to seven similarity-based joins with respect to recall@1 and recall@10. 
Our baselines are joins using Levenshtein distance, four variations of Jaccard Similarity, BM25, Auto-FuzzyJoin~\citep{autofj}, and a pretrained embedding-based approach. 
We evaluate downstream EM and search workloads with respect to previously reported state-of-the-art and benchmark solutions~\citep{deepmatcher,deeper,ditto,marcohomepage,bertmarco}.
%We evaluate downstream EM workloads with respect to previously reported state-of-the-art~\citep{deepmatcher,deeper,ditto}. 
%For the search workload, we provide comparison against reported BM25 and BERT baselines, and state-of-the-art~\citep{marcohomepage,bertmarco}. 
The remainder of our workloads were constructed to isolate context enrichment from the downstream task, and do not have standard baselines. 

\minihead{\sys Default Configuration} Tasks use a \sentence \preparer, and perform 20 epochs of self-supervised pretraining.
\sys uses a single DistilBERT$_{\text{base}}$ \encoder trained with a triplet \loss and \red{stratified} hard negative \sampler. %when triples are not provided by the user.
Self-supervision and the \sampler use BM25 to identify similar \sentences to concatenate from each data source, and to mark as hard negatives, respectively. 
The output \embedding size is 200, and models are trained with a batch size of 8 using an ADAM optimizer~\citep{adam} with initial learning rate of $1\mathrm{e}{-5}$.
The default \texttt{join sizes} are 1 and 10.
Results are five-trial averages.


\minihead{Implementation} We use a server with two Intel Xeon Gold 6132 CPUs (56 threads) with 504GB of RAM, and four Titan V GPUs with 12GB of memory.
We implement \sys in Python and PyTorch~\citep{pytorch}, with pretrained models and tokenizers from HuggingFace Transformers~\citep{hf}. 
We use Faiss for MIPS~\citep{faiss}, Magellan for similarity join baselines~\citep{magellan}, rank-BM25 for BM25~\citep{bm25_code}, and AutoFuzzyJoin~\citep{autofj}.


\subsection{Generalizability}
\label{subsec:general}

We show that \sys's recall and runtime meets or outperforms that of the following similarity-join baselines in nearly all tasks:

\minihead{Levenshtein-Distance (LD)} LD is the number of character edits needed to convert one string to another. 
This join returns the closest records with respect to single-character edits over provided key columns. We filter and only return results under a 30 edit threshold.


\minihead{Jaccard-Similarity, Specified Key (JK-WS, JK-2G)} The Jaccard similarity between sets $A$ and $B$ is $J(A, B) = \frac{|A\cap B|}{|A \cup B|}$.
Defining a Jaccard-similarity based join over textual inputs requires tokenizer selection.
We consider a whitespace tokenizer (WS) and a 2-gram tokenizer (2G) to capture different granularities. 
JK-WS and JK-2G return the closest records with respect to Jaccard similarity over provided key columns using a WS or 2G tokenizer.
We set a filtering threshold to return results with at least 0.3 Jaccard similarity.

\minihead{Jaccard-Similarity, Unspecified Key (J-WS, J-2G)} J-WS and J-2G return the closest records with respect to Jaccard similarity using a WS or 2G tokenizer, after a \sentence \preparer.
We set a filtering threshold to return results with over 0.3 Jaccard similarity.

\minihead{BM25 (BM25)} BM25 is a bag-of-words ranking function used in retrieval~\citep{bm25}. This join returns the closest records with respect to the Okapi BM25 score using default parameters k1=1.5 and b=0.75.

\minihead{Pretrained-Embedding (BERT)}
%Pretrained Transformer-based embeddings can be used to perform similarity-based queries over common vocabularies. 
BERT generates embeddings for each prepared \sentence via a pretrained DistilBERT$_{\text{base}}$ model, and returns the closest records based on the $\ell_2$-norm between them. 

\red{\minihead{Auto-FuzzyJoin (AutoFJ)}
AutoFJ automatically identifies join functions for unsupervised similarity joins~\citep{autofj} by assuming one input is a "reference table" with few or no duplicates, which does not always hold in context enrichment.
If duplicates are present, or records in the reference table are not sufficiently spread, precision estimation may break down (\sys trivially accounts for these scenarios).
AutoFJ optimizes for a precision target, and does not expose any \texttt{join size} semantics.
We find a single result is typically returned per record, so we only consider recall@1 at a low precision target of 0.5. 
We comment on workloads that completed in 1.5 days on our machines using all cores. 
As AutoFJ exhaustively computes record similarities for each considered join configuration, this means we omit results for MS MARCO, EM-T Company, EM-S BeerAdvo-RateBeer, and several others consisting of large text spans, or where blocking may not be as effective.
Users must manually align \emph{matching} columns, which do not always exist thus ignore information in our tasks (e.g., IMDb-wiki): as input, we pass the output of a \sentence \preparer if column names are not identical.
}
\\

\noindent For multi-column datasets, we provide a plausible key column if the method requires.
In FJ, EM, and R, this is a title or name column. 

\subsubsection{Retrieval Quality} We show that \sys is competitive with or exceeds the best performing alternatives with respect to Recall@1 and Recall@10 (Table~\ref{tab:baselines}). 
In both tables, we highlight the methods that are within 1\% of the top performing method. 
No method dominates the others across the different workloads, while BERT underperformed all alternatives.  
Broadly, character-based joins (LD, JK-2G, J-2G) tend to perform well in scenarios where a join key exists but may be perturbed (FJ, EM-S, EM-D); word-based joins (J-WS, BM25) tend to perform well in scenarios with word-level join keys (EM-S), or where a join key does not exist but common phrases still link the two datasets (R, EM-D).
Neither performs well otherwise (S, EM-T).
\sys most consistently outperforms or is comparable with alternatives across the tasks: a learned approach is necessary for generalization. 
The exception is with the synthetic FJ workload that is, by construction, suited for character-based joins. 

\red{We do not report AutoFJ in Table~\ref{tab:baselines} due to incompleteness. 
AutoFJ is tailored for the EM and FJ: many-to-one joins with identical schema. 
Of those completed, \sys is sometimes outperformed by up to 8\% recall@1 (Amazon-Google), but is otherwise comparable or far exceeds AutoFJ when considering recall@10.
%For FJ, if the user realizes AutoFJ retrieved a single match for each record in the unperturbed dataset due to the focus on precision
AutoFJ's recall is 37.9\% for QA, and 38.5\% for R.
As AutoFJ over the Wikipedia summary (task R) did not terminate, we only use the title column.
}

\subsubsection{Query Runtime} Using optimized MIPS routines improved query runtime performance by up to two orders of magnitude.
We note that this reflects \sys joining time, not pretraining and representation learning, which may require several hours.
As the two FJ datasets are synthetic and follow identical generation methods, we consider just IMDb-hard.
For our largest dataset, MS MARCO (S) with 8.8M auxiliary records, \sys indexes and retrieves results from the entire corpus, but each baseline only considers each of the up to 1000 relevant records provided by the MS MARCO dataset for each base record. 
Even when using CPU-only Faiss~\citep{faiss}, \sys takes \red{7.24} seconds on average for the MIPS-based joining step. 
Embedding the query table takes \red{24.52} seconds on average.
The most expensive dataset with respect to MIPS runtime is MS MARCO (S), which required \red{1.97} minutes when indexing all 8.8M records; excluding it reduces the average to \red{0.31} seconds.
For embedding time, this was EM-T Company, requiring \red{3.96} minutes, whose exclusion reduces the average to \red{11.19} seconds.
In contrast, the fastest baseline method (JK-WS), took \red{5.02} minutes on average; excluding MS MARCO (\red{79.73} minutes) reduces the average to \red{21.18} seconds.
The slowest method (LD), took \red{23.64} minutes on average, with the most expensive dataset, EM-T Company, requiring \red{321.98} minutes.

%\input{tables/baselines-k}


\subsection{Extensibility: Architecture Lesion}
\label{subsec:micros}
We demonstrate modularity and justify our architectural defaults by evaluating \sys's performance when modifying components as follows, each of which requires a single line configuration change (all reported percentages are relative unless explicitly specified): 
\begin{enumerate}
    \item Replacing MLM pretraining and representation learning (RL) with a pretrained \encoder.
    \item Removing RL, leaving only MLM pretraining.
    \item Replacing the fine-tuned Transformer model with a frozen pretrained embedding and a learned dense layer.
    \item Removing MLM pretraining.
    \item Random negatives compared to hard negative sampling
    \item Using an \encoder for each dataset versus a single \encoder.
    \item Removing the joining index-query optimization.
\end{enumerate}

\subsubsection{Pretrained \encoder (\textsc{-mlm, rl})}
We remove MLM pretraining and RL, and use a pretrained DistilBERT$_{\text{base}}$ encoder---i.e., the same as BERT in Table~\ref{tab:baselines}. 
%We report our results in Table~\ref{table:micros} in terms of the relative difference from \sys's default. 
We report our results in Figure~\ref{fig:lesion} normalized by \sys's default. 
\sys's performance dramatically declines, sometimes by three orders of magnitude (e.g., recall dropped to 0.04 in R).
It is only feasible when the contents of the datasets to be joined are similar, as in certain EM-S and EM-D tasks, and FJ-IMDb. 


\subsubsection{Removing Representation Learning (\textsc{-rl})}
We remove representation learning (RL) and only pretrain an \encoder using the BM25-based MLM procedure from Section~\ref{sec:preprocessing}.
%In scenarios where a user is unable to provide any form of supervision, \sys must fall back to this setting. 
%We report our results in Table~\ref{table:micros} in terms of the relative difference from \sys's default.
We report our results in Figure~\ref{fig:lesion}. 
\sys's performance declines by up to an order of magnitude, though it improves performance compared to \textsc{-mlm, rl} on tasks whose datasets do not match the original natural text Wikipedia corpus (e.g., EM-S, FJ). 
Primarily textual datasets do not see as large an improvement over \textsc{-mlm, rl}, and for QA, where the corpus is derived from Wikipedia, \textsc{-rl} performs slightly worse.

\subsubsection{Remove Transformer fine-tuning (\textsc{-ft})}
We replace RL with fixed MLM pretrained embeddings followed by a learned fully-connected layer (i.e., we do not fine tune the entire BERT-based \encoder, just the final output layer). 
%We report our results in Table~\ref{table:micros}.
We report our results in Figure~\ref{fig:lesion}.
Without end-to-end Transformer fine-tuning, \sys slightly outperforms using just a pretrained encoder (\textsc{-rl}) at times. 
We primarily observe benefits in text-heavy workloads, where the pretrained encoder provides meaningful representations (QA, S, R, EM-T) without relying on positional information from Transformers. 
While we do not perform an exhaustive comparison of pretrained embeddings or non-Transformer-based architectures, this shows that \sys's architecture is a strong out-of-the-box baseline. 

\subsubsection{Remove MLM Pretraining (\textsc{-mlm})}
%We eliminate MLM pretraining from the pipeline, and report our results in Table~\ref{table:micros} as \textsc{-mlm}.
We eliminate MLM pretraining from the pipeline, and report our results in Figure~\ref{fig:lesion} as \textsc{-mlm}.
\sys meets or exceeds this setting in all but QA, though by a smaller margin than the previous experiments (up to 20.5\% in IMDb-hard). 
MLM pretraining is not effective for QA as the corpus is drawn from Wikipedia---one of the two corpora BERT was trained with---and both base and auxiliary datasets consist of the same, primarily textual vocabulary. 
In such cases, users may wish to disable MLM pretraining, although performance is not significantly impacted.
In contrast, of the non-EM tasks, MLM pretraining is most helpful for FJ IMDb-hard, where random perturbations result in many records with words that are not in the original vocabulary. 
%In addition, the largest gains from MLM pretraining arise in the purely structured EM-S and EM-D tasks.
%This validates the optimization we describe in Section~\ref{sec:preprocessing}, where we only perform MLM pretraining for structured datasets whose content differs from the original BERT pretraining datasets.


\subsubsection{No Negative Sampling (\textsc{-NS})}
We replace hard negative sampling with random sampling of unrelated records, and report our results in Figure~\ref{fig:lesion}. 
Hard negative sampling tends to improve performance by a similar margin as MLM pretraining, and only negatively impacted the EM-T Company dataset (by up to 8.72\% absolute recall). 
We find larger improvements when the join condition is more ambiguous than recovering a potentially obfuscated join key, as in tasks S (30\% R@1), QA (15\% R@1), and EM-D (15\% R@1).
We use BM25-based sampling for all but FJ and QA, where we have prior knowledge, and develop custom samplers based on Jaccard similarity, and sentence origin, respectively.
This improved performance over the BM25-based sampler by 1\% absolute recall for FJ, and 8.7\% and 5.6\% absolute recall@1 and recall@10, respectively, for QA.


\begin{figure*}
\includegraphics[width=\textwidth]{figures/lesion_s.pdf}
\caption{Architecture lesion displaying recall@k normalized to the default seen in Table~\ref{tab:baselines} (All) for: a pretrained DistilBERT$_{\text{base}}$ model with no representation learning (\textsc{-mlm,rl}), MLM pretraining with no RL (\textsc{-rl}), RL with no Transformer fine tuning (\textsc{-ft}), RL with no MLM pretraining (\textsc{-mlm}), no hard negative sampling (\textsc{-ns}), and one encoder per dataset (\textsc{te}).}
\label{fig:lesion}
\end{figure*}

\subsubsection{\encoder Configuration (\textsc{te})}
%We use two \encoders, one for each dataset, instead of our default single \encoder configuration (all DistilBERT$_{base}$), and report our results in Table~\ref{table:micros}. 
We use two \encoders, one for each dataset, instead of our default single \encoder configuration, and report our results in Figure~\ref{fig:lesion}. 
We find that using two \encoders performs up to two orders of magnitude worse than using a single encoder, especially for strictly structured datasets.
We observe that through the course of the \encoder training procedure, the performance of using two identically initialized \encoders often \emph{degrades}---inspecting the resulting embeddings even when running \sys over two identical tables shows that the exact same terms diverge from one another in the training process.
However, we still provide the option to use a distinct encoder for each data source for future extension to non text-based data, such as audio or image. 


\subsubsection{Index Optimization}
For \texttt{INNER} and \texttt{FULL OUTER JOIN}s, we optimize for join execution time by indexing the larger dataset, which reduces the number of queries made by the system.
Due to \encoder training, this reflects a small fraction of the end-to-end pipeline execution time at our data sizes, but can be a substantial cost at scale.
We evaluate this optimization by running the joining step while indexing the larger dataset, and then the smaller dataset for \emph{all} tasks. 
On average, this optimization reduces join time by \red{1.76}$\times$, and up to \red{2.81}$\times$. However, this improvement is only meaningful in the MS MARCO workload, saving \red{2.7} minutes. 
%In the single-thread setting, we reduce join time by \red{XXX}$\times$, and up to \red{XXX}$\times$, where we save \red{YYY} minutes  in MS MARCO.

\subsection{Extensibility: End-to-End Workloads}
\label{subsec:extensibility}
We show how to extend and use \sys in an end-to-end context. 

\minihead{Entity Matching} Recent deep-learning-based EM systems focus on the matching phase of that two-part (i.e., blocking and matching) end-to-end EM pipeline~\citep{deeper,deepmatcher,ditto}: given a pair of candidate records, these systems must identify if the pair correspond to the same entity.  
For end-to-end EM, \sys must generate candidate blocks with a low rate of false negatives such that it can be efficiently followed by downstream matchers; we verify this in Table~\ref{table:dm_all} (R@10).
Perhaps surprisingly, we find that treating \sys results from a top-1 query as binary classifier achieves performance that is comparable to or better than previous, custom-built state-of-the-art with respect to F1 score.
We believe incorporating general operators for data augmentation and domain knowledge integration to enable the custom advances presented in the current state-of-the-art EM system, Ditto, may allow \sys to entirely bridge this gap~\citep{ditto}. 

\input{tables/dm}

\minihead{Search} In MS MARCO passage ranking, results are ranked in relevance order, and rankings are evaluated via mean reciprocal rank (MRR) of the top 10 results. 
We rank \sys results based on their query distance, and compare MRR@10 with existing MS MARCO  baselines.
We obtain \red{MRR@10 of $0.266$} on the dev set after just 2.5M training examples, outperforming the official Anserini BM25 baseline solution of $0.167$.
Our results exceed K-NRM, a kernel based neural model, with a dev set MRR@10 of 0.218~\citep{knrm}, and is slightly below the state-of-the-art from the time, IRNet, with 0.278 MRR@10~\citep{marcohomepage}. 
For comparison, the first state-of-the-art BERT-based model uses BERT$_\text{large}$ to achieve MRR@10 of 0.365 after training with 12.8M examples~\citep{bertmarco}, and current state-of-the-art is 0.439~\citep{rocketqa}. 
By developing an additional joining operator, \sys can implement ColBERT~\citep{colbert}, a previous state-of-the-art method that achieves 0.384 MRR@10 in MS MARCO document ranking that operates on larger input passages: we must remove the pooling step from \sys's \encoder (1 line config change), and develop a \retriever that indexes and retrieves bags of embeddings for each record. %0.167 
%\minihead{Question Answering} Need to get the package working...

\minihead{Recommendation} In Application B of task R, we estimate the IMDb ratings of movies in the test set given a training dataset and Wikipedia corpus.
We report the mean squared error (MSE) between the rating estimates and the true rating.
The task is easy: predicting the average training rating returns 1.19 MSE, and a gradient-boosted decision tree (GBDT) over the joined data returns 0.82 MSE.
We aim to show extensibility while meeting GBDT performance.

There are two approaches to enable this analysis with \sys by reusing the representation learned for the IMDb-wiki task: similarity defined in a single hop in terms of the labeled training data, or by first going through the Wikipedia data in two hops.

In the first method, users configure \sys to index labeled IMDb training data (with ratings) and retrieve records related to the test data (without ratings) via an \texttt{INNER JOIN}. 
Users then post-process the output by averaging the labels of the returned \records.
%This requires 3 lines of config changes, and a 7-line post-processing module.
In the second method, users require two \texttt{LEFT JOIN}s that index the Wikipedia training data against the IMDb test dataset, and the IMDb train dataset against the Wikipedia training data. 
Following a two-hop methodology, users first retrieve the closest Wikipedia summary to each test IMDb record, and then 
retrieve the closest labeled IMDb instances to each previously retrieved Wikipedia summary, which is post-processed via averaging. 

Both approaches reuse the pretrained encoder from the IMDb-wiki task, and require at most \red{6} configuration changes and a 7-line post-processing module.
We report results when aggregating with a \texttt{join size} of 1, 10, 20, and 30; both approaches improve performance as the number of neighbors increase, until a plateau is reached. 
The two-hop approach attains MSE of 1.69, 0.92, 0.89, and 0.89 for \texttt{join size} 1, 10, 20, and 30, respectively, while the one-hop approach performs better with 1.59, 0.89, 0.86, and 0.85. 




\subsection{Low Development Effort}
\label{subsec:easy}

We describe \sys's configuration to show the low number of config changes we made, and comment on the supervision required.

\subsubsection{Configuration}
Perhaps surprisingly, we found that exposing only join specification parameters (Listing~\ref{listing:config}) is a strong out-of-the-box baseline.
We require input datasets and supervision to follow a fixed naming convention, under which obtaining the results in Table~\ref{tab:baselines} relies on a default set of configurations options, where only the data directory must be changed.
%In Table~\ref{table:datasets}, we list how many config changes are required for the best results from Table~\ref{table:micros}.
In Table~\ref{table:datasets}, we list how many config changes are required for the best results from Figure~\ref{fig:lesion}.
\eat{
%\begin{Listing}[t]
%\small
\begin{lstlisting}[frame=single,caption={Core configuration lines annotated with options.},captionpos=b,float=t,label={listing:config}]
\begin{Verbatim}[commandchars=\\\{\}]
\small
\dred{"data_dir"}: \dred{"IMDb-wiki"},      
\dred{"join_type"}: \dred{"INNER"},    \textcolor{teal}{# or "LEFT", "RIGHT", "FULL"}
\dred{"left_size"}: 1,
\dred{"right_size"}: 1,
\end{Verbatim}
\end{lstlisting}
}


%\begin{Listing}[t]
%\small

\begin{lstlisting}[frame=single,caption={Core configuration lines annotated with options.},captionpos=b,float=t,label={listing:config}, language=Python,basicstyle=\small,commentstyle=\textcolor{teal},stringstyle=\dred]
"data_dir": "IMDb-wiki",      
"join_type": "INNER", # or "LEFT", "RIGHT", "FULL"
"left_size": 1,
"right_size": 1,
\end{lstlisting}



%We generate each microbenchmark in Table~\ref{table:micros} by altering the following unsurfaced configuration options: number of encoders, encoder intialization, encoder finetuning (boolean), fraction of supervision used, negative sampler.
We generate each result in Figure~\ref{fig:lesion} by altering the following unsurfaced options: number of encoders, encoder intialization, encoder finetuning (boolean), fraction of supervision, negative sampler.
Users can additionally specify lower-level hyperparameters, which we fix across our experiments: epochs, batch size, embedding size, pooling type, tokenizer, learning rate, loss function parameters.


\eat{
\subsubsection{FJ: 1 Line Changed}
\label{case:FJ}
As an FJ task is symmetric (i.e., there is no difference between which dataset is considered the base or auxiliary for the downstream task), \sys can rely on the default configuration and indexing optimization to index the smaller of the two tables.
This requires a change in the input directory path in the config file. 




%However, in this scenario, we note that returning recall@1 will not identify all possible matches due to one-to-many join semantics; the user must create a post-processing script to instead being analyses at recall@5 (i.e., the number of perturbed rows generated). 
%To avoid this overhead, the user can instead modify the default configuration to skip this 
%we have two options when using \sys. 
%In the first option, we set the perturbed dataset as the base dataset $D_0$ to be queried, and the original dataset as the auxiliary dataset $D_1$ to be indexed. 
%In this scenario, using the default operators to identify the closest records in $D_1$ to each record in $D_0$ will return the true join. 
%In the second option, we reverse the roles of the two datasets. 
%In this scenario, we note that returning recall@1 will not identify all possible matches due to the one-to-many join semantics; the user must create a post-processing scirpt to instead being analyses at recall@5 (i.e., the number of perturbed rows generated). 
%Both scenarios require one change in the input directory path in the config file. 

%In the second option, we reverse the roles of the two datasets. 
%All operators remain identical, but a post-processing module must be included to account for the many-to-one  except for the \retriever: the user must change the \retriever configuration to return the top five closest records to each row .
%This requires 3 changes to the config file. 
%In this case study, we choose to perform the simpler, first scenario.

\subsubsection{EM: 1 or 2 Lines Changed}
\label{case:EM}
EM tasks are symmetric.
Thus, we rely on the indexing optimization to index the smaller of the two tables.
As the output task is based on pairwise labels, given a pair of records that refer to as the query and target, we define a positive match as one where the target record is in the set of retrieved neighbors when querying \sys's index with the query record.
The default configuration retrieves a single neighbor, and requires a single config change.
To retrieve multiple neighbors requires an additional line changed.
First, we can simply treat the closest retrieved record as a predicted positive example, and all other records as negatives. 
Our result post-processing script consists of a 9-lines of python code to process the retrieved results and compute the necessary precision, recall, and F1 metrics. 

%\input{tables/retrieval}

\subsubsection{S: 2 Lines Changed}
\label{case:IR}
We denote the dataset with the queries as the base dataset, and the passage collection as the auxiliary dataset as the goal is to retrieve passages relevant to each query.
This is the configuration set by \sys's default indexing optimization, as the passage collection is the larger of the two. 
Thus, we preserve the default configuration, but modify the \retriever to return the top 10 most related \records, and add a post-processing module that computes MRR. 
This requires 2 changes to the config file, and our post-processing module consists of 11 lines of code.


\subsubsection{QA: 2 Lines Changed}
\label{case:QA}
For the QA task, we denote the question dataset as the base dataset, and the collection of sentences as the auxiliary dataset. 
The sentence corpus is smaller than the question corpus, thus, we override the indexing optimization. 
As the SQuAD corpus is based off Wikipedia, the dataset is of the same vocabulary as the pretraining corpus used by BERT.
Thus, \sys does not perform MLM pretraining by default.
Overriding the indexing optimization requires one configuration line edited.


\subsubsection{R Application A: 1 Line Changed}
\label{case:rec}
As both datasets are the same size, the choice of base and auxiliary dataset is irrelevant. This is a standard context enrichment problem, thus we preserve the default configuration for the join task. 

\subsubsection{R Application B: 3 or 5 Lines Changed} One means of solving the second application is to identify movies in the test set that are similar to those in the train set (with ratings), and aggregate the rating of the similar movies as the predicted rating. 
\sys can perform this operation with similarity defined in a single hop, in terms of the labeled training data, or in two hops, by first going through the Wikipedia data.
We report the performance of both.
In either instance---as there are no labeled examples connecting the train and test data---users retain the default operator configuration up to the representation learning step.

In the first method, users configure \sys to index labeled IMDb training data (with ratings), and retrieve records related to the test data (without ratings) with a \retriever set to return multiple related (labeled) records. The user then post-processes the output by averaging the labels of the returned \records.
This requires 3 lines of config changes, and a 7-line post-processing module.

In the second method, users configure \sys to index both the train Wikipedia and IMDb dataset. 
Following a two-hop methodology, users then configure a standard \retriever over the Wikipedia index that returns the closest Wikipedia summary to each test IMDb record. 
Users configure a second \retriever over the IMDb train dataset that returns the closest labeled IMDb instances to each previously retrieved Wikipedia summary, which can then be post-processed via averaging. 
This requires 5 lines of config changes, and a 7-line post-processing module
}

\subsubsection{Dependence on Labeled Data}
A key user input is labeled examples of relevant record pairs.
%With the exception of MS MARCO, we use all available labeled examples of \textit{relevant pairs} in Tables~\ref{tab:baselines} and~\ref{table:micros}.
With the exception of MS MARCO, we use all available labeled examples of \textit{relevant pairs} in Table~\ref{tab:baselines} and Figure~\ref{fig:lesion}.
In MS MARCO, we use 2.5M of the 397M of the provided labeled \textit{triples}, which is just $0.63\%$ of the provided triples.
For the remaining datasets, we evaluate how many labeled examples are required to match performance of our reported results. 
We found that 9 of the 17 datasets required all of the provided examples.
The remaining datasets required $54.4\%$ of labeled relevant data on average to meet Recall@1 performance, and $44.5\%$ for Recall@10. 
In the best case, for EM-S DBLP-ACM, only $30\%$ and $1\%$ of the data is required to achieve the same Recall@1 and Recall@10, respectively.

==> context enrichment 8/grave.tex <==


%\red{[Structured data has hobbled along compared to unstructured data.]}
%Machine learning (ML) systems increasingly power critical applications spanning search, recommendation, and question answering~\citep{ml1, ml2, ml3}. 
%However, this ML revolution has largely influenced unstructured data, such as image, video, and natural language.
Machine learning (ML) systems thrive on context-rich information: methods to extract structural and semantic context from images~\citep{alexnet} and text~\citep{bert, gpt2} revolutionized computer vision and natural language processing tasks such as object detection and translation. 

%in computer vision, an image contains most of the context required to perform classification tasks, and in natural language processing, unsupervised textual data sources contain context that can be extracted using Transformers~\citep{transformers}, which has revolutionized tasks such as text generation and translation~\citep{bert,gpt2}.

\begin{figure}
\includegraphics[width=\columnwidth]{figures/tables.pdf}
\caption{An end-to-end task requiring context enrichment. Predicting the rating of and recommending a new product (\texttt{A82}), requires relating the Asics products (highlighted in dark gray) via a keyless join (top). This process is manual due to data heterogeneity---we aim to automate it (bottom).}
\label{fig:example}
\vspace{-1em}
\end{figure}

Unfortunately, structured data repositories, which consist of datasets with pre-defined schemas, suffer from context fragmentation: they commonly scatter information regarding a data record across domain-specific datasets with potentially unique schemas.
These datasets adhere to fixed schemas that are optimized for task-specific querying, and often lack explicit linking keys, such as primary key-foreign key (KFK) relationships.
This constrains users to a single view of an entity that is specialized for a specific business need. 
For instance, in Figure~\ref{fig:example}B, information regarding \textsc{Asics} shoes is scattered across three catalogs with unique schemas. 

Associating these fragmented data contexts is critical in enabling ML-powered applications over structured datasets---a process we denote as \emph{context enrichment}.
While modern, no-code ML systems are rapidly shifting practitioners towards higher-level abstractions for developing ML applications~\citep{ludwig, overton, h20, robot,gcloud}, context enrichment is still left as a user-performed data preparation step.\footnote{https://cloud.google.com/automl-tables/docs/prepare}
Consequently, engineers develop solutions for context enrichment tailored to their domain, such as similarity-based blocking in data integration~\citep{blocking}, retriever models in question answering~\citep{retriever}, or retrieval functions in search~\citep{bm25} (see Section~\ref{sec:applications}). 
However, constructing independent solutions is repetitive, time-consuming, and results in a complicated landscape of overlapping, domain-specific methods.
For instance, consider the scenario depicted in Figure~\ref{fig:example}:

%As a result, performing \emph{context enrichment}, or associating fragmented data contexts, is a pervasive need across a wide spectrum of ML-powered applications that operate over structured datasets, including recommendation, search, question answering, and data integration. 
%While modern no-code ML systems support the end-application given curated datasets, they leave context enrichment as a user-performed feature engineering step\footnote{https://cloud.google.com/automl-tables/docs/prepare}~\citep{ludwig, overton, gcloud}.
%Consequently, each vertical must construct independent, domain-specific solutions for their applications, which is time-consuming and repetitive.
%For instance, consider the following scenario (Figure~\ref{fig:example}):


\eat{
%Structured data repositories (i.e., data stores with a pre-defined schema) scatter context, or information regarding an entity or data record, across domain-specific datasets of differing schema.
%These datasets adhere to fixed schemas that are optimized for task-specific querying and manipulation, which constrains users to a single view of an entity that is specialized to a vertical or business need. 

%Context fragmentation is at odds with machine learning (ML) systems that thrive given context-rich features, as is typical of unstructured data: an image contains most of the context required to perform an image classification task, and leveraging context from unsupervised textual data sources via Transformers~\citep{transformers} revolutionized natural language processing~\citep{bert,gpt2}. 
%Thus, associating fragmented data contexts prior to performing downstream tasks, a process we refer to as \emph{context enrichment}, is a common and critical step to enable end-to-end ML systems for structured data.

%For instance, consider the following scenario (Figure~\ref{fig:example}):


%Machine learning (ML) systems have revolutionized applications over unstructured data, such as image, video, and natural language~\citep{ml1,ml2,ml3}.
%\emph{Structured} data (i.e., with a pre-defined schema) has not experienced the same success despite its prevalence~\citep{lakehouse}, largely due to context fragmentation.


%\red{[This disparity is because of a lack of context and datasets.]} \\
%A core reason for this disparity is that structured datasets scatter information regarding an entity or data point (i.e., \emph{context}) across numerous domain-specific datasets of differing schema.
%As these datasets are optimized for querying and manipulation, not ML, they adhere to fixed schemas, which constrain users to a single view of an entity that is specialized to a vertical or business needs. 
%As a result, information regarding an entity or data point (i.e., \emph{context}), is fragmented across numerous domain-specific datasets of differing schema, often with an unclear means of joining them~\citep{arda}.
%This fragmentation is at odds with ML models that thrive given abundant context-rich information, as is typical of unstructured data: a single image contains most of the context required to perform an image classification task, and leveraging context from unsupervised textual data sources via transformers~\citep{transformers} revolutionized natural language processing~\citep{bert,gpt2}. 


%\red{[We need to associate these contexts to enable ML]} \\
%Associating these fragmented data contexts prior to performing downstream tasks, a process we refer to as \emph{context enrichment}, is key to enabling the next-generation of ML systems for structured data.
%For instance, consider the following scenario (Figure~\ref{fig:example}):
%A natural question that arises is, how can we associate disparate information sources for the same real-world entity (e.g., product), to enable the next-generation of data analytics platforms? 
}
%\vspace{5pt}
\vspace{-7pt}
\emph{\\An e-commerce company has a proprietary product catalog, and aggregates product information from several external vendors to perform market analysis. 
Each vendor uses a unique product catalog, each with unique product representations (i.e., schema) ranging from free-form text to tabular product descriptions; products may overlap and evolve (Figure~\ref{fig:example}B).
Given normalized tables containing user and rating data, an engineer wishes to estimate the rating for a candidate new product (\texttt{A82}) and identify users to recommend the product to (Figure~\ref{fig:example}A).
%While the company has labeled a small number of product matches across the different catalogs, no global product identifier exists as a unifying join key.
%The engineer must join products across catalogs, and display those relevant to the user.
}
\vspace{5pt}


The engineer must first perform context enrichment by joining information across tables to extract features that capture similarities between the new (\texttt{A82}) and existing (\texttt{A80}, \texttt{P8}) products.
The engineer can then estimate the product rating, and recommend the new product to users based on how they rated related products.


The classic data management approach is to denormalize datasets using KFK joins. 
However, not all tables can be joined when relying on only KFK relationships.
For instance, there is no KFK relationship between Catalog B and Catalogs A or C; no join key unites fundamentally disparate product catalogs. 
Even when KFK relationships exist, as between Catalogs A and C (\textsc{\texttt{ITEM}}), relying on just KFK semantics will fail to capture the similarity between \texttt{A82} and \texttt{A80}.
The engineer must realize that the \texttt{Description} column in Catalog A relates to the \texttt{Brand} and \texttt{Model} columns in Catalog B and the \texttt{Size}, \texttt{Make}, and \texttt{Color} columns in Catalog C, and then perform a custom similarity-based join depending on the two tables---e.g., a join based on Jaccard similarity or Levenshtein distance.
%The engineer must perform this join for all modified products, and may have to repeat this entire procedure as catalogs evolve. 
As database semantics do not natively support \emph{keyless joins} that require similarity-based indexing, joining arbitrary catalogs remains heavily manual---even large companies rely on vendors to categorize listings, which results in duplicate listings.\footnote{https://sell.amazon.com/sell.html}
No out-of-the-box query interface allows users to surface the relatedness between \texttt{A80}, \texttt{A82}, and \texttt{P8} (all \texttt{Asics}, two \texttt{GT-1000}, and two \texttt{blue}), and link these records to the Ratings table with minimal intervention. 

To combat this tedious context enrichment process, we evaluate how to bring recent no-code semantics from ML systems such as Ludwig~\citep{ludwig}, H20.ai~\citep{h20}, and Data Robot~\citep{robot} to context enrichment.
The challenge in developing a no-code context enrichment system is to construct an architecture that is simultaneously:
\begin{enumerate}
    \item \textbf{General}: Applicable to a wide variety of tasks and domains.
    %\item \textbf{Query-time Scalability}: Efficiently queries new data.
    \item \textbf{Extensibile}: Customizable for domain or downstream needs.
    \item \textbf{Low Effort}: Usable with minimal configuration.
\end{enumerate}

We propose \sys, a no-code context enrichment framework that provides these three functionalities.
\sys's architecture generalizes across a variety of tasks, and is easily customized using a high-level configuration file.
As input, users provide a base data source, an auxiliary data source, and a set of examples of related records across the sources (Figure~\ref{fig:overview}).
For each record in the base data source, \sys returns related records from the auxiliary data source as characterized by the examples, which can be post-processed for downstream tasks (e.g., concatenated or averaged).

\sys's key insight is to simplify context enrichment by abstracting an interface that performs a new class of join: a \textit{learned keyless join} that operates over record-level similarity. 
Just as traditional database joins provide an abstraction layer for combining structured data sources given KFK relationships, we propose formalizing keyless joins as an abstraction layer for context enrichment.

\sys implements a keyless join abstraction layer by constructing an index populated with task-specific embeddings.
Drawing inspiration from successes in applying Transformers~\citep{transformers,bert} to structured datasets~\citep{tabert,neuraldb}, we rely on Transformers as building blocks for embedding generation. 
%Unlike KFK joins that operate at the schema-level, keyless joins must consider record-level similarities to identify if records from different tables are related---not the similarities of specific column values to identify exact matches.
%Advances in Transformer-based encoders applied to structured datasets can power a general method to identify contextually similar records. 
We present a three-step system architecture that enables index construction via Transformer-based embeddings: preprocessing, representation learning, and joining.

%The resulting research challenge is in exploring the design space to determine the system architecture and operators required to enable context enrichment via keyless joins across domains spanning recommendation, search, question answering, and data integration.

\eat{
%While modern no-code ML systems support downstream workloads, they treat context enrichment as a user-performed feature engineering step~\cite{ludwig, overton}. 
%When developing such ML systems for structured data, we realized that this procedure for context enrichment can be simplified via the introduction of a new class of join: a \emph{keyless} join that performs a join based on data point similarity. 

%When developing such ML systems for structured data, we realized that the need for context enrichment is pervasive across a wide spectrum of downstream applications including recommendation (as above), search, question answering, and data integration. 
%However, each vertical constructs an independent, domain-specific solution for these tasks, which is time-consuming and repetitive.
%While modern no-code ML systems support the end-application, they treat this context enrichment as a user-performed feature engineering step~\citep{ludwig, overton}.
%As a result, enrichment remains tedious, requiring domain-specific techniques.
%Consequently, in this paper, we evaluate if is it possible to develop a scalable and general context enrichment system that can be applied across all of these workloads with no code modifications.
}

%A system that implements a scalable and general keyless join enrichment layer must address three design decisions. 


%In this paper, we propose \sys, a no-code context enrichment framework that implements these three elements.
%As input to \sys's default architecture, users provide a base data source, an auxiliary data source, and a set of examples of related records across the two sources (Figure~\ref{fig:overview}).
%For each record in the base data source, \sys returns the most related records from the auxiliary data source.
%These outputs can then be post-processed for downstream tasks (e.g., concatenated or averaged).
%We introduce both \sys's high level architecture and the implementation of \sys's default operator configuration to demonstrate how a single system can generalize to all of our target workloads by changing a high-level configuration file. 
%workloads spanning recommendation (as in Figure~\ref{fig:example}), search, entity matching, fuzzy joins, and question answering by changing a high-level configuration file. 

\eat{
\begin{figure}
\includegraphics[width=\columnwidth]{figures/Categorization.pdf}
\caption{}
\label{fig:categories}
\vspace{-1em}
\end{figure}
}


\eat{
%The key insight behind \sys is that new Transformer-based methods for embedding generation~\citep{transformers,bert} can serve as the building blocks for a no-code keyless join enrichment layer. 
%Keyless joins must operate at the record-level, unlike KFK joins that operate at the schema-level. 
%As a result, \sys must consider record-level similarities to identify if records from different tables are related---rather than considering the similarities of specific column values to identify exact matches.
%By building off recent advances in Transformer-based encoders applied to records in structured datasets, we provide a general method to identify contextually similar entities. 
%At a high-level, \sys provides an interface for keyless joins by constructing an index that is populated with task-specific embeddings.
%To enable this functionality, we propose a three-step system architecture: preprocessing, representation learning, and joining.


%that we can simplify context enrichment by defining and and abstracting this new class of join: a \emph{keyless} join that performs a join based on record similarity. 
%Just as traditional database joins provide an abstraction layer for combining structured data sources given KFK relationships, we propose keyless joins as an abstraction layer for context enrichment (Figure~\ref{fig:categories}).


%In this paper, we evaluate how to develop a general context enrichment system that requires no code modification.  
%We show how abstracting keyless joins as a fundamental primitive for context enrichment can help achieve this goal.
%close the loop for developing simple, no-code ML pipelines over structured data. 
%The resulting research challenge is in exploring the design space to determine the architecture and abstractions required to enable general keyless joins. 
%In response, we propose \sys, a no-code context enrichment framework.


%As input to \sys's default architecture, users simply provide a base data source, an auxiliary data source, and a small set of examples of related records across the two sources (Figure~\ref{fig:overview}.
%For each record in the base data source, \sys then returns the most related records from the auxiliary data source.
%These outputs can then be processed for use in a downstream task (e.g., concatenated or averaged).

%We develop \sys as a no-code framework for context enrichment to demonstrate that keyless joins enable generalization to workloads spanning search, entity matching, fuzzy joins, question answering, and recommendation (as in Figure~\ref{fig:example}) by only changing a high-level configuration file. 
%When using \sys's default architecture and operators, users simply provide a base data source, an auxiliary data source, and a small set of examples of related records across the two sources.
%For each record in the base data source, \sys then returns the most related records from the auxiliary data source.
%These outputs can then be processed for use in a downstream task (e.g., concatenated or averaged).

%The key insight behind \sys is that new Transformer-based methods for embedding generation~\citep{transformers,bert} can serve as the building blocks for a no-code keyless join enrichment layer. 
%Keyless joins must operate at the record-level, unlike KFK joins that operate at the schema-level. 
%As a result, \sys must consider record-level similarities to identify if records from different tables are related---rather than considering the similarities of specific column values to identify exact matches.
%By building off recent advances in Transformer-based encoders applied to records in structured datasets, we provide a general method to identify contextually similar entities. 
%At a high-level, \sys provides an interface for keyless joins by constructing an index that is populated with task-specific embeddings.
%To enable this functionality, we propose a three-step system architecture: preprocessing, representation learning, and joining.
}

%We identify three elements that a system must provide to implement a general keyless join enrichment layer.
%First, the system must represent records from different data sources in a comparable format regardless of schema.
%Second, these representations must be automatically tuned to identify contextually similar records as defined by a downstream application. 
%Finally, similar records must be quickly retrieved using the tuned representations. 


\minihead{Preprocessing} \sys transforms records from different data sources to a common representation, which allows us to apply the same methods across tasks to enable generality (1). 
%We answer: how can we represent records from different sources in a comparable format?
Although classic means of representing structured data often focused on integer encoding, Transformer-based encoders such as BERT and GPT have demonstrated success across data types including structured data~\citep{tabert,neuraldb}.
Thus, by default, \sys represents each record as a natural language sentence for input to a Transformer-based encoder, which we optionally pretrain using self-supervision.
%Building off this recent success, by default, \sys represents each record as a natural language sentence consisting of the column names and values in key-value format for input to a Transformer-based encoder.
We demonstrate that depending on the data vocabulary, encoder pretraining to bootstrap the pipeline with domain knowledge can increase recall of retrieved relevant records by up to \red{24\%}. 

\begin{figure}
\includegraphics[width=\columnwidth]{figures/overview.pdf}
\caption{\sys's interface for context enrichment. \sys retrieves related auxiliary records for each base record.}
\label{fig:overview}
\vspace{-1em}
\end{figure}

\minihead{Representation Learning} \sys automatically tunes the representations from the first step to identify contextually similar records as defined by a downstream application to improve ease-of-use (3).
Learning this representation is task-dependent: we show that a natural first approach of using pretrained Transformer-based embeddings (e.g., BERT) with no fine-tuning performs up to three orders of magnitude worse than a fine-tuned approach, often returning less than \red{10\%} of relevant records.  
%orders of magnitude worse than standard information retrieval methods (i.e., BM25); learning a representation to reflect relatedness is task-dependent.
Domain-specific pretraining in the first step can increase recall by over \red{30\%}, but this is still insufficient in isolation.
Thus, \sys relies on supervised examples of related records and a contrastive triplet loss~\citep{tripletloss} to learn a representation that encourages similar records to be close while pushing away dissimilar records in the induced embedding space. 
We evaluate how many labeled examples are required to match the performance of using all provided examples, and find that at times, \red{1\%} of the labels is sufficient, and that operators for automatic hard negative sampling improve performance by up to \red{25\%} recall.
%\sys provides negative sampling utilities to sample unrelated records, should a user only provide examples of related records.

\minihead{Joining} \sys quickly retrieves related records using the tuned representations to perform the keyless join.
%We answer: how can we quickly compare and identify related records?
A na\"ive means of identifying similar records would require exhaustive pairwise comparison of potentially joinable records.
However, this procedure scales quadratically with the number of considered records. 
While similarity-based join techniques as in data blocking~\citep{blocking} also aim to identify related records for a given base record, we show that the best method with respect to recall is domain-specific.
As we learned an embedding space to capture record similarity in the second step, \sys can instead populate an index with the learned embeddings, and use optimized maximum inner product search (MIPS) to identify the nearest neighbors of a given record.
This procedure allows \sys to capture one-to-one and one-to-many join semantics across a variety of downstream applications with low query-time overhead.
We demonstrate that \sys meets or exceeds the performance of seven similarity-based join baselines including BM25~\citep{bm25}, jaccard-similarity-based joins, and Levenshtein distance-based joins with respect to recall and query runtime.   

%We answer: what architecture and supervision is required to learn a representation where contextually similar records are close together in embedding space?
%As previously noted, we rely on Transformer-based encoders.
%While a na\"ive encoder architecture may train independent encoders for each data source, we find that for our context enrichment tasks, using a single encoder performs best.
%With respect to supervision, we demonstrate the leveraging pretrained BERT embeddings with no supervised fine-tuning performs orders of magnitude worse than standard information retrieval methods (i.e., BM25); learning a representation to reflect relatedness is task-dependent.
%While domain-specific pretraining in the preprocessing step helps bridge this gap, it is still insufficient in isolation.
%Thus, \sys instead uses supervised examples of related and unrelated records in this step.
%By default, \sys uses a contrastive triplet loss~\citep{tripletloss} to learn a representation; the triplet loss encourages similar records to be close and pushes away dissimilar records under the induced embedding space. 
%\sys provides negative sampling utilities to sample unrelated records, should a user only provide examples of related records.

%In the joining step, we perform the keyless join.
%We answer: how can we quickly compare and identify related records?
%A classic means of identifying similar records would require exhaustive comparison between all pairs of potentially joinable records (either the entire dataset, or a set of candidate records or a data block)~\citep{}.
%However, this procedure scales quadratically with the number of records considered. 
%As we are working in embedding space that has been tuned to capture record similarity, \sys can instead push the similarity check to the final pipeline step. 
%\sys populates an index with the learned embeddings, and uses optimized maximum inner product search (MIPS) to identify the nearest neighbors of a given record in the embedding space.

Although conventional wisdom in data management often says to rely on domain-specific pipelines for context enrichment, we introduce no-code ML semantics to context enrichment and empirically show how a single system can generalize to heterogeneous downstream tasks, providing extensibility (2).
We report on our experiences in deploying \sys across five tasks: fuzzy joining, entity matching, question answering, search, and recommendation.
We demonstrate that \sys generalizes to each, requires as little as a single line configuration change, and extends to downstream similarity-based analyses for search, entity matching, and recommendation as in Figure~\ref{fig:example}. 

In summary, we present the following contributions in this paper:

\begin{itemize}
    \setlength\itemsep{.75em}
    \item We propose keyless joins as a new abstraction layer for context enrichment. To our knowledge, this is the first work to abstract and generalize similarity-based tasks across data integration, natural language processing, search, and recommendation as a data management problem.
    \item We design and develop \sys, the first no-code framework for context enrichment that implements keyless joins.
    \item We empirically demonstrate that \sys generalizes to five workloads by meeting or exceeding the recall of baselines with fewer than 5 lines of configuration changes, and evaluate the design of \sys's default architecture.
\end{itemize}












































%\red{[similarity search + downstream; too short and redundant with previous?]} \\
%Finally, given the fine-tuned model, \sys identifies data points that should be joined using an optimized routine for maximum inner product search~\citep{faiss}.
%By pushing the similarity check to the final step of the architecture, \sys eliminates the costly quadratic comparison needed by classic systems~\citep{}. 
%The outputs of \sys can either be directly used by a downstream task with similar records concatenated or averaged, or the representation in the original data sources can be directly used.

\eat{
%Methods for automated machine learning (AML) that integrate ML and data processing have become increasingly prevalent~\citep{seehamlet} as machine learning (ML) now powers a wide variety of data-driven applications such as search, ranking, and query answering~\citep{randomstuff}.
%These methods typically assume that data is obtained from a single source (e.g., a single database table, or an collection of text records), or that there exists a join key that connects multiple normalized data sources to one another either directly or via simple preprocessing (e.g., aggregation or interpolation)~\citep{hamlet,arda}. 
%However, when a single data source is not sufficiently informative for a given task, the sources that users may wish to augment their data with provide different, yet overlapping views of the same underlying information, where no explicit join key can be used to unite the data sources. 
}
\eat{
Rising data volumes in conjunction with human processing and labeling efforts have resulted in unprecedented amounts of task-specific, high-fidelity\eat{supervised and unsupervised} training data.
This data has enabled machine learning (ML) systems to power a wide array of critical applications spanning search, recommendation, and question answering~\citep{ml1, ml2, ml3}. 
However, as our demand for ML-powered applications grows, it becomes infeasible to develop and process task-specific datasets from scratch~\citep{snorkel,crossmodal}.
As a result, a single dataset may not be sufficient in isolation for a given task~\citep{arda}.
We must instead leverage a combination of heterogeneous, potentially overlapping datasets that have been generated and stored for other uses~\citep{lakehouse,gpt2}. For instance, consider the following scenario:
}
\eat{
%Great training data has enabled ML to power a huge array of cool things.  % maybe instead make a sell here about attention and training data/processing not meeting pace with it %todo: establigh the heterogeneity and overlappingness of these datasets
%As the space grows, we find that oftentimes a single dataset is not used in isolation---either due to collecting data to improve improve model performance by leveraging additional information to enrich the input training data or as a result of an increasing ecosystem of collected data that can be leveraged.  
}
\eat{
\vspace{5pt}
\emph{An e-commerce company operates a store that sources products from several vendors. Each vendor provides a unique product catalog, where catalogs may overlap and evolve based on supplier inventory.  
An ML engineer at this company wishes to display the most relevant shopping results for a user given their purchase history.
Catalogs have unique product representations (i.e., schema) ranging from free-form text to highly-structured tabular product descriptions. 
While the company has labeled a small number of product matches across the different catalogs, no global product identifier exists as a unifying join key.
Thus, the engineer must develop a system to join products across the catalogs, and display the most relevant products for a user's query.}\vspace{5pt}

We refer to the process of joining datasets that are heterogeneous yet overlapping in information as \emph{context enrichment}, where multiple auxiliary data sources (e.g., product catalogs) are combined to augment, or enrich, a base data source (e.g., the e-commerce company's global product list).
Although similar to existing problems in data augmentation~\citep{dataaug} or management~\citep{arda,hamlet,hamletpp,tableunion}, existing methods assume that practitioners operate over either a single data source, or can learn explicit join keys to unite multiple data sources.
In contrast, context enrichment is tailored to the rising class of data-intensive workloads that manage multiple data sources without such join keys, as present in data lakes~\citep{lakehouse}.
These workloads span both classic data management, (e.g., data integration, information retrieval, relational data augmentation, fuzzy joining) and machine learning (e.g., entity disambiguation, question answering, multi-hop question answering). 
As our data ecosystems and need for data-driven applications continue to grow, we require scalable systems for context enrichment to power the next generation of data analytics and ML platforms. 
}

\eat{
In response, we introduce the \enrich operator, a declarative relational operator that performs context enrichment.
Given a base and auxiliary data sources, the \enrich operator identifies data points in the auxiliary sources that share context with the base data source, and returns the joined result. 
Rather than relying on information solely present in each column to join datasets, \enrich instead learns a representation for each data point such that their distance in the induced embedding space reflects their similarity to one another \reword{for use in a downstream workload}. 
To enable scalable, generalizable context enrichment, the \enrich operator overcomes two key bottlenecks: human attention and computational resources. 
}
\eat{
First, as human attention is fundamentally limited compared to computational and storage capacity~\citep{mbcidr}, a system for general context enrichment cannot rely on excessive human supervision and processing for \emph{each} join that must be performed.
Typical automated means for identifying candidate matches across datasets require large amounts of supervised training data (i.e., examples of matching and not matching data points) to train an ML model~\citep{deepmatcher}.
The \enrich operator instead leverages recent advances in self-supervised learning and transformer models in natural language processing to alleviate this need.  
We first represent each data source's data points as natural language sentences, which enables us to represent heterogeneous textual and numeric data sources with a shared vocabulary.
We then automatically identify similar data points using unsupervised ranking from information retrieval (i.e., BM25), and use these data points to perform pre-training via masked language modeling to bootstrap a transformer model.
This pre-training step enables us to use a small subset of labeled examples to fine-tune our data representation.
}
\eat{
Second, as data volumes rapidly grow, a system for context enrichment must scale with an increasing number of large, heterogeneous datasets.
A na\"ive yet classic means of identifying similar data points would require exhaustive comparison between all pairs of potentially joinable data points (either the entire dataset, or a set of candidate data points or a data block).
However, this procedure scales quadratically with the number of data points considered. 
The \enrich operator instead scales to large data volumes by learning a representation over which maximum inner product search identifies related records across heterogeneous data sources.
We use a small subset of labeled data points to fine-tune the representation learned from the pre-training step using a contrastive loss~\citep{tripletloss}, so similar data points are close to one another in the embedding space induced by the representation.
Given this representation, we can identify data points that should be joined using an optimized routine for maximum inner product search~\citep{faiss}.
}
\eat{
%The \enrich operator addresses the scaling challenges across people, machine, and application as follows. 
%To realize this opportunity, a system for context enrichment must overcome three \reword{bottlenecks} in uniting heterogeneous datasets for an end-task: human attention, computational resources, and \reword{diversity of target application.} 
%First, as human attention is fundamentally limited compared to computational and storage capacity~\citep{mbcidr}, a system for context enrichment cannot rely on excessive human supervision for each join.
%Second, as data volumes rapidly grow, a system for context enrichment must scale with increasing number of heterogeneous datasets and their size.
%Finally, as target applications diversify, a system for context enrichment must provide a generalizable architecture and interface amenable for reuse.


%First, the \enrich operator reduces the need for human supervision by leveraging recent advances in self-supervised learning and attention in natural language processing. 
%We instead first represent each data point as a natural language sentence, and automatically identify candidate similar data points using unsupervised ranking from information retrieval (i.e., BM25). 
%We use these candidate data points to perform pre-training via masked language modeling to bootstrap a transformer model.
%This pre-training step enables us to then use a small subset of labeled examples to fine-tune our data representation.

%Second, the \enrich operator scales to large data volumes by learning a representation over which maximum inner product search identifies related records across heterogeneous data sources. 
%A na\"ive yet classic means of identifying similar data points would require exhaustive comparison between all pairs of potentially joinable data points (either the entire dataset, or set of candidate data points or a data block).
%However, this procedure scales quadratically with the number of data points considered. 
%Thus, we instead use the small subset of labeled data points to fine-tune the learned representation above using a contrastive loss~\citep{tripletloss}, where similar data points are close to one another.
%Given this representation, we can identify data points that should be joined using an optimized routine for maximum inner product search~\citep{faiss}.
}
\eat{
% We refer to this procedure as context enrichment, where multiple auxiliary data sources are combined to augment, or enrich, a base table.
%Context enrichment differs from more traditional means of data augmentation as they either operate over a  a single data source/table, or assume the presence of join keys to unite multiple data sources/tables together.
% In particular, these techniques do not address the case where heterogeneous data sources cannot be combined with an explicit join key, but instead consists of overlapping views of related information. 

% Unlike the canonical database join that links multiple data sources, where explicit join keys unite and augment data sources, context enrichment relies on  information that unites these tables are  


%Existing methods that integrate ML and data processing typically ignore this challenge, or assume 




% ML powers a bunch of stuff, so AML that integrates ML and data processing has become increasingly prevalent. 
% This work either only deals with single tables, or assumes the presence of a join key. 
% For example ....
% 


Different types of joins
\begin{enumerate}
    \item Joining because mentions are in different namespaces, but same things -- record linkage and dedupe
    \item Joining because you have different entities that have overlap in content or context -- retrieval, predictive, etc
\end{enumerate}


Traditional DB focuses on the first. However, the latter is also huge. But if you don't have primary-key/foreign-key, unfortunately, there is very limited tooling to join things together. 
 
This is a new type of joins that relies on embeddings. 

It appears in question answering, information retrieval, entity disambiguation, etc.


We present BLAH, a new operator that represents these embedding-based joins, and provides a unified interface for enabling such queries. 

bm25 is index creation for the join (can be anything you want; tfidf)

how to connect with traditional join with this 

join by random doesn't work. different columns for each, doesn't work. 
}

%Much of machine learning's success with unstructured data is a result of our ability to extract information relevant to a downstream task from large volumes of \emph{context-rich training data.} 
%For instance, a single image contains most of the context required to perform an image classification task---large supervised image datasets and efficient deep learning architectures to extract this context revolutionized computer vision~\citep{alexnet}. 
%Similarly, the ability to integrate and leverage context from unsupervised textual data sources via transformers~\citep{transformers} revolutionized natural language processing~\citep{bert,gpt2}. 
%On the other hand, structured data suffers from context being scattered across numerous, nonuniform datasets.
%\red{[Structured data's design --> fragmentation; we must overcome]}
%Structured datasets are typically in a form optimized for efficient querying and manipulation---e.g., in normalized form specialized to a single set of business needs. 
%Thus, context for a single data point is split across multiple data sources, which is at odds with ML models that thrive given an abundance of context-rich information.

%While classic solutions for context enrichment often do not apply, newer ML-based methods rely on humans for supervision and to develop custom systems for each enrichment task. 
%The classic data management approach is to denormalize datasets using primary key-foreign key (KFK) joins.
%However, for an increasing number of tasks, as the one above, KFK dependencies are not present.
%Practitioners may alternatively turn to ML-based approaches to join entities across datasets, but this requires large amounts of hand-labeled training data, which is often time-consuming and arduous to collect for each enrichment task~\citep{snorkel}. 
%Finally, even if a team is able to develop a method for effective context enrichment for a given task, they do so in an end-to-end manner~\citep{deepmatcher}.
%As a result, they start from scratch for each new enrichment domain---entity matching (as in the example), information retrieval, fuzzy joins, and even question answering and entity disambiguation.
%The lack of a unified approach to context enrichment leads to redundant solutions that waste human time: the ML engineer in the above example is unlikely to interface directly with the advertising team at the same company, who may encounter similar challenges. 
%\sys instead learns a representation for each data point such that their distance in the induced embedding space reflects their similarity to one another. 
%\sys proceeds in a three-step architecture: pre-training, fine-tuning, joining.





%The outputs of \sys can be configured to be directly used by a downstream task with related data points concatenated or averaged.

%utilizes optimized maximum inner product search (MIPS) to identify the nearest neighbors of a given record in the embedding space.
%By pushing the similarity check to the final step of the architecture, \sys eliminates the costly quadratic comparison needed by classic systems~\citep{}. 
%We show how the outputs of \sys can be used for general similarity-based analysis as in the e-commerce example. 



%The resulting research challenge when developing \sys is determining the architecture and abstractions required to enable no-code keyless joins. 
%In response, we introduce both \sys's high level architecture, as well as the implementation of \sys's default operator configuration. 

%We propose a three-step system architecture: preprocessing, representation learning, and joining.
%First we must process the input datasets of varying schema such that we can apply a general architecture — while the input schema is known, they are heterogenous.

%Performing a keyless join requires computing record similarity for a downstream task, and performing the join based on the computed similarity. 
%In response, we propose a three-step architecture when designing \sys: preprocessing, representation learning, and joining.  
%The goal of the first step is to learn a data representation such that similarity in the induced embedding space is proportional to the data points' relatedness, or similarity for the downstream task. 
%Given the learned representation, the joining step identifies and returns data points that are most similar to one another. 
%In effect, \sys provides an interface for keyless joins by constructing an index that is populated with task-specific embeddings.
%Developing the operators necessary to enable this two-step architecture requires answering three key technical questions. 

%First, how can we represent data points from different sources in a comparable format for the first step? 
%Although classic means of representing structured data has often remained limited to integer encoding, advances in pre-trained transformer-based encoders such as BERT have demonstrated success across many data types, including structured data~\citep{}.
%We \sys relies on these encoders to generate embeddings for each data point by forming sentences using each key-value pair in a data source. 
%While na\"ive approach to leveraging these encoders may seek to train independent encoders for each data source, we find that for our context enrichment tasks, using a single encoding source performs best in practice. 
%Thus, \sys's default configuration is a single BERT encoder, and we provide configuration options to use either multiple encoder modules as part of the first step. 
%We show that using a single encoder performs up to \red{XXX} better. 

%Second, what supervision is required to learn a representation where similar data points are close together in embedding space?
%Learning a representation to reflect relatedness is task dependent.
%As such, \sys requires a small amount of supervised examples of data points that are related and unrelated to a subset of query data points.
%\sys provides negative sampling utilities to sample unrelated data points, should a user be incapable of providing such supervision.
%By default, \sys uses a contrastive triplet loss~\citep{tripletloss} to learn a representation; the triplet loss encourages similar points to be close and pushes away dissimilar points under the induced embedding space. 
%While the loss function used is a configurable parameter, we find that the triplet loss performs well across our tasks, and is the default operator. 
%In addition, for tasks that may benefit from pre-training the encoder module, we provide operators that can leverage either fully supervised or self supervised methods to bootstrap representation learning. 
%We show that self-supervised pre-training can improve the performance of tasks by up to \red{XXX.} 


%Finally, how can we quickly compare data points to identify those that are related to one another in the second step?
%A na\"ive yet classic means of identifying similar data points would require exhaustive comparison between all pairs of potentially joinable data points (either the entire dataset, or a set of candidate data points or a data block).
%However, this procedure scales quadratically with the number of data points considered. 
%As we are working in embedding space that has been tuned to capture data point similarity, \sys instead utilizes optimized maximum inner product search (MIPS) to identify the nearest neighbors of a given data point in the embedding space.
%By pushing the similarity check to the final step of the architecture, \sys eliminates the costly quadratic comparison needed by classic systems~\citep{}. 
%The outputs of \sys can be configured to be directly used by a downstream task with related data points concatenated or averaged.
%We show how the outputs of \sys can be used for general similarity-based analysis as in the e-commerce example. 


%We report on our experiences in applying \sys across \reword{five} different domains. 
%We demonstrate how no-code context enrichment allows users to go from zero-to-one on a variety of target applications by abstracting away previously tedious procedures. In summary, we present the following contributions in this paper:


%Traditional data-intensive workloads that perform context enrichment as an inherent primitive are developed in isolation from one another, and fail to capitalize on advances made in each domain. 
%By developing a unified framework for context enrichment with limited supervision, we provide a system for solving for such tasks \reword{easier than before, with less supervision.} 
\eat{\begin{itemize}
    \setlength\itemsep{.75em}
    \item We propose keyless joins as a new abstraction layer to enable no-code context enrichment.
    \item We design and develop \sys, the first no-code framework that implements the keyless join abstraction layer for context enrichment.
    \item We evaluate \sys's default configuration, and demonstrate that \sys generalizes \reword{five} workloads across domains spanning data systems and natural language processing via a high-level configuration file.
\end{itemize}}


\eat{
%\red{[What's wrong with context enrichment in ML?]} \\
Practitioners may alternatively turn to ML-based approaches to join entities across datasets, but this requires large amounts of hand-labeled training data, which is often time-consuming and arduous to collect for each enrichment task~\citep{snorkel}. 
Even if a team is able to develop a method for effective context enrichment for a given task, they do so in an end-to-end manner~\citep{deepmatcher}.
As a result, they start from scratch for each new enrichment domain---entity matching (as in the example), information retrieval, fuzzy joins, and even question answering and entity disambiguation.
The lack of a unified approach leads to redundant solutions that waste human time: the ML engineer in the above example is unlikely to interface directly with the advertising team at the same company, who may encounter similar challenges. 
Context enrichment requires a generic, unifying operation that processes structured data for ML workloads.


%\red{[Main Idea]} \\
Our key insight to tackle context enrichment---and the need for a generic operator to perform keyless joins---is to leverage the context that we wish to unite to learn a common data representation across tables where data points' distance in the induced embedding space reflects their similarity to one another. 
We can then holistically evaluate and cluster related data points to join datasets rather than relying on information present in a small set of KFK dependencies.




%\red{[our proposal]} \\
To realize this, we propose \sys, a new context enrichment system  that generalizes and optimizes for keyless joins.
Given a base and auxiliary data sources, \sys identifies data points in the auxiliary sources that share context with the base data source, and returns the joined result. 
Just as databases created an abstraction layer for querying structured data, \sys provides an abstraction layer for context enrichment for downstream ML tasks. 
\sys consists of two components.
First, \sys learns a common data representation for the data sources. For generalizability, \sys must perform this step while reducing the amount of training data required compared to learning this representation from scratch.
Second, \sys identifies data points across the data sources that share context with one another.
For scalability, \sys must perform this step without without comparing all possible data points to see if they are a match. 
%\sys provides a \emph{generalizable architecture} that leverages recent advances in self-supervision in natural language processing to \emph{reduce human supervision} by up to \red{XXX} across \red{YYY} tasks.  using recent advances in self-supervision in natural language processing


%\red{[pre-training/fine-tuning to reduce supervision needed]} \\
In the first step, \sys performs self-supervised masked language modeling to pre-train its embedding using context from each data source, followed by a fine-tuning phase to learn the embedding. 
%As human attention is fundamentally limited compared to computational and storage capacity~\citep{mbcidr}, a system for general context enrichment cannot rely on excessive human supervision and processing for \emph{each} join that must be performed.
Typical automated means for identifying candidate matches across datasets require large amounts of supervised training data (i.e., examples of matching and not matching data points) to train an ML model~\citep{deepmatcher}.
\sys instead first represents each data source's data points as natural language sentences, which enables us to represent heterogeneous textual and numeric data sources with a shared vocabulary.
\sys then automatically identifies similar data points using unsupervised ranking from information retrieval (i.e., BM25), and uses these data points to perform pre-training via masked language modeling to bootstrap the parameters of a transformer model.
Finally, \sys fine-tunes the pre-trained transformer model given a set of labeled examples to learn a data representation where similar items are close in the induced embedding space.

%\red{[similarity search + downstream; scales]}
In the second step, \sys identifies data points that should be joined using an optimized routine for maximum inner product search~\citep{faiss} (MIPS).
A na\"ive yet classic means of identifying similar data points would require exhaustive comparison between all pairs of potentially joinable data points (either the entire dataset, or a set of candidate data points or a data block).
However, this procedure scales quadratically with the number of data points considered. 
The \sys instead scales to large data volumes by learning a representation over which maximum inner product search identifies related records across heterogeneous data sources.
We use a small subset of labeled data points to fine-tune a task-specific representation learned from the pre-training step using a contrastive loss~\citep{tripletloss}, so similar data points are close to one another in the embedding space induced by the representation, and can be retrieved via MIPS.
By pushing the similarity check to the final step of the architecture, \sys eliminates the costly quadratic comparison needed by classic systems~\citep{}. 
The outputs of \sys can either be directly used by a downstream task with similar records concatenated or averaged, or the representation in the original data sources can be directly used.

%\red{[results]}
\sys provides a flexible interface for a variety of target applications by providing a generalizable architecture and interface amenable for reuse. 
Context enrichment is a key primitive in several seemingly unrelated tasks spanning: entity matching, entity disambiguation, information retrieval, relational data augmentation, and question answering.
%Traditional data-intensive workloads that perform context enrichment as an inherent primitive are developed in isolation from one another, and fail to capitalize on advances made in each domain. 
By developing a unified framework for context enrichment with limited supervision, we provide a system for solving for such tasks \reword{easier than before, with less supervision.} 
In summary, we present the following contributions:
\begin{itemize}
    \setlength\itemsep{.75em}
    \item We introduce \sys, a system that performs context enrichment given two or more datasets.
    \item We demonstrate how \sys generalizes workloads across data systems and natural language processing to provide a unified interface for tasks relating multiple data sources.
    \item We empirically show that \sys reduces the number of training examples needed for downstream tasks by up to \red{XXX} to maintain performance.
\end{itemize}
}





\eat{



\minihead{Results} We report Retrieval@1, Retrieval@10, and MRR@10 of IMDb and IMDb-hard in Table~\ref{table:retrieval}, computed with the post-processing module described in Section~\ref{case:IR}. 
\sys outperforms BM25, and only drops at most 4 points (in Retrieval@1) in the IMDb versus IMDb-hard tasks, while BM25 degrades by over 20 points. 


\minihead{Results} We report our F1 score on the test set compared to several baselines in Table~\ref{table:dm_all}.
\sys@1 refers to retrieving the top match, and \sys@best refers to retrieving the number of \records that provides the best F1 score, set via validation. 

The first three results columns reflect the numbers reported from the four deep-learning-based solutions from the deepmatcher package, where DM$_\text{SIF}$ refers to their simple aggregate function model,
DM$_\text{RNN}$ refers to their sequence-aware bidirectional RNN model,
DM$_\text{att}$ refers to their sequence alignment model that uses decomposable attention, and DM$_\text{hyb}$ refers to their hybrid sequence-aware model with decomposable attention ~\citep{deepmatcher}, each of which is customized for EM.
DM$_\text{SIF}$ and DM$_\text{RNN}$ are comparable to the previous standard deep learning method for EM, DeepER~\citep{deeper}. 
The fourth results column reflects the numbers reported by the current state-of-the-art deep-learning-based system, Ditto~\citep{ditto}.
Ditto achieves these results using pre-trained language models, with custom optimizations that allow users to tag input text spans, perform sentence summarization for long records, and apply data augmentation to find hard examples.

Without any such optimizations, \sys@best provides results within 2 F1 points of Ditto in 3 tasks, outperforms at least one other custom deep-learning-based solution on 10 of the 13 tasks, and outperforms all but Ditto on 5 tasks  (underperforming compared to DM$_\text{hyb}$ by less than 1 F1 point on 4 others). 

As an added benefit of our MIPS-based approach, upon inspection of our returned results, we identified mislabeled examples in the training dataset. 
For instance, in the abt-buy dataset, we found a cluster of records in the specified right table that contain the same column values: rtable-id 799, 800, 801. 
However, ltable-id value 720 erroneously lists rtable-id 800 as not a match in the train set, when rtable-id 799 is a match in the test set.


\minihead{Results} We report our results in Table~\ref{table:retrieval} after training once over 10M of the 397M training examples, as training the full dataset for even one epoch requires over a week with our hardware. 
Notably, we obtain MRR@10 of 0.231 after just 250K training examples---which is just  0.07\% of the provided training dataset.
We report the official BM25 baseline solution, which we outperform by 1.49$\times$.
Our results are on par with K-NRM, a kernel based neural model, which achieves a dev set performance of 0.218~\cite{marcobert}, and slightly below the state-of-the-art from the time, IRNet, with 0.278 MRR@10~\citep{irnet}. 
For comparison, the first state-of-the-art BERT-based model uses BERT$_\text{large}$ to achieve MRR@10 of 0.365 after training on 12.8M examples~\cite{bertthing}, and current state-of-the-art achieves 0.439~\cite{rocketQA}. 
With further development and configuration of \sys \encoder aggregation method, \sys can implement ColBERT~\cite{colbert}, a previous state-of-the-art method that achieves 0.384 MRR@10 on the MS MARCO document ranking task, passage ranking's sister task that operates on larger input passages (i.e., "documents"). 


\minihead{Results} We report Retrieval@1, Retrieval@10, and MRR@10 of the modified SQuAD workload Table~\ref{table:retrieval}. In each case, we outperform BM25, where the gap between the two methods grows from  as \sys retrieves more records. 


\minihead{Results} We report Retrieval@1, Retrieval@10, and MRR@10 of the IMDb-wiki-join application Table~\ref{table:retrieval}. 
\sys significantly outperforms BM25 when retrieving the top \record. 
BM25 closes the gap when considering retrieval@10, but still lags far in MRR@10. 

In the IMDb-wiki-rec application, we report the mean squared error (MSE) between the rating estimates and the true rating when aggregating 1, 10, 20, and 30 nearest neighbors. The task is a fairly easy workload for which predicting the average training rating provides a MSE 1.19, and a gradient-boosted decision tree over the joined data returns 0.82 MSE.
We aim to meet or exceed the GBDT's performance. 
Both one- and two-hop approaches improve performance as the number of neighbors increase, until a plateau is reached. 
The two-hop approach attains MSE of 1.69, 0.92, 0.89, and 0.89 for 1, 10, 20, and 30 neighbors, respectively, while the one-hop approach performs better with 1.59, 0.89, 0.86, and 0.85. 
}

==> context enrichment 8/intro.tex <==
\section{Introduction}


Machine learning (ML) systems that extract structural and semantic context from unstructured datasets have revolutionzed domains such as  computer vision~\citep{alexnet} and natural language processing~\citep{bert,gpt2}.
Unfortunately, applying these sytems to structured and semi-structured data repositories that consist of datasets with pre-defined schemas is challenging as their context is often \textit{fragmented}: they frequently scatter information regarding a data record across domain-specific datasets with unique schemas.
For instance, in Figure~\ref{fig:example}B, information regarding \textsc{Asics} shoes is scattered across three catalogs with unique schemas.
These datasets adhere to fixed schemas that are optimized for task-specific querying, and often lack explicit linking keys, such as primary key-foreign key (KFK) relationships.
This constrains users to a single view of an entity that is specialized for a specific business need. 
 
 

\begin{figure}
\includegraphics[width=\columnwidth]{figures/tables.pdf}
\caption{An end-to-end task requiring context enrichment. Predicting the rating of and recommending a new product (\texttt{A82}), requires relating the Asics products (highlighted in dark gray) via a keyless join (top). This process is manual due to data heterogeneity---we aim to automate it (bottom).}
\label{fig:example}
\vspace{-1em}
\end{figure}


Associating these fragmented data contexts is critical in enabling ML-powered applications over such datasets---a process we denote as \emph{context enrichment}---yet is a heavily manual endeavor due to task and dataset heterogeneity.
Engineers develop solutions for context enrichment tailored to their task, such as similarity-based blocking in data integration~\citep{blocking}, retriever models in question answering~\citep{retriever}, or retrieval functions in search~\citep{bm25} (see Section~\ref{sec:applications}). 
Constructing these independent solutions is repetitive, time-consuming, and results in a complicated landscape of overlapping, domain-specific methods.
For instance, consider the scenario depicted in Figure~\ref{fig:example}:


%\vspace{5pt}
\vspace{-7pt}
\emph{\\An e-commerce company has a proprietary product catalog, and aggregates product information from several external vendors to perform market analysis. 
Each vendor uses a unique product catalog, each with unique product representations (i.e., schema) ranging from free-form text to tabular product descriptions; products may overlap and evolve (Figure~\ref{fig:example}B).
Given normalized tables containing user and rating data, an engineer wishes to estimate the rating for a candidate new product (\texttt{A82}) and identify users to recommend the product to (Figure~\ref{fig:example}A).
}
\vspace{5pt}


The engineer must first perform context enrichment by joining information across tables to extract features that capture similarities between the new (\texttt{A82}) and existing (\texttt{A80}, \texttt{P8}) products.
They can then estimate the product rating, and recommend the new product to users based on how they rated related products.

The classic data management approach is to denormalize datasets using KFK joins. 
This fails to solve the problem due to two reasons.
First, not all tables can be joined when relying on only KFK relationships (e.g., there is no KFK relationship between Catalog B and Catalogs A or C). 
Second, even when KFK relationships exist, as between Catalogs A and C (\textsc{\texttt{ITEM}}), relying on only KFK semantics fails to capture the similarity between \texttt{A82} and \texttt{A80}.

Alternatively, the engineer can rely on similarity-based join techniques, as in data blocking~\citep{blocking}, built to avoid exhaustive, pairwise comparison of potentially joinable records.
However, as we show in Section~\ref{subsec:general}, the optimal choice of join operator to maximize recall of relevant records is task-dependent, and may not scale at query time when new records arrive.
The engineer must first note that the \texttt{Description} column in Catalog A relates to the \texttt{Brand} and \texttt{Model} columns in Catalog B and the \texttt{Size}, \texttt{Make}, and \texttt{Color} columns in Catalog C.
They can then select a custom join based on table properties: for matching primarily short, structured data records, they may want to join based on Jaccard similarity, whereas BM25 may be better suited for purely textual records (see Table~\ref{tab:baselines}).
As database semantics do not natively support these \emph{keyless joins} that require similarity-based indexing, joining arbitrary catalogs remains heavily manual---even large companies rely on vendors to categorize listings, which results in duplicate listings.\footnote{https://sell.amazon.com/sell.html}

To counter this manual process, we draw inspiration from recent no-code ML systems such as Ludwig~\citep{ludwig}, H20.ai~\citep{h20}, and Data Robot~\citep{robot} that are rapidly shifting practitioners towards higher-level configuration-based abstractions for developing ML applications.
Despite their success, these systems leave context enrichment as a user-performed data preparation step.\footnote{https://cloud.google.com/automl-tables/docs/prepare}
In this paper, we evaluate how to bring no-code semantics to context enrichment. 

No out-of-the-box query interface surfaces the relatedness between \texttt{A80}, \texttt{A82}, and \texttt{P8} (all \texttt{Asics}, two \texttt{GT-1000}, and two \texttt{blue}), and links these records to the Ratings table with minimal intervention. 
The challenge in developing a no-code context enrichment system to enable this is to construct an architecture that is simultaneously:
\begin{enumerate}
    \item \textbf{General}: Applicable to a wide variety of tasks and domains.
    %\item \textbf{Query-time Scalability}: Efficiently queries new data.
    \item \textbf{Extensibile}: Customizable for domain or downstream needs.
    \item \textbf{Low Effort}: Usable with minimal configuration.
\end{enumerate}

Our key insight to enable such a system is to simplify context enrichment by abstracting an interface for a new class of join: a \textit{learned keyless join} that operates over record-level similarity. 
Just as traditional database joins provide an abstraction layer for combining structured data sources given KFK relationships, we formalize keyless joins as an abstraction layer for context enrichment. 

We then propose \sys: a no-code context enrichment framework that implements a keyless join abstraction layer.
\sys creates an index populated with task-specific embeddings that can be quickly retrieved at query time, and can operate over arbitrary semi-structured datasets with unique but fixed schema.  
To provide generality, \sys relies on Transformers~\citep{transformers} as building blocks for embedding generation, as they have demonstrated success across textual, semi-structured, and structured workloads~\citep{picket,tabert,bert,gpt2,neuraldb}.
To provide extensibility, \sys is composed of a modular, three step architecture with configurable operators. 
To provide ease of use, \sys can be configured using a simple json-based configuration file, and provides a default configuration that works well across five tasks with a single line change per task.

As input, users provide \sys with: \textbf{(1)} a base data source, \textbf{(2)} an auxiliary data source, \textbf{(3)} a set of examples of related records across the sources.
For each record in the base data source, \sys returns related records from the auxiliary data source as characterized by the examples, which can be post-processed for downstream tasks (e.g., concatenated or averaged).
We present \sys's three-step modular architecture that enables index construction via Transformer-based embeddings to facilitate related record retrieval: preprocessing, representation learning, and joining (Figure~\ref{fig:overview}).

\eat{
\begin{enumerate}
    \item A base data source
    \item An auxiliary data source
    \item A set of examples of related records across the sources
\end{enumerate}
}

\minihead{Preprocessing} \sys transforms records from different data sources to a common representation, which allows us to apply the same methods across tasks. 
By default, \sys uses operators that convert each record to a natural language sentence for input to a Transformer-based encoder, which we optionally pretrain using self-supervision.
We demonstrate that depending on the data vocabulary, encoder pretraining to bootstrap the pipeline with domain knowledge can increase recall of relevant records by up to \red{20.5\%}. 

\begin{figure}
\includegraphics[width=\columnwidth]{figures/overview.pdf}
\caption{\sys's interface for context enrichment. \sys retrieves related auxiliary records for each base record.}
\label{fig:overview}
\vspace{-1em}
\end{figure}

\minihead{Representation Learning} \sys tunes the preprocessed representations to identify contextually similar records as defined by supervised examples.
Learning this representation is task-dependent: we show that a natural approach of using pretrained Transformer-based embeddings with no fine-tuning performs up to three orders of magnitude worse than a fine-tuned approach, often returning less than \red{10\%} of relevant records.  
Pretraining in the first step can increase recall by over \red{30\%}, but this is still insufficient.
Thus, \sys relies on operators that use supervised examples of related records and a contrastive triplet loss~\citep{tripletloss} to learn a representation that encourages similar records to be close while pushing away dissimilar records in the induced embedding space. 
We evaluate how many labeled examples \sys needs to match the performance of using all provided examples, and find that at times, \red{1\%} of the labels is sufficient, and that operators for hard negative sampling improve performance by up to \red{30\%} recall, further improving ease of use.

\minihead{Joining} \sys quickly retrieves related records using the tuned representations to perform the keyless join.
 \sys populates an index with the embeddings learned to capture record similarity, and uses optimized maximum inner product search (MIPS) to identify the nearest neighbors of a given record.
This procedure allows \sys to capture one-to-one and one-to-many join semantics across a variety of downstream applications with low query-time overhead.
We demonstrate that \sys meets or exceeds the performance of eight similarity-based join baselines including BM25~\citep{bm25}, Jaccard-similarity-based joins, Levenshtein distance-based joins, and AutoFuzzyJoin~\citep{autofj} with respect to recall and query runtime.   


Although conventional wisdom in data management often says to rely on domain-specific pipelines for context enrichment, we introduce no-code ML semantics to context enrichment and empirically show how a single system can generalize to heterogeneous downstream tasks.
We report on our experiences in deploying \sys across five tasks: fuzzy joining, entity matching, question answering, search, and recommendation.
We demonstrate that \sys generalizes to each, requires as little as a single line configuration change, and extends to downstream similarity-based analyses for search, entity matching, and recommendation as in Figure~\ref{fig:example}. 

In summary, we present the following contributions in this paper:

\begin{itemize}
    \setlength\itemsep{.75em}
    \item We propose keyless joins with a join specification to serve as an abstraction layer for context enrichment. To our knowledge, this is the first work to generalize similarity-based tasks across data integration, natural language processing, search, and recommendation as a data management problem.
    \item We design and develop \sys, the first no-code framework for context enrichment that implements keyless joins, and provides an API for extending and optimizing keyless joins.
    \item We empirically demonstrate that \sys generalizes to five workloads by meeting or exceeding the recall of baselines while using \red{6} or fewer configuration line changes, and evaluate the modular design of \sys's default architecture.
\end{itemize}


==> context enrichment 8/joining.tex <==
\section{Joining}
\label{sec:joining}

In this section, we describe the last step of \sys's pipeline: joining. 
Given the \embeddings output by the trained \encoders, \sys executes the  keyless join by identifying related points across the input datasets, and processing them for downstream use.
\sys indexes the learned \embeddings and queries this index to find candidate related records.
The \texttt{join sizes} determine the number of returned results per query, and we also allow users to configure a similarity threshold for each candidate match.
We now detail the indexing and retrieval procedure, post-processing, and multi-dataset extension.

\minihead{Indexing and Query Retrieval}
Given two records, \sys computes the similarity between their \embeddings to determine if the records are related. 
Many traditional solutions to our motivating applications perform such pairwise checks across all possible pairs either na\"ively or with blocking~\citep{deepmatcher, blocking, bertmarco} to identify related records. 
However, the choice of operator is both domain-specific, and scales quadratically at query time with the size of the input datasets and blocking mechanisms used (see Section~\ref{subsec:general}).
We eliminate the need for pairwise checking by indexing our \embeddings, which are optimized for clustering related records, and rely on efficient libraries for maximum inner product search (MIPS)~\citep{faiss}.

For a \texttt{LEFT} or \texttt{RIGHT OUTER JOIN}, \sys constructs an index over the base ($D_0$) or auxiliary ($D_1$) datasets, respectively. 
\sys then queries the index with each \embedding of the remaining dataset, and returns the \record and \embedding corresponding to the most similar records using a \retriever operator.
For a \texttt{FULL OUTER} or \texttt{INNER JOIN}, \sys may jointly index and query both datasets to identify related entries in either direction. 
By default, \sys only indexes the larger dataset to reduce runtime---an optimization we evaluate in Section~\ref{subsec:micros} that improves query runtime by up to \red{2.81}$\times$.
\sys's default configuration is an \texttt{INNER JOIN}.

%\sys first constructs an index over the \embeddings of the auxiliary dataset $D_1$.
%\sys then queries the constructed index with each \embedding of the base dataset $D_0$, and returns the \record and \embedding corresponding to the most similar records in $D_1$ using a \retriever operator. 
%Users can configure which dataset is to be indexed (is $D_0$), and which to query (is $D_1$) if such semantics are necessary (e.g., in the case of search). 


\minihead{Post-Processing}
The user-provided \texttt{join size} configures the \retriever to return the top-$k$ records with the closest embeddings in the indexed dataset.
\sys additionally supports threshold-based retrieval.
%This enables one-to-one and one-to-many join semantics.
The former is useful for applications such as search, where a downstream task may be to display the top-$k$ search results to a user in sorted order.
The latter is useful for applications where there may not be related records for each record in the base dataset. 
\sys's default \retriever is configured for a 1-to-10 join.

If the task $T$ is not to simply return related records, users can construct pipelines on top of \sys's outputs, relying on keyless-join-based context enrichment as a key primitive.
Examples of such workloads include the recommendation example from Figure~\ref{fig:example}, which we simulate as a case study in Section~\ref{subsec:extensibility}, open domain question answering, data augmentation, or applications that involve humans in the loop to verify matches or drive business needs. 

\minihead{Multi-Dataset Extension} The joining step may vary in the multi-dataset case in two ways. 
In a first scenario, each auxiliary data source $D_i$ is indexed, and the query retrieval phase will query each of these indexes and return candidate related data points for each pairwise interaction. 
If multiple data sources must be sequentially aligned and a DAG can be specified over this sequence, a user can chain context enrichment subroutines by querying the next index with the records retrieved by the previous subroutine; we provide a toy example of this scenario in Section~\ref{subsec:extensibility} under Recommendation. 

%\sys does not currently support other potential use cases for a keyless join enrichment layer, and is an area for future work.

==> context enrichment 8/keyless.tex <==
\section{Learned Keyless Joins for Context Enrichment}

Although the applications in Section~\ref{sec:applications} implicitly or explicitly perform the \emph{same} context enrichment, many state-of-the-art systems for these tasks re-implement and rediscover primitives across domains spanning machine learning, databases, information retrieval, and natural language processing~\citep{colbert,ditto,knnlm,rpt}.
We propose learned \textit{keyless joins} as an abstraction to unify context enrichment across these tasks and provide a vehicle to develop a no-code system with out-of-the-box recall exceeding na\"ive baselines.
In this section, we define keyless joins, provide a keyless join API specification, and introduce Transformer models that enable general keyless joins. 

\subsection{Keyless Joins: Definition and Objective}
\label{subsec:keyless}

%We identify that the common required functionality is to align data sources \emph{without} explicit primary key-foreign key (KFK) relationships.
%In response, we ask, is it possible to develop a general framework for context enrichment that enables practitioners to initialize pipelines across all motivating applications using a high-level configuration file?
%Our goal is to develop a no-code system with out-of-the-box performance exceeding na\"ive baselines across all of these tasks.
%To answer this question, we identify that the common required functionality is to align data sources \emph{without} explicit primary key-foreign key (KFK) relationships.
Context enrichment requires a similarity-based join that operates at the record-, not schema-, level to retrieve related records without primary key-foreign key (KFK) relationships. 
We propose learned \emph{keyless joins} as an abstraction to enable this functionality.
The goal of a keyless join is to quantify the relatedness of records across different datasets to identify records referring to similar entities.

A keyless join must learn a common embedding space $\mathbf{X}$ for all records $d_{ij}$ across datasets $D_0 \cup D$ that reflects entity similarity.
For each $\mathbf{D_i}$, a keyless join learns a function $F_i: \mathbf{D_i} \rightarrow \mathbf{X}$ that maps elements of $D_i$ to the space $\mathbf{X}$.
We denote each transformed data point $F_i(d_{ij})$ as $x_{ij}$.
This mapping must be optimized such that related values map to similar feature vectors in $\mathbf{X}$ and unrelated values map to distant feature vectors in $\mathbf{X}$: $sim(x_{ij}, x_{kl}) > sim(x_{ij}, x_{mn})$ implies that the $j^{th}$ entity in the $i^{th}$ dataset is more closely related to the $l^{th}$ entity in the $k^{th}$ dataset than the $n^{th}$ entity in the $m^{th}$ dataset.
For instance, if we define similarity with respect to an $\ell_p$-norm, the above condition is equal to optimizing for  $\|x_{ij} -  x_{kl}\|_p < \|x_{ij} - x_{mn}\|_p$.

%In this paper, we describe how building a configurable system that implements a keyless join abstraction layer enables context enrichment.

\begin{figure*}
\includegraphics[width=\linewidth]{figures/full_pipeline.pdf}
\caption{\sys system architecture.}
\label{fig:pipeline}
%\vspace{-1em}
\end{figure*}


\subsection{Join Specification for Context Enrichment}
\label{subsec:keyless_spec}

%By leveraging keyless joins as a building block to surface and and quantify relatedness across entities, 
We propose a minimal join specification for our applications using keyless joins as a building block (Listing~\ref{listing:spec}).
Given a pair of data sources to join (\texttt{base\_table\_ref}, \texttt{aux\_table\_ref}), and examples of similar records across them (\texttt{supervision}), users first specify the \texttt{join type}: an inner join to only return enriched records, or outer join (left, right, full) to return enriched and unenriched records.
Users then specify the \texttt{join size}: how many records from one data source joins to a single record in the other data source to indicate one-to-one, one-to-many, or many-to-many semantics. 

As output, joined tuples (matches) between the two tables are the most similar records across them as learned using the keyless join objective. 
Results are ranked in order of greatest entity similarity, and the top k results are returned based on \texttt{join size}. 

\eat{
\begin{listing}[t]
\small
%\usemintedstyle{trac}
\begin{minted}{python}
base_table_ref [join_type] "KEYLESS JOIN" aux_table_ref 
"LEFT SIZE" integer "RIGHT SIZE" integer
"USING" supervision;

join_type = "INNER" | "LEFT" | "RIGHT" | "FULL";
\end{minted}
\caption{Keyless join specification and syntax, which defaults to an inner join.}
\label{listing:spec}
\end{listing}
}


\begin{lstlisting}[frame=single,caption={Keyless join specification (inner join default).},captionpos=b,float=t,label={listing:spec}, language=Python,commentstyle=\textcolor{teal},stringstyle=\dred,showstringspaces=false,belowskip=-2pt]
base_table_ref [join_type] "KEYLESS JOIN" aux_table_ref 
"LEFT SIZE" integer "RIGHT SIZE" integer
"USING" supervision;

join_type = "INNER" | "LEFT" | "RIGHT" | "FULL";
\end{lstlisting}






For instance, an entity matching application is written as follows to retrieve a single matching record between each data source:
\vsepfbox{%
    \parbox{.975\linewidth}{%
        \small{\texttt{%
            entity\_mentions\_A \dred{INNER KEYLESS JOIN} entity\_mentions\_B \\
            \dred{LEFT SIZE} 1 \dred{RIGHT SIZE} 1 \dred{USING} matching\_mentions;
        }}
    }%
}

\eat{\texttt{
\dred{entity\_mentions\_A} INNER KEYLESS JOIN \dred{entity\_mentions\_B}
LEFT SIZE \dred{1} RIGHT SIZE \dred{1}
}}


A search application is written as follows to retrieve 10 documents for each search query, else return the unenriched query: \\
\vsepfbox{%
    \parbox{.975\linewidth}{%
        \small{\texttt{%
        query\_corpus \dred{LEFT KEYLESS JOIN} document\_corpus \\
        \dred{LEFT SIZE} 1 \dred{RIGHT SIZE} 10 \dred{USING} relevant\_docs\_for\_query;
        }}
    }%
}

A recommendation application is written as follows to retrieve 10 items for each user, and 20 users who like each item: \\
\vsepfbox{%
    \parbox{.975\linewidth}{%
        \small{\texttt{%
        user\_database \dred{INNER KEYLESS JOIN} product\_database \\
        \dred{LEFT SIZE} 20 \dred{RIGHT SIZE} 10 \dred{USING} relevant\_docs\_for\_query;
        }}
    }%
}

In the remainder of paper, we describe our prototype system that implements this keyless join abstraction layer for enrichment.



\subsection{Background: Transformer-Based Encoders}
\label{subsec:transformer}

Our main tools for creating a representation optimized for the objective in Section~\ref{subsec:keyless} are Transformers~\citep{transformers}, as they have demonstrated success across a range of structured, semi-structured, and unstructured domains~\citep{tabert,bert,gpt2,neuraldb,picket}.
They consist of an encoder-decoder architecture, where the Transformer first encodes the input to an intermediate representation, and then decodes this representation to produce the end output.
Stacking encoder (e.g., BERT~\citep{bert}) or decoder (e.g., GPT-2~\citep{gpt2}) modules allows us to learn high-quality word embeddings that can either be used for a wide array of downstream applications. 
We focus on BERT-based embeddings. 

BERT embeddings used for a downstream task are trained in a two-step procedure. 
The first step is self-supervised pretraining using a masked language model (MLM) objective: a random subset of tokens are masked, and the model must predict each masked token given the surrounding text as context. 
Pretraining is performed with general purpose corpora such as Wikipedia. %is compute-intensive and 
The second step is task-specific fine-tuning. 
Additional layers are appended to the final layer of the pretrained model based on the downstream task, and all model parameters are updated given small amounts of downstream supervision. 
Rather than relying solely on fine-tuning, an additional MLM pretraining step can be performed prior to fine-tuning to introduce additional domain knowledge. %in the presence of altered data vocabulary. 


==> context enrichment 8/preprocessing.tex <==
\section{Preprocessing}
\label{sec:preprocessing}

In this section, we describe the first step of \sys's pipeline: preprocessing. 
Users provide base and auxiliary datasets with examples of related records across the two. 
\sys first processes the input datasets so all records are represented in a comparable format. 
\sys then pretrains the \encoders for the representation learning step. 
%The processed data and pretrained \encoders are passed to the next step.
We describe these phases, and then multi-dataset extension.


\minihead{Data Preparing (Figure~\ref{fig:pipeline}A.1)} This phase converts each \record $d_{ij}$ into a format that can be used for downstream Transformer-based \encoders regardless of schema.  
Motivated by recent work in representing structured data as sentences~\citep{tabert, neuraldb}, \sys's default pipeline uses a \sentence \preparer $P$ to convert input \records $d_{ij}$ into \sentences $P(d_{ij}) = s_{ij}$. 
Each key-value pair in $d_{ij}$ is converted to a string and separated by the \encoder's separator token as \texttt{``key\_1 value\_1 [SEP] key\_2 value\_2 [SEP]..."} (Figure~\ref{fig:preprocess}).

\minihead{Optional Pretraining (Figure~\ref{fig:pipeline}A.2)}
Our default BERT-based \encoder is trained over natural language corpora (Wikipedia and BookCorpus~\citep{wiki,bookcorpua}). 
Structured data is often domain-specific, and is of a different distribution than natural language.
Thus, we find that bootstrapping the pipeline's \encoders via additional pretraining can improve performance by up to \red{2.08$\times$}.
\sys provides a pretraining configuration option that is enabled by default.

Users can pretrain the pipeline's \encoders via BM25-based self-supervision (out-of-the-box) or by developing weak supervision-based \labelers (custom-built).
%By default, \sys provides a self-supervised MLM pretraining routine.
We add a standard Masked Language Modeling (MLM) head to each pipeline \encoder, and pretrain it following the original BERT pretraining procedure that fits a reconstruction loss. %: 15\% of the tokens are selected for prediction, of which 80\% are masked at random, 10\% are replaced with a random token, and 10\% are kept the same. 
To  encourage the spread of contextual information across the two tables, we concatenate one \sentence from each table to one other as pretraining input as \texttt{``$s_{ij}$ [SEP] $s_{kl}$"} (Figure~\ref{fig:preprocess}). 
We select \sentence pairs that are likely to share information in an unsupervised manner via BM25, a bag-of-words relevance ranking function~\citep{bm25}, though any domain-specific unsupervised similarity join can be used, such as from Magellan~\citep{magellan} or AutoFJ~\citep{autofj}. 
We evaluate BM25-based MLM pretraining in Section~\ref{subsec:micros}.
%For domain-specific pretraining, users must provide their own weak supervision \labelers or similarity functions. 
%We find BM25-based pretraining works well for tasks that where similarity as defined by the downstream task is correlated with overlapping phrases. 
%For other notions of domain-specific similarity, users must provide their own weak supervision \labelers or similarity functions. 
During development, we explored learning conditional representations of each table given the other by selectively masking one table's \sentences, but found no change in performance compared to uniform masking. 

\minihead{Multi-Dataset Extension} 
Depending on the encoder configuration used in the multi-dataset case, the BM25-based pretraining step will be applied to all \sentences across all datasets at once (anchored from the base table), or each dataset pairwise. 

\begin{figure}
\includegraphics[width=\columnwidth]{figures/preprocessing.pdf}
\caption{Examples of the data preparing and pretraining phases of the preprocessing architecture step.}
\label{fig:preprocess}
\vspace{-1em}
\end{figure}

==> context enrichment 8/relwork.tex <==
\section{Related Work}
\label{sec:relwork}

\minihead{Similarity Joins} Similarity-based, or fuzzy, joins often focus on the unsupervised setting~\citep{surajit,fj1,fj2}. 
State-of-the art systems such as AutoFJ~\citep{autofj} are tailored for the case where tables can be joined using exact keys or shared phrases that do not differ greatly in distribution (e.g., our EM tasks)---not complex context enrichment.
\sys generalizes to arbitrary notions of similarity and join semantics at the expense of supervised pairs, and can also leverage unsupervised methods for negative sampling or MLM pretraining.

\minihead{Automated Machine Learning} Automated Machine Learning (AML) systems aim to empower users to develop high-performance ML pipelines minimal intervention or manual tuning. They support various types of data preprocessing, feature engineering, model training and monitoring modules. Examples of AML tools include Ludwig~\citep{ludwig}, Overton~\citep{overton}, Google Cloud AutoML~\citep{gcloud}, and H20.ai~\citep{h20}. However, these platforms do not focus on context enrichment, leaving it as an exercise for users to perform prior to data ingestion. 

\minihead{Relational Data Augmentation}
Relational data augmentation systems seek to find new features for a downstream predictive task by deciding whether or not to perform standard database joins across a base table and several auxiliary tables~\citep{hamlet, hamletpp, arda}. 
Similar to context enrichment, these systems aim to augment a base table for a downstream ML workload. 
However, they assume the existence of KFK relationships that simply must be uncovered. 

\minihead{Data Discovery} Data discovery systems find datasets that may be joinable with or related to a base dataset, and to uncover relationships between different datasets using dataset schema, samples, and metadata~\citep{dd1,dd2,dd3,dd4,dd5,dd6,dd7}.
These systems typically surface KFK relationships, and do not tune for downstream ML workloads.


\minihead{NLP and Data Management} A recurring aim in data management is to issue natural language commands to interface with structured data~\citep{nlidb,csc}. Recent work in Neural Databases~\citep{neuraldb} aims to replace standard databases with Transformer-powered schemaless data stores that are updated and queried with natural language commands. Related to this work are systems that leverage advances in NLP to provide domain-specific functionality, such as converting text to SQL~\citep{text2sql1,text2sql2}, correlating structured and unstructured data~\citep{tabert}, enabling interpretable ML over structured data~\citep{tabnet}, or automating data preparation~\citep{rpt}. We focus on the broader problem of context enrichment of entities for downstream tasks. To our knowledge, this has not been formally addressed in the literature, which often assumes entity information has been resolved~\citep{neuraldb}.

==> context enrichment 8/representation.tex <==
\section{Representation Learning}
\label{sec:representation}

In this section, we describe the second step of \sys's pipeline: representation learning.
Given the \sentences and optionally pretrained \encoders from the first step, \sys fine-tunes the \encoders such that \embeddings from related records are close in embedding space. 
These \embeddings are then passed to the final pipeline step. 
Users can choose how many \encoders to configure, the \encoder architecture and output dimension, and how to train the \encoders, which we now detail prior to describing multi-dataset extension.

\minihead{\texttt{Encoder} configuration} \sys provides a choice of training independent \encoders, $E_i$ for each data source, or using a single \encoder $E_0$ common to all data sources. 
In all of our scenarios, using a single, common \encoder performs best, sometimes by over an order of magnitude, and is set as \sys's default configuration.
In our tasks, we found that using separate encoders perturbs the representations such that exact matches no longer share a representation---thus, the encoders must relearn correspondences, and often fail to.
%We found that for our tasks, using separate encoders with no additional forms of supervision perturbs the representations such that exact matches no longer share a representation---thus, the encoders must relearn correspondences, and often fail to.
%However, to extend \sys to non-textual data sources, or hybrid structured-unstructured settings (e.g., text-image for image captioning or joint sentiment analysis, or text-audio tasks), users must leverage source-specific \encoders---we provide them as a configurable option.
However, to extend \sys to non-textual data (e.g., images, video, text-image for image captioning or joint sentiment analysis, or text-audio tasks), users must leverage source-specific \encoders---thus, we provide them as a configurable option.

\minihead{\texttt{Encoder} architecture} \sys lets users configure each \encoder's base architecture and the size of the learned \embeddings. 
Users can choose BERT$_{\text{base}}$ or DistilBERT$_{\text{base}}$ as the core architecture; \sys's default is the 40\% smaller, and 60\% faster DistilBERT model.
We use models from HuggingFace Transformers~\citep{hf}; thus, integrating new architectures requires few additional lines of code.

We remove the MLM head used in the preprocessing step for optional pretraining, and replace it with a fully connected layer that transforms BERT's default 768-dimensional output to a user-specified \embedding output dimension, $d$. 
The output of the fully connected layer is a $d$-dimensional embedding for each input token. 
Users can choose one of two types of aggregation methods that will return a single $d$-dimensional output per input \sentence: averaging all of the embeddings, or using the embedding of the leading \texttt{CLS} token that BERT appends to its input data (Figure~\ref{fig:preprocess}). 
\sys defaults to \texttt{CLS}-based aggregation with a 200-dimensional output.
%Evaluating alternative means of aggregation, such as concatenation followed by dimensionality reduction, is left for future work. 

\minihead{\texttt{Encoder} training} The \encoders' goal is to learn a representation (\embedding), for the data sources such that \sentences that refer to similar entities are grouped in the underlying embedding space. 
Recall that to perform a keyless join under an $\ell_p$-norm, each \encoder must learn a function that maps elements of $D_i$ to the space $\mathbf{X}$, such that $\|x_{ij} -  x_{kl}\|_p < \|x_{ij} - x_{mn}\|_p$ when the $j^{th}$ entity in the $i^{th}$ dataset is more closely related to the $l^{th}$ entity in the $k^{th}$ dataset than the $n^{th}$ entity in the $m^{th}$ dataset.
We directly optimize for this objective function by training \encoders using a contrastive, triplet loss together with user-provided supervision.

Given an anchor \record  $d_{0\text{a}}$ from $D_0$, and  \records $d_{1\text{p}}$ and $d_{1\text{n}}$ in $D_1$ that are related and unrelated to $d_{0\text{a}}$, respectively, let $F_0(d_{0\text{a}}) = x_{0\text{a}}$, $F_1(d_{1\text{p}}) = x_{1\text{p}}$, and $F_1(d_{1\text{n}}) = x_{1\text{n}}$ be their \embeddings following the composition of the \sentence \preparer $P$ and \encoder $E_i$ operators ($F_i=E_i \circ P$).
%, with only  $F_0=E_0 \circ P$ in the default single-\encoder case. 
We minimize the triplet loss, defined as:
$$ \mathcal{L}(x_{0\text{a}}, x_{1\text{p}}, x_{1\text{n}}) = \max\{\|x_{0\text{a}} - x_{1\text{p}}\|_p,  \|x_{0\text{a}} - x_{1\text{n}}\|_p + \alpha, 0\}$$

\noindent where $\alpha$ is a hyperparameter controlling the margin between related and unrelated \embeddings.
%Intuitively, this contrastive loss encourages representations for related data points to be closer together than representations for unrelated data points. 
Users could use an alternative \loss function: a cosine similarity loss would provide representations that similarly encourage related points to be close and unrelated points to be far, and a standard binary cross-entropy loss may be used as well, where the final layer in the trained \encoder would be the end embeddings.
However, they do not explicitly optimize for \textit{relative} distances between related and unrelated records. 

Users often have examples of related pairs, but no unrelated examples to form triples.
In our tasks, only the search workload provides triples, while the rest provide lists of related pairs, which we represent with a \labeler. 
As a result, we provide negative \sampler operators to convert \labelers that operate over pairs to the triples required by the triplet \loss. 
If the user-provided \labeler already contains a related and unrelated example for a \record, we form a triple using these examples.
If a \record does not contain a related and unrelated example, for each \record $d_{0j}$ in $D_0$ with a labeled related record, we use either a random \sampler or a stratified hard negative \sampler. 
The random \sampler selects a \record at random (that is not a supervised related pair) as an example unrelated \record. The stratified \sampler provides tiers for different degrees of relatedness for the negative examples---a user can specify a region of hard examples to sample from, given prior domain knowledge.
We provide a default stratified \sampler with a single tier of relatedness defined using BM25 or Jaccard similarity, though any unsupervised join method can be used (including AutoFJ~\citep{autofj}). We show that a hard negative \sampler improves recall by up to \red{30\%} compared to a random \sampler in Section~\ref{subsec:micros}.



\minihead{Multi-Dataset Extension} The \encoder configuration and architecture are unchanged in the multi-dataset case. 
There are two options for the \encoder training procedure.
The first scenario follows the context enrichment problem definition---where a base table $D_0$ must be augmented with several auxiliary data sources $D$. 
In this case, each \encoder can be trained pairwise with $D_0$ and $D_i$ as described above.
In the case where multiple data sources must be aligned in sequence, a user can successively apply \sys over a data DAG created using their prior knowledge---effectively creating several, sequential context enrichment problems as described in Section~\ref{subsec:target} for multi-hop question answering. 
Else, \sys can induce a DAG and sequentially traverse the space of possible keyless joins based on the cardinality of each dataset, in ascending order.




==> context enrichment 8/shortcuts.tex <==
\usepackage{graphicx}
\usepackage{balance}  % for  \balance command ON LAST PAGE  (only there!)
%\usepackage{xcolor}
%\usepackage[dvipsnames]{xcolor}
\usepackage{comment}
\usepackage{xspace}
\usepackage{cite}
\usepackage{enumitem}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{multirow}
\usepackage{fancyvrb}
\usepackage{listings}

\lstset{
  basicstyle=\sffamily\small,
  columns=fixed,
  fontadjust=true,
  basewidth=0.5em,
  frame=single, % adds a frame around the code
  xleftmargin=3.4pt,
  xrightmargin=3.4pt,
}
%\usepackage[table,xcdraw]{xcolor}
%\usepackage[table,xcdraw]{xcolor}
\usepackage{colortbl}
\usepackage{hhline}
\usepackage{listings}
\usepackage{newfloat}
\usepackage{fancyvrb}



\definecolor{mahogany}{HTML}{85200c}

% Comments
\newcommand{\reword}[1]{{\color{violet}{#1}}}
\newcommand{\todo}[1]{{\color{red}TODO: {#1}}}
%\newcommand{\new}[1]{{\color{violet} {#1}}}
\newcommand{\new}[1]{{{#1}}}
\newcommand{\red}[1]{{\color{black} {#1}}}
\newcommand{\dred}[1]{{\color{mahogany} {#1}}}
\newcommand{\ch}[1]{{{#1}}}


% Macros for Names
\newcommand{\orgres}{organizational resource\xspace}
\newcommand{\enrich}{\textsc{enrich}\xspace}
\newcommand{\sys}{\textsc{Ember}\xspace}
\newcommand{\record}{\texttt{record}\xspace}
\newcommand{\sentence}{\texttt{sentence}\xspace}
\newcommand{\encoder}{\texttt{encoder}\xspace}
\newcommand{\labeler}{\texttt{labeler}\xspace}
\newcommand{\embedding}{\texttt{embedding}\xspace}
\newcommand{\loss}{\texttt{loss}\xspace}
\newcommand{\sampler}{\texttt{sampler}\xspace}
\newcommand{\preparer}{\texttt{preparer}\xspace}
\newcommand{\retriever}{\texttt{retriever}\xspace}
\newcommand{\records}{\texttt{record}s\xspace}
\newcommand{\sentences}{\texttt{sentence}s\xspace}
\newcommand{\encoders}{\texttt{encoder}s\xspace}
\newcommand{\labelers}{\texttt{labeler}s\xspace}
\newcommand{\embeddings}{\texttt{embedding}s\xspace}
\newcommand{\losses}{\texttt{loss}es\xspace}
\newcommand{\samplers}{\texttt{sampler}s\xspace}
\newcommand{\preparers}{\texttt{preparer}s\xspace}
\newcommand{\retrievers}{\texttt{retriever}s\xspace}


% Miniheads
\newcommand{\miniheadnostop}[1]{{\vspace{.4em}\noindent\textbf{#1} }}
\newcommand{\minihead}[1]{{\vspace{.45em}\noindent\textbf{#1.} }}
\newcommand{\miniheadit}[1]{{\vspace{.45em}\noindent\textit{#1.} }}
\newcommand{\miniheadnopd}[2]{{\vspace{.4em}\noindent\textbf{#1}\hspace{.5em}{#2}\vspace{.4em} }}
\newcommand{\minidef}[1]{{\vspace{.25em}\noindent\textit{#1} }}



% Comment
\newcommand{\eat}[1]{}

% new vsep box
\newcommand*{\vsepfbox}[1]{%
  \begingroup
    \sbox0{\fbox{#1}}%
    \setlength{\fboxrule}{0pt}%
    \mbox{\kern-\fboxsep\fbox{\unhbox0}\kern-\fboxsep}%
  \endgroup
}


% newfloat for listing
\DeclareFloatingEnvironment[
  fileext = los ,
  listname = {List of listings} ,
  name = Listing
]{llisting}

==> context enrichment 8/tables/baselines-k.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll|c|c|c|c|c|c|c|c|}
\cline{3-10}
\textbf{}                           & \textbf{}        & \multicolumn{8}{c|}{\textbf{k-to-90}}                                                                                                                                                                \\ \hline
\multicolumn{1}{|l|}{\textbf{Task}} & \textbf{Dataset} & \textbf{\textsc{ld}} & \textbf{\textsc{jk-ws}} & \textbf{\textsc{jk-2g}} & \textbf{\textsc{l-ws}} & \textbf{\textsc{J-2g}} & \textbf{\textsc{bert}} & \textbf{\textsc{bm25}} & \textbf{\textsc{emb}} \\ \hline
\multicolumn{1}{|l|}{FJ}            & IMDb-easy        &                      &                         & \textbf{}               &                        & \textbf{}              &                        &                        &                       \\ \hline
\multicolumn{1}{|l|}{FJ}            & IMDb-med         &                      &                         &                         &                        & \textbf{}              &                        &                        &                       \\ \hline
\multicolumn{1}{|l|}{QA}            & SQuAD            &                      &                         &                         &                        &                        &                        &                        & \textbf{}             \\ \hline
\multicolumn{1}{|l|}{S}             & MS MARCO         &                      &                         &                         &                        &                        &                        &                        & \textbf{}             \\ \hline
\multicolumn{1}{|l|}{R}             & IMDb-wiki-join   &                      &                         &                         & \textbf{}              &                        &                        &                        &                       \\ \hline
\multicolumn{1}{|l|}{EM-T}          & Abt-Buy          &                      &                         & \textbf{}               &                        &                        &                        &                        & \textbf{}             \\ \hline
\multicolumn{1}{|l|}{EM-T}          & Company          &                      &                         &                         &                        &                        &                        & \textbf{}              & \textbf{}             \\ \hline
\multicolumn{1}{|l|}{EM-S}          & Avg,  < 200 Test &                      &                         &                         &                        &                        &                        & \textbf{}              &                       \\ \hline
\multicolumn{1}{|l|}{EM-S}          & Avg, > 200 Test  &                      &                         &                         &                        & \textbf{}              &                        & \textbf{}              & \textbf{}             \\ \hline
\multicolumn{1}{|l|}{EM-D}          & Avg. < 200 Test  &                      &                         &                         &                        &                        &                        & \textbf{}              &                       \\ \hline
\multicolumn{1}{|l|}{EM-D}          & Avg. > 200 Test  &                      &                         &                         & \textbf{}              & \textbf{}              &                        & \textbf{}              & \textbf{}             \\ \hline
\end{tabular}%
}
\caption{Number of records retrieved to achieve a 90\% recall.}
\label{tab:kneeded}
\end{table}

==> context enrichment 8/tables/baselines.tex <==
\eat{
% \cellcolor[HTML]{FEA9A9}\textsc{emb}
% \hhline{~~----------------}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|c|c|c|c|c|c|c|c||c|c|c|c|c|c|c|c|}
\hhline{~~----------------}
\textbf{}                                                   & \textbf{}        & \multicolumn{8}{c||}{\cellcolor[HTML]{EFEFEF}\textbf{Recall@1}}                                                                                                                                                                                                                                                 & \multicolumn{8}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Recall@10}}                                                                                                                                                                                                                                \\ \hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}\textbf{Task}} & \textbf{Dataset} & \textbf{\textsc{ld}}                   & \textbf{\textsc{J-2g}}                  & \textbf{\textsc{JK-2g}}                & \textbf{\textsc{JK-ws}} & \textbf{\textsc{J-ws}}                 & \textbf{\textsc{BM25}}                 & \textbf{\textsc{bert}} & \cellcolor[HTML]{A4C8E9}\textbf{\textsc{emb}} & \textbf{\textsc{ld}}                   & \textbf{\textsc{J-2g}}                  & \textbf{\textsc{JK-2g}}                & \textbf{\textsc{JK-ws}} & \textbf{\textsc{J-ws}}                 & \textbf{\textsc{BM25}} & \textbf{\textsc{bert}} & \cellcolor[HTML]{A4C8E9}\textbf{\textsc{emb}} \\ \hline
\multicolumn{1}{|l|}{FJ}                                    & IMDb-easy        & \cellcolor[HTML]{DCEAF7}\textbf{99.32} & \cellcolor[HTML]{DCEAF7}\textbf{100.00} & \cellcolor[HTML]{DCEAF7}\textbf{99.42} & 88.41                   & 91.61                                  & 91.81                                  & 45.85                  & 97.86                                         & \cellcolor[HTML]{DCEAF7}\textbf{99.99} & \cellcolor[HTML]{DCEAF7}\textbf{100.00} & \cellcolor[HTML]{DCEAF7}\textbf{99.96} & 96.13                   & 96.30                                  & 96.33                  & 69.83                  & \cellcolor[HTML]{DCEAF7}\textbf{99.79}        \\ \hline
\multicolumn{1}{|l|}{FJ}                                    & IMDb-med         & 95.54                                  & \cellcolor[HTML]{DCEAF7}\textbf{98.87}  & 95.30                                  & 63.13                   & 52.29                                  & 54.58                                  & 8.72                   & 88.92                                         & \cellcolor[HTML]{DCEAF7}\textbf{99.04} & \cellcolor[HTML]{DCEAF7}\textbf{99.82}  & 98.55                                  & 80.62                   & 64.34                                  & 65.82                  & 21.11                  & 98.37                                         \\ \hline
\multicolumn{1}{|l|}{QA}                                    & SQuAD            & 5.52                                   & 34.71                                   & 41.28                                  & 30.56                   & 27.28                                  & 49.17                                  & 11.37                  & \cellcolor[HTML]{DCEAF7}\textbf{52.91}        & 6.07                                   & 52.84                                   & 61.20                                  & 46.44                   & 43.22                                  & 67.08                  & 27.03                  & \cellcolor[HTML]{DCEAF7}\textbf{78.85}        \\ \hline
\multicolumn{1}{|l|}{S}                                     & MS MARCO         & 0.26                                   & 1.66                                    & 1.66                                   & 1.15                    & 1.15                                   & 2.31                                   & 0.01                   & \cellcolor[HTML]{DCEAF7}\textbf{16.34}        & 0.96                                   & 7.38                                    & 7.38                                   & 5.11                    & 5.11                                   & 4.10                   & 0.10                   & \cellcolor[HTML]{DCEAF7}\textbf{46.98}        \\ \hline
\multicolumn{1}{|l|}{R}                                     & IMDb-wiki-join   & 59.10                                  & 11.01                                   & 82.58                                  & 88.36                   & \cellcolor[HTML]{DCEAF7}\textbf{99.83} & 63.25                                  & 0.04                   & 97.02                                         & 64.78                                  & 18.80                                   & 93.13                                  & 94.36                   & \cellcolor[HTML]{DCEAF7}\textbf{99.83} & 96.25                  & 0.26                   & \cellcolor[HTML]{DCEAF7}\textbf{98.89}        \\ \hline
\multicolumn{1}{|l|}{EM-T}                                  & Average All      & 25.34                                  & 20.05                                   & 36.56                                  & 36.97                   & 37.21                                  & 61.09                                  & 6.88                   & \cellcolor[HTML]{DCEAF7}\textbf{71.93}        & 35.81                                  & 37.60                                   & 49.00                                  & 56.26                   & 53.11                                  & 71.90                  & 21.45                  & \cellcolor[HTML]{DCEAF7}\textbf{83.29}        \\ \hline
\multicolumn{1}{|l|}{EM-S}                                  & Average All      & 53.39                                  & 73.50                                   & 72.30                                  & 69.87                   & 72.71                                  & \cellcolor[HTML]{DCEAF7}\textbf{76.59} & 38.98                  & \cellcolor[HTML]{DCEAF7}\textbf{77.20}        & 71.76                                  & 94.41                                   & \cellcolor[HTML]{DCEAF7}\textbf{97.90} & 94.13                   & 93.33                                  & 95.19                  & 55.88                  & \cellcolor[HTML]{DCEAF7}\textbf{97.58}        \\ \hline
\multicolumn{1}{|l|}{EM-D}                                  & Average All      & 36.84                                  & 64.69                                   & 52.05                                  & 53.55                   & 61.94                                  & 65.47                                  & 30.61                  & \cellcolor[HTML]{DCEAF7}\textbf{66.56}        & 48.41                                  & 90.86                                   & 80.92                                  & 79.77                   & 89.85                                  & 92.31                  & 43.92                  & \cellcolor[HTML]{DCEAF7}\textbf{97.83}        \\ \hline
\end{tabular}%
}
\caption{Baseline comparison, where we highlight all methods within 1\% of the best for each task. No single baseline dominates the other, but Ember (\textsc{emb}) is competitive with or better than alternatives in nearly all tasks with respect to Recall@k.}
\label{tab:baselines}
\end{table*}}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|c|c|c|c|c|c|c|c||c|c|c|c|c|c|c|c|}
\hhline{~~----------------}
                                                   &                                 & \multicolumn{8}{c||}{\cellcolor[HTML]{EFEFEF}\textbf{Recall@1}}                                                                                                                                                                                                                                          & \multicolumn{8}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Recall@10}}                                                                                                                                                                                                                         \\ \hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}Task} & \cellcolor[HTML]{EFEFEF}Dataset & \textbf{\textsc{LD}}                   & \textbf{\textsc{J-2g}}                  & \textbf{\textsc{JK-2g}}                & \textbf{\textsc{JK-ws}} & \textbf{\textsc{J-ws}} & \textbf{\textsc{BM25}}                 & \textbf{\textsc{bert}} & \cellcolor[HTML]{A4C8E9}\textbf{\textsc{emb}} & \textbf{\textsc{LD}}                   & \textbf{\textsc{J-2g}}                  & \textbf{\textsc{JK-2g}}                & \textbf{\textsc{JK-ws}} & \textbf{\textsc{J-ws}} & \textbf{\textsc{BM25}} & \textbf{\textsc{bert}} & \cellcolor[HTML]{A4C8E9}\textbf{\textsc{emb}} \\ \hline
\multicolumn{1}{|l|}{FJ}                           & IMDb                       & \cellcolor[HTML]{DCEAF7}\textbf{99.32} & \cellcolor[HTML]{DCEAF7}\textbf{100.00} & \cellcolor[HTML]{DCEAF7}\textbf{99.42} & 71.54                   & 91.61                  & 91.81                                  & 45.85                  & 97.86                                         & \cellcolor[HTML]{DCEAF7}\textbf{99.99} & \cellcolor[HTML]{DCEAF7}\textbf{100.00} & \cellcolor[HTML]{DCEAF7}\textbf{99.96} & 96.13                   & 96.30                  & 96.33                  & 69.83                  & \cellcolor[HTML]{DCEAF7}\textbf{99.79}        \\ \hline
\multicolumn{1}{|l|}{FJ}                           & IMDb-hard                       & 95.54                                  & \cellcolor[HTML]{DCEAF7}\textbf{98.87}  & 95.02                                  & 33.42                   & 52.29                  & 54.58                                  & 8.72                   & 88.92                                         & \cellcolor[HTML]{DCEAF7}\textbf{99.04} & \cellcolor[HTML]{DCEAF7}\textbf{99.82}  & 98.26                                  & 42.68                   & 64.34                  & 65.82                  & 21.11                  & 98.37                                         \\ \hline
\multicolumn{1}{|l|}{QA}                           & SQuAD                           & 1.37                                   & 34.70                                   & 41.26                                  & 29.47                   & 27.26                  & 49.17                                  & 11.37                  & \cellcolor[HTML]{DCEAF7}\textbf{52.91}        & 1.50                                   & 52.82                                   & 61.18                                  & 44.79                   & 43.18                  & 67.08                  & 27.03                  & \cellcolor[HTML]{DCEAF7}\textbf{78.85}        \\ \hline
\multicolumn{1}{|l|}{S}                            & MS MARCO                        & 0.26                                   & 1.66                                    & 1.66                                   & 1.15                    & 1.15                   & 2.31                                   & 0.01                   & \cellcolor[HTML]{DCEAF7}\textbf{16.34}        & 0.96                                   & 7.38                                    & 7.38                                   & 5.11                    & 5.11                   & 4.10                   & 0.10                   & \cellcolor[HTML]{DCEAF7}\textbf{46.98}        \\ \hline
\multicolumn{1}{|l|}{R}                          & IMDb-wiki                       & 58.96                                  & 11.01                                   & 82.57                                  & 86.08                   & 18.30                  & 63.25                                  & 0.04                   & \cellcolor[HTML]{DCEAF7}\textbf{97.02}        & 64.62                                  & 18.80                                   & 93.12                                  & 91.93                   & 18.30                  & 96.25                  & 0.26                   & \cellcolor[HTML]{DCEAF7}\textbf{98.89}        \\ \hline
\multicolumn{1}{|l|}{EM-T}                         & Average                         & 18.20                                  & 20.06                                   & 36.56                                  & 36.90                   & 37.21                  & 61.09                                  & 6.88                   & \cellcolor[HTML]{DCEAF7}\textbf{71.93}        & 25.73                                  & 37.57                                   & 49.00                                  & 56.15                   & 53.11                  & 71.90                  & 21.45                  & \cellcolor[HTML]{DCEAF7}\textbf{83.29}        \\ \hline
\multicolumn{1}{|l|}{EM-S}                         & Average                         & 52.26                                  & 73.50                                   & 72.30                                  & 69.25                   & 72.71                  & \cellcolor[HTML]{DCEAF7}\textbf{76.59} & 38.98                  & \cellcolor[HTML]{DCEAF7}\textbf{77.20}        & 70.26                                  & 94.41                                   & \cellcolor[HTML]{DCEAF7}\textbf{97.90} & 93.51                   & 93.33                  & 95.19                  & 55.88                  & \cellcolor[HTML]{DCEAF7}\textbf{97.58}        \\ \hline
\multicolumn{1}{|l|}{EM-D}                         & Average                         & 18.70                                  & 64.69                                   & 52.05                                  & 53.41                   & 61.94                  & 65.47                                  & 30.61                  & \cellcolor[HTML]{DCEAF7}\textbf{66.56}        & 24.60                                  & 90.86                                   & 80.92                                  & 79.41                   & 89.85                  & 92.31                  & 43.92                  & \cellcolor[HTML]{DCEAF7}\textbf{97.83}        \\ \hline
\end{tabular}%
}
\caption{Baseline comparison, where we highlight all methods within 1\% of the best for each task. No single baseline dominates the other, but Ember (\textsc{emb}) is competitive with or better than alternatives in nearly all tasks with respect to Recall@k.}
\label{tab:baselines}
\vspace{-15pt}
\end{table*}

==> context enrichment 8/tables/datasets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|lrrrrr|}
\hline
\textbf{\textbf{Task}} & \textbf{\textbf{Dataset}} & \textbf{\textbf{\# base}} & \textbf{\textbf{\# aux}} & \textbf{\textbf{\# + train}} & \textbf{\textbf{\# + test }} & \textbf{\textbf{\# LoC}} \\ \hline
FJ                     & IMDb                      & 50000                     & 10000                     & 40000                     & 10000                     & 1                    \\ \hline
FJ                     & IMDb-hard                 & 50000                     & 10000                     & 40000                     & 10000                     & 1                    \\ \hline
QA                     & SQuAD                     & 92695                     & 64549                    & 86668                      & 6472                      & 2                        \\ \hline
S                      & MS MARCO                  & 508213                    & 8.8M                     & 418010                     & 7437                      & 1                       \\ \hline
R                      & IMDb-wiki                 & 47813                     & 47813                    & 38250                     & 9563                      & 1 (6)                       \\ \hline
EM-T                   & Abt-Buy                   & 1081                      & 1092                     & 616                        & 206                       & 2                      \\ \hline
EM-T                   & Company                   & 28200                     & 28200                    & 16859                      & 5640                      & 2                      \\ \hline
EM-S                   & BeerAdvo-RateBeer         & 4345                      & 3000                     & 40                         & 14                        & 1                        \\ \hline
EM-S                   & iTunes-Amazon             & 6907                      & 55923                    & 78                         & 27                        & 1                        \\ \hline
EM-S                   & Fodors-Zagat              & 533                       & 331                      & 66                         & 22                        & 1                        \\ \hline
EM-S                   & DBLP-ACM                  & 2616                      & 2294                     & 1332                       & 444                       & 1                        \\ \hline
EM-S                   & Amazon-Google             & 1363                      & 3226                     & 699                        & 234                       & 1                        \\ \hline
EM-S                   & DBLP-Scholar              & 2616                      & 64263                    & 3207                       & 1070                      & 1                        \\ \hline
EM-S                   & Walmart-Amazon            & 2554                      & 22074                    & 576                        & 193                       & 1                        \\ \hline
EM-D                   & DBLP-ACM                  & 2616                      & 2294                     & 1332                       & 444                       & 1                        \\ \hline
EM-D                   & DBLP-Scholar              & 2616                      & 64263                    & 3207                       & 1070                      & 1                        \\ \hline
EM-D                   & iTunes-Amazon             & 6907                      & 55923                    & 78                         & 27                        & 1                        \\ \hline
EM-D                   & Walmart-Amazon            & 2554                      & 22074                    & 576                        & 193                       & 1                        \\ \hline
\end{tabular}%
}
\caption{Data source record count, related pair (supervision) count, and number of configuration lines changed for the best recall@k, and for downstream tasks in parenthesis.}
\label{table:datasets}
\vspace{-10pt}
\end{table}


==> context enrichment 8/tables/dm.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|l|r||r|r|r|r|r|}
\hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{F3F3F3}\textbf{Task}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}\textbf{Dataset}} & \multicolumn{1}{c||}{\cellcolor[HTML]{F3F3F3}\textbf{R@10}} & \multicolumn{1}{c|}{\cellcolor[HTML]{a4c8e9}\textbf{\textsc{emb}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}\textbf{DM$_\text{RNN}$}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\textbf{DM$_\text{att}$}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\textbf{DM$_\text{hyb}$}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\textbf{Ditto}} \\ \hline
EM-T                                                        & Abt-Buy                                                       & 96.70                                                      & \cellcolor[HTML]{DCEAF7}85.05                            & \cellcolor[HTML]{DCEAF7}39.40                                         & \cellcolor[HTML]{DCEAF7}56.80                                         & \cellcolor[HTML]{DCEAF7}62.80                                         & 89.33                                                       \\ \hline
EM-T                                                        & Company                                                       & 69.89                                                      & \cellcolor[HTML]{DCEAF7}74.31                            & 85.60                                                                 & 89.80                                                                 & 92.70                                                                 & 93.85                                                       \\ \hline
EM-S                                                        & Beer                                                          & 92.86                                                      & \cellcolor[HTML]{DCEAF7}91.58                            & \cellcolor[HTML]{DCEAF7}72.20                                         & \cellcolor[HTML]{DCEAF7}64.00                                         & \cellcolor[HTML]{DCEAF7}78.80                                         & 94.37                                                       \\ \hline
EM-S                                                        & iTunes-Amzn                                                   & 100                                                        & \cellcolor[HTML]{DCEAF7}84.92                            & 88.50                                                                 & \cellcolor[HTML]{DCEAF7}80.80                                         & 91.20                                                                 & 97.06                                                       \\ \hline
EM-S                                                        & Fodors-Zagat                                                  & 100                                                        & \cellcolor[HTML]{DCEAF7}88.76                            & 100                                                                   & \cellcolor[HTML]{DCEAF7}82.10                                         & 100                                                                   & 100                                                         \\ \hline
EM-S                                                        & DBLP-ACM                                                      & 100                                                        & \cellcolor[HTML]{DCEAF7}98.05                            & \cellcolor[HTML]{DCEAF7}98.30                                         & \cellcolor[HTML]{DCEAF7}98.40                                         & \cellcolor[HTML]{DCEAF7}98.45                                         & \cellcolor[HTML]{DCEAF7}98.99                               \\ \hline
EM-S                                                        & Amazon-Google                                                 & 98.94                                                      & \cellcolor[HTML]{DCEAF7}70.43                            & \cellcolor[HTML]{DCEAF7}59.90                                         & \cellcolor[HTML]{DCEAF7}61.10                                         & \cellcolor[HTML]{DCEAF7}70.70                                         & 75.58                                                       \\ \hline
EM-S                                                        & DBLP-Scholar                                                  & 96.29                                                      & 57.88                                                    & 93.00                                                                 & 93.30                                                                 & 94.70                                                                 & 95.60                                                       \\ \hline
EM-S                                                        & Walmart-Amzn                                                  & 94.97                                                      & \cellcolor[HTML]{DCEAF7}69.60                            & \cellcolor[HTML]{DCEAF7}67.60                                         & \cellcolor[HTML]{DCEAF7}50.00                                         & 73.60                                                                 & 86.76                                                       \\ \hline
EM-D                                                        & DBLP-ACM                                                      & 99.96                                                      & \cellcolor[HTML]{DCEAF7}97.58                            & \cellcolor[HTML]{DCEAF7}97.50                                         & \cellcolor[HTML]{DCEAF7}97.40                                         & \cellcolor[HTML]{DCEAF7}98.10                                         & 99.03                                                       \\ \hline
EM-D                                                        & DBLP-Scholar                                                  & 95.99                                                      & 58.08                                                    & 93.00                                                                 & 92.70                                                                 & 93.80                                                                 & 95.75                                                       \\ \hline
EM-D                                                        & iTunes-Amazon                                                 & 100                                                        & \cellcolor[HTML]{DCEAF7}64.65                            & 79.40                                                                 & \cellcolor[HTML]{DCEAF7}63.60                                         & 79.40                                                                 & 95.65                                                       \\ \hline
EM-D                                                        & Walmart-Amzn                                                  & 95.39                                                      & \cellcolor[HTML]{DCEAF7}67.43                            & \cellcolor[HTML]{DCEAF7}39.60                                         & \cellcolor[HTML]{DCEAF7}53.80                                         & \cellcolor[HTML]{DCEAF7}53.80                                         & 85.69                                                       \\ \hline
\end{tabular}%
}
\caption{Recall@10 for \sys (R@10) and F1 Scores for the EM workloads using \sys with \texttt{join size = 1} (\textsc{emb}) compared to deep-learning-based EM solutions from DeepMatcher (DM$_*$) and Ditto. \sys meets or exceeds (highlighted) at least one recent, state-of-the-art classifier in most workloads. \sys has a low false negative rate (1 - R@10), and can be used \textit{with} these methods to increase precision}
\label{table:dm_all}
\vspace{-25pt}
\end{table}

==> context enrichment 8/tables/dm_micros.tex <==
\begin{table}[]
\small
\begin{tabular}{|c|lrrrr||r|}
\hline
\textbf{\textbf{Task}} & \textbf{\textbf{Dataset}} & \multicolumn{1}{l}{\textsc{all}} & \multicolumn{1}{l}{\textsc{-mlm,rl}} & \multicolumn{1}{l}{\textsc{-rl}} & \multicolumn{1}{l|}{\textsc{-mlm}} & \multicolumn{1}{|c|}{\textsc{te}} \\ \hline
EM-T                   & Abt-Buy                   & 87.45                            & 3.92                                 & 2.96                             & 1.08                               & 5.30                             \\ \hline
EM-T                   & Company                   & 86.38                            & 3.14                                 & 1.97                             & 1.02                               & 2.40                             \\ \hline
EM-S                   & BeerAdvo-RateBeer         & 89.99                            & 2.16                                 & 1.10                             & 1.52                               & 33.75                            \\ \hline
EM-S                   & iTunes-Amazon             & 75.77                            & 1.84                                 & 1.14                             & 1.43                               & inf                              \\ \hline
EM-S                   & Fodors-Zagat              & 86.42                            & 1.46                                 & 1.14                             & 1.33                               & 26.46                            \\ \hline
EM-S                   & DBLP-ACM                  & 98.51                            & 1.07                                 & 1.02                             & 1.01                               & 1.19                             \\ \hline
EM-S                   & amazon-google             & 69.83                            & 1.49                                 & 1.30                             & 1.01                               & 3.85                             \\ \hline
EM-S                   & DBLP-Scholar              & 81.50                            & 1.22                                 & 1.15                             & 0.94                               & 2.74                             \\ \hline
EM-S                   & Walmart-Amazon            & 73.11                            & 1.96                                 & 2.26                             & 1.02                               & 15.56                            \\ \hline
EM-D                   & DBLP-ACM                  & 98.00                            & 1.19                                 & 1.05                             & 1.00                               & 1.33                             \\ \hline
EM-D                   & DBLP-Scholar              & 81.16                            & 1.30                                 & 1.05                             & 0.94                               & 3.20                             \\ \hline
EM-D                   & iTunes-Amazon             & 67.63                            & 1.93                                 & 1.61                             & 1.73                               & 16.15                            \\ \hline
EM-D                   & Walmart-Amazon            & 69.27                            & 3.03                                 & 2.12                             & 1.04                               & 5.96                             \\ \hline
\end{tabular}
\caption{Microbenchmarks evaluating \sys's architecture, reflecting how many times better \sys is compared to: using a pretrained DistilBERT$_{\text{base}}$ model, without representation learning, without MLM pretraining, and when using one encoder for each dataset.}
\label{table:dm_micros}
\end{table}

==> context enrichment 8/tables/micros.tex <==
% \hhline{~~--------------}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|
>{\columncolor[HTML]{FFFFFF}}r rrr
>{\columncolor[HTML]{6FA8DC}}r |r|}
\hline
\multicolumn{8}{|c|}{\cellcolor[HTML]{EFEFEF}\textbf{Recall@1}}                                                                                                                                                                                                                                                                                                                                            \\ \hline
\cellcolor[HTML]{F3F3F3}\textbf{\textbf{Task}} & \cellcolor[HTML]{F3F3F3}\textbf{\textbf{Dataset}} & \cellcolor[HTML]{F3F3F3}\textbf{{\textsc{-mlm,rl}}} & \cellcolor[HTML]{F3F3F3}\textbf{{\textsc{-rl}}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-ft}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-mlm}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-ns}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{te}} \\ \hline
FJ                                             & IMDb                                              & -53.15\%                                            & \cellcolor[HTML]{A4C8E9}-19.78\%                & \cellcolor[HTML]{AACCEB}-22.25\%              & \cellcolor[HTML]{72AADD}-1.69\%                & -0.84\%                                       & \cellcolor[HTML]{BAD6EF}-28.02\%             \\ \hline
FJ                                             & IMDb-hard                                         & -90.19\%                                            & \cellcolor[HTML]{DCEAF7}-68.29\%                & \cellcolor[HTML]{D4E5F5}-63.31\%              & \cellcolor[HTML]{8EBBE4}-20.54\%               & -1.82\%                                       & \cellcolor[HTML]{AFCFEC}-41.02\%             \\ \hline
QA                                             & SQuAD                                             & \cellcolor[HTML]{FAFCFE}-78.5\%                     & \cellcolor[HTML]{FFFFFF}-81.88\%                   & \cellcolor[HTML]{E6F0F9}-67.09\%              & \cellcolor[HTML]{6FA8DC}3.2\%                  & \cellcolor[HTML]{8EBBE4}-14.72\%              & \cellcolor[HTML]{C6DDF2}-48.08\%             \\ \hline
S                                              & MS MARCO                                          & -99.91\%                                            & \cellcolor[HTML]{E2EEF8}-81.06\%                & \cellcolor[HTML]{DEEBF7}-78.26\%              & \cellcolor[HTML]{6FA8DC}-6.36\%                & \cellcolor[HTML]{94BFE5}-30.32\%              & \cellcolor[HTML]{ADCEEB}-46.34\%             \\ \hline
R                                              & IMDb-wiki                                         & -99.96\%                                            & \cellcolor[HTML]{FEFEFF}-98.79\%                & \cellcolor[HTML]{F8FBFE}-94.88\%              & \cellcolor[HTML]{78AEDF}-6.66\%                & -0.75\%                                       & \cellcolor[HTML]{FEFFFF}-99.\%               \\ \hline
EM-T                                           & Average All                                       & -90.43\%                                            & \cellcolor[HTML]{F0F6FC}-80.98\%                & \cellcolor[HTML]{EBF3FB}-78.25\%              & \cellcolor[HTML]{75ACDE}-7.75\%                & -4.59\%                                       & \cellcolor[HTML]{FBFDFE}-87.8\%              \\ \hline
EM-S                                           & Average All                                       & \cellcolor[HTML]{BFD9F0}-49.51\%                    & \cellcolor[HTML]{8FBBE4}-24.07\%                & \cellcolor[HTML]{92BEE5}-25.9\%               & \cellcolor[HTML]{6FA8DC}-7.47\%                & \cellcolor[HTML]{72AADD}-9.02\%               & \cellcolor[HTML]{FFFFFF}-83.47\%                \\ \hline
EM-D                                           & Average All                                       & \cellcolor[HTML]{D6E6F5}-54.01\%                    & \cellcolor[HTML]{A8CBEA}-34.46\%                & \cellcolor[HTML]{A5C9EA}-33.13\%              & \cellcolor[HTML]{6FA8DC}-10.18\%               & \cellcolor[HTML]{7AAFDF}-14.65\%              & \cellcolor[HTML]{FFFFFF}-71.74\%                \\ \hline \hline
\multicolumn{8}{|c|}{\cellcolor[HTML]{EFEFEF}\textbf{Recall@10}}                                                                                                                                                                                                                                                                                                                                           \\ \hline
\cellcolor[HTML]{F3F3F3}\textbf{Task}          & \cellcolor[HTML]{F3F3F3}\textbf{Dataset}          & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-mlm,rl}}   & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-rl}}   & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-ft}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-mlm}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-ns}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{te}} \\ \hline
FJ                                             & IMDb                                              & -30.02\%                                            & \cellcolor[HTML]{9EC4E8}-9.83\%                 & \cellcolor[HTML]{9EC4E8}-9.77\%               & \cellcolor[HTML]{70A9DD}-0.39\%                & -0.25\%                                       & \cellcolor[HTML]{84B5E2}-4.54\%              \\ \hline
FJ                                             & IMDb-hard                                         & -78.54\%                                            & \cellcolor[HTML]{D3E4F5}-54.26\%                & \cellcolor[HTML]{B9D5EE}-40.1\%               & \cellcolor[HTML]{78AEDF}-5.17\%                & -0.52\%                                       & \cellcolor[HTML]{80B3E1}-9.52\%              \\ \hline
QA                                             & SQuAD                                             & \cellcolor[HTML]{E9F2FA}-65.71\%                    & \cellcolor[HTML]{FFFFFF}-78.28\%                   & \cellcolor[HTML]{D6E6F5}-54.89\%              & \cellcolor[HTML]{6FA8DC}2.29\%                 & \cellcolor[HTML]{7CB0E0}-4.64\%               & \cellcolor[HTML]{A0C6E8}-24.6\%              \\ \hline
S                                              & MS MARCO                                          & -99.79\%                                            & \cellcolor[HTML]{DAE9F6}-75.02\%                & \cellcolor[HTML]{D5E6F5}-71.74\%              & \cellcolor[HTML]{6FA8DC}-4.85\%                & \cellcolor[HTML]{89B8E3}-21.8\%               & \cellcolor[HTML]{A1C6E9}-37.48\%             \\ \hline
R                                              & IMDb-wiki                                         & -99.74\%                                            & \cellcolor[HTML]{FAFCFE}-95.76\%                & \cellcolor[HTML]{E4EFF9}-80.58\%              & \cellcolor[HTML]{73ABDD}-2.54\%                & 0.03\%                                        & \cellcolor[HTML]{F7FAFD}-93.8\%              \\ \hline
EM-T                                           & Average All                                       & -74.24\%                                            & \cellcolor[HTML]{D6E7F6}-51.34\%                & \cellcolor[HTML]{D1E4F4}-48.41\%              & \cellcolor[HTML]{7FB2E0}-2.74\%                & 6.11\%                                        & \cellcolor[HTML]{E4EFF9}-58.91\%             \\ \hline
EM-S                                           & Average All                                       & \cellcolor[HTML]{C0D9F0}-42.73\%                    & \cellcolor[HTML]{89B8E3}-15.41\%                & \cellcolor[HTML]{8EBBE4}-17.89\%              & \cellcolor[HTML]{73ABDD}-4.77\%                & -2.9\%                                        & \cellcolor[HTML]{FFFFFF}-74.11\%                \\ \hline
EM-D                                           & Average All                                       & \cellcolor[HTML]{E6F0F9}-53.54\%                    & \cellcolor[HTML]{A1C6E8}-26.12\%                & \cellcolor[HTML]{A0C6E8}-26.04\%              & \cellcolor[HTML]{82B4E1}-13.93\%               & -6.7\%                                        & \cellcolor[HTML]{FFFFFF}-63.57\%                \\ \hline
\end{tabular}%
}
\caption{%Microbenchmarks evaluating \sys's architecture. 
Microbenchmarks reflecting the percent difference from the default architecture (Table~\ref{tab:baselines}) compared to: a pretrained DistilBERT$_{\text{base}}$ model without representation learning (\textsc{-mlm,rl}), MLM pretraining without RL (\textsc{-rl}), RL with no Transformer fine tuning (\textsc{-ft}), RL with no MLM pretraining (\textsc{-mlm}), no hard negative sampling (\textsc{-ns}), and one encoder per dataset (\textsc{te}). Better results within each row are darker.}
\label{table:micros}
\end{table}

==> context enrichment 8/tables/retrieval.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|l|cc|cc|cc|}
\hline
\textbf{Task}          & \textbf{Dataset} & \multicolumn{2}{c|}{Ret@1} & \multicolumn{2}{c|}{Ret@10} & \multicolumn{2}{c|}{MRR@10} \\ \cline{3-8} 
\multicolumn{1}{|l|}{} &                  & BM25         & \textsc{Emb}        & BM25         & \textsc{Emb}          & BM25         & \textsc{Emb}          \\ \hline
FJ                     & IMDb             &     86.35         &      95.06       &      91.27        &       99.02       &      0.879        &      0.965        \\ \hline
FJ                     & IMDb-hard        &     64.44         &      91.19       &      74.12        &       98.43       &      0.676        &      0.938        \\ \hline
QA                     & SQuAD            &     53.34         &      59.34      &      71.53        &       84.84       &      0.593        &       0.679      \\ \hline
S                      & MS MARCO         &     -             &     16.62        &     -             &      44.76        &     0.167        &      0.249        \\ \hline
R                      & IMDb-wiki-join   &     63.25         &     96.44        &      96.25        &      98.92        &      0.771        &      0.973        \\ \hline
\end{tabular}}
\caption{End-to-end performance of \sys compared to using BM25 after the preprocessing step.}
\label{table:retrieval}
\end{table}

==> context enrichment 8/tables/types.tex <==
\begin{table}[]
\small
\begin{tabular}{lll}
\hline
\textbf{Data Types}                                                                                                                                              &                                                                                                                                                                                                                                                                                                                                                                                                               &                                                                                            \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}\texttt{record}\\ \texttt{sentence}\\ \texttt{embedding}\end{tabular}}                                                             & \begin{tabular}[c]{@{}l@{}}\texttt{Dict[str, Union[str, int, float]]}\\ \texttt{str}\\ \texttt{List[float]}\end{tabular}                                                                                                                                                                                                                                                                                      &                                                                                            \\ \hline
\textbf{Operators}                                                                                                                                               &                                                                                                                                                                                                                                                                                                                                                                                                               & \multicolumn{1}{c}{\textbf{Step}}                                                          \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}\texttt{preparer}\\ \texttt{labeler}\\ \texttt{sampler}\\ \texttt{loss}\\ \\ \texttt{encoder} \\ \texttt{retriever}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\texttt{record \textrightarrow{} sentence}\\ \texttt{Tuple[record, record] \textrightarrow{} bool}\\ \texttt{List[Generic[T]] \textrightarrow{} Generic[T]}\\ \texttt{Tuple[emb., Union[emb.,} \\ \hspace{1.75cm} Tuple[emb., emb.]]] \texttt{\textrightarrow{} float}\\ \texttt{sentence \textrightarrow{} embedding}\\ \texttt{List[emb.] \textrightarrow{} List[Tuple[record, emb.]]}\end{tabular} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1\\ 1, 2\\ 2\\ 1, 2\\ \\ 1, 2 \\ 3\end{tabular}} \\ \hline
\end{tabular}
\caption{ \sys data types and operators used in each step}
\label{table:types}
\vspace{-1em}
\end{table}

==> grave.tex <==


%\red{[Structured data has hobbled along compared to unstructured data.]}
%Machine learning (ML) systems increasingly power critical applications spanning search, recommendation, and question answering~\citep{ml1, ml2, ml3}. 
%However, this ML revolution has largely influenced unstructured data, such as image, video, and natural language.
Machine learning (ML) systems thrive on context-rich information: methods to extract structural and semantic context from images~\citep{alexnet} and text~\citep{bert, gpt2} revolutionized computer vision and natural language processing tasks such as object detection and translation. 

%in computer vision, an image contains most of the context required to perform classification tasks, and in natural language processing, unsupervised textual data sources contain context that can be extracted using Transformers~\citep{transformers}, which has revolutionized tasks such as text generation and translation~\citep{bert,gpt2}.

\begin{figure}
\includegraphics[width=\columnwidth]{figures/tables.pdf}
\caption{An end-to-end task requiring context enrichment. Predicting the rating of and recommending a new product (\texttt{A82}), requires relating the Asics products (highlighted in dark gray) via a keyless join (top). This process is manual due to data heterogeneity---we aim to automate it (bottom).}
\label{fig:example}
\vspace{-1em}
\end{figure}

Unfortunately, structured data repositories, which consist of datasets with pre-defined schemas, suffer from context fragmentation: they commonly scatter information regarding a data record across domain-specific datasets with potentially unique schemas.
These datasets adhere to fixed schemas that are optimized for task-specific querying, and often lack explicit linking keys, such as primary key-foreign key (KFK) relationships.
This constrains users to a single view of an entity that is specialized for a specific business need. 
For instance, in Figure~\ref{fig:example}B, information regarding \textsc{Asics} shoes is scattered across three catalogs with unique schemas. 

Associating these fragmented data contexts is critical in enabling ML-powered applications over structured datasets---a process we denote as \emph{context enrichment}.
While modern, no-code ML systems are rapidly shifting practitioners towards higher-level abstractions for developing ML applications~\citep{ludwig, overton, h20, robot,gcloud}, context enrichment is still left as a user-performed data preparation step.\footnote{https://cloud.google.com/automl-tables/docs/prepare}
Consequently, engineers develop solutions for context enrichment tailored to their domain, such as similarity-based blocking in data integration~\citep{blocking}, retriever models in question answering~\citep{retriever}, or retrieval functions in search~\citep{bm25} (see Section~\ref{sec:applications}). 
However, constructing independent solutions is repetitive, time-consuming, and results in a complicated landscape of overlapping, domain-specific methods.
For instance, consider the scenario depicted in Figure~\ref{fig:example}:

%As a result, performing \emph{context enrichment}, or associating fragmented data contexts, is a pervasive need across a wide spectrum of ML-powered applications that operate over structured datasets, including recommendation, search, question answering, and data integration. 
%While modern no-code ML systems support the end-application given curated datasets, they leave context enrichment as a user-performed feature engineering step\footnote{https://cloud.google.com/automl-tables/docs/prepare}~\citep{ludwig, overton, gcloud}.
%Consequently, each vertical must construct independent, domain-specific solutions for their applications, which is time-consuming and repetitive.
%For instance, consider the following scenario (Figure~\ref{fig:example}):


\eat{
%Structured data repositories (i.e., data stores with a pre-defined schema) scatter context, or information regarding an entity or data record, across domain-specific datasets of differing schema.
%These datasets adhere to fixed schemas that are optimized for task-specific querying and manipulation, which constrains users to a single view of an entity that is specialized to a vertical or business need. 

%Context fragmentation is at odds with machine learning (ML) systems that thrive given context-rich features, as is typical of unstructured data: an image contains most of the context required to perform an image classification task, and leveraging context from unsupervised textual data sources via Transformers~\citep{transformers} revolutionized natural language processing~\citep{bert,gpt2}. 
%Thus, associating fragmented data contexts prior to performing downstream tasks, a process we refer to as \emph{context enrichment}, is a common and critical step to enable end-to-end ML systems for structured data.

%For instance, consider the following scenario (Figure~\ref{fig:example}):


%Machine learning (ML) systems have revolutionized applications over unstructured data, such as image, video, and natural language~\citep{ml1,ml2,ml3}.
%\emph{Structured} data (i.e., with a pre-defined schema) has not experienced the same success despite its prevalence~\citep{lakehouse}, largely due to context fragmentation.


%\red{[This disparity is because of a lack of context and datasets.]} \\
%A core reason for this disparity is that structured datasets scatter information regarding an entity or data point (i.e., \emph{context}) across numerous domain-specific datasets of differing schema.
%As these datasets are optimized for querying and manipulation, not ML, they adhere to fixed schemas, which constrain users to a single view of an entity that is specialized to a vertical or business needs. 
%As a result, information regarding an entity or data point (i.e., \emph{context}), is fragmented across numerous domain-specific datasets of differing schema, often with an unclear means of joining them~\citep{arda}.
%This fragmentation is at odds with ML models that thrive given abundant context-rich information, as is typical of unstructured data: a single image contains most of the context required to perform an image classification task, and leveraging context from unsupervised textual data sources via transformers~\citep{transformers} revolutionized natural language processing~\citep{bert,gpt2}. 


%\red{[We need to associate these contexts to enable ML]} \\
%Associating these fragmented data contexts prior to performing downstream tasks, a process we refer to as \emph{context enrichment}, is key to enabling the next-generation of ML systems for structured data.
%For instance, consider the following scenario (Figure~\ref{fig:example}):
%A natural question that arises is, how can we associate disparate information sources for the same real-world entity (e.g., product), to enable the next-generation of data analytics platforms? 
}
%\vspace{5pt}
\vspace{-7pt}
\emph{\\An e-commerce company has a proprietary product catalog, and aggregates product information from several external vendors to perform market analysis. 
Each vendor uses a unique product catalog, each with unique product representations (i.e., schema) ranging from free-form text to tabular product descriptions; products may overlap and evolve (Figure~\ref{fig:example}B).
Given normalized tables containing user and rating data, an engineer wishes to estimate the rating for a candidate new product (\texttt{A82}) and identify users to recommend the product to (Figure~\ref{fig:example}A).
%While the company has labeled a small number of product matches across the different catalogs, no global product identifier exists as a unifying join key.
%The engineer must join products across catalogs, and display those relevant to the user.
}
\vspace{5pt}


The engineer must first perform context enrichment by joining information across tables to extract features that capture similarities between the new (\texttt{A82}) and existing (\texttt{A80}, \texttt{P8}) products.
The engineer can then estimate the product rating, and recommend the new product to users based on how they rated related products.


The classic data management approach is to denormalize datasets using KFK joins. 
However, not all tables can be joined when relying on only KFK relationships.
For instance, there is no KFK relationship between Catalog B and Catalogs A or C; no join key unites fundamentally disparate product catalogs. 
Even when KFK relationships exist, as between Catalogs A and C (\textsc{\texttt{ITEM}}), relying on just KFK semantics will fail to capture the similarity between \texttt{A82} and \texttt{A80}.
The engineer must realize that the \texttt{Description} column in Catalog A relates to the \texttt{Brand} and \texttt{Model} columns in Catalog B and the \texttt{Size}, \texttt{Make}, and \texttt{Color} columns in Catalog C, and then perform a custom similarity-based join depending on the two tables---e.g., a join based on Jaccard similarity or Levenshtein distance.
%The engineer must perform this join for all modified products, and may have to repeat this entire procedure as catalogs evolve. 
As database semantics do not natively support \emph{keyless joins} that require similarity-based indexing, joining arbitrary catalogs remains heavily manual---even large companies rely on vendors to categorize listings, which results in duplicate listings.\footnote{https://sell.amazon.com/sell.html}
No out-of-the-box query interface allows users to surface the relatedness between \texttt{A80}, \texttt{A82}, and \texttt{P8} (all \texttt{Asics}, two \texttt{GT-1000}, and two \texttt{blue}), and link these records to the Ratings table with minimal intervention. 

To combat this tedious context enrichment process, we evaluate how to bring recent no-code semantics from ML systems such as Ludwig~\citep{ludwig}, H20.ai~\citep{h20}, and Data Robot~\citep{robot} to context enrichment.
The challenge in developing a no-code context enrichment system is to construct an architecture that is simultaneously:
\begin{enumerate}
    \item \textbf{General}: Applicable to a wide variety of tasks and domains.
    %\item \textbf{Query-time Scalability}: Efficiently queries new data.
    \item \textbf{Extensibile}: Customizable for domain or downstream needs.
    \item \textbf{Low Effort}: Usable with minimal configuration.
\end{enumerate}

We propose \sys, a no-code context enrichment framework that provides these three functionalities.
\sys's architecture generalizes across a variety of tasks, and is easily customized using a high-level configuration file.
As input, users provide a base data source, an auxiliary data source, and a set of examples of related records across the sources (Figure~\ref{fig:overview}).
For each record in the base data source, \sys returns related records from the auxiliary data source as characterized by the examples, which can be post-processed for downstream tasks (e.g., concatenated or averaged).

\sys's key insight is to simplify context enrichment by abstracting an interface that performs a new class of join: a \textit{learned keyless join} that operates over record-level similarity. 
Just as traditional database joins provide an abstraction layer for combining structured data sources given KFK relationships, we propose formalizing keyless joins as an abstraction layer for context enrichment.

\sys implements a keyless join abstraction layer by constructing an index populated with task-specific embeddings.
Drawing inspiration from successes in applying Transformers~\citep{transformers,bert} to structured datasets~\citep{tabert,neuraldb}, we rely on Transformers as building blocks for embedding generation. 
%Unlike KFK joins that operate at the schema-level, keyless joins must consider record-level similarities to identify if records from different tables are related---not the similarities of specific column values to identify exact matches.
%Advances in Transformer-based encoders applied to structured datasets can power a general method to identify contextually similar records. 
We present a three-step system architecture that enables index construction via Transformer-based embeddings: preprocessing, representation learning, and joining.

%The resulting research challenge is in exploring the design space to determine the system architecture and operators required to enable context enrichment via keyless joins across domains spanning recommendation, search, question answering, and data integration.

\eat{
%While modern no-code ML systems support downstream workloads, they treat context enrichment as a user-performed feature engineering step~\cite{ludwig, overton}. 
%When developing such ML systems for structured data, we realized that this procedure for context enrichment can be simplified via the introduction of a new class of join: a \emph{keyless} join that performs a join based on data point similarity. 

%When developing such ML systems for structured data, we realized that the need for context enrichment is pervasive across a wide spectrum of downstream applications including recommendation (as above), search, question answering, and data integration. 
%However, each vertical constructs an independent, domain-specific solution for these tasks, which is time-consuming and repetitive.
%While modern no-code ML systems support the end-application, they treat this context enrichment as a user-performed feature engineering step~\citep{ludwig, overton}.
%As a result, enrichment remains tedious, requiring domain-specific techniques.
%Consequently, in this paper, we evaluate if is it possible to develop a scalable and general context enrichment system that can be applied across all of these workloads with no code modifications.
}

%A system that implements a scalable and general keyless join enrichment layer must address three design decisions. 


%In this paper, we propose \sys, a no-code context enrichment framework that implements these three elements.
%As input to \sys's default architecture, users provide a base data source, an auxiliary data source, and a set of examples of related records across the two sources (Figure~\ref{fig:overview}).
%For each record in the base data source, \sys returns the most related records from the auxiliary data source.
%These outputs can then be post-processed for downstream tasks (e.g., concatenated or averaged).
%We introduce both \sys's high level architecture and the implementation of \sys's default operator configuration to demonstrate how a single system can generalize to all of our target workloads by changing a high-level configuration file. 
%workloads spanning recommendation (as in Figure~\ref{fig:example}), search, entity matching, fuzzy joins, and question answering by changing a high-level configuration file. 

\eat{
\begin{figure}
\includegraphics[width=\columnwidth]{figures/Categorization.pdf}
\caption{}
\label{fig:categories}
\vspace{-1em}
\end{figure}
}


\eat{
%The key insight behind \sys is that new Transformer-based methods for embedding generation~\citep{transformers,bert} can serve as the building blocks for a no-code keyless join enrichment layer. 
%Keyless joins must operate at the record-level, unlike KFK joins that operate at the schema-level. 
%As a result, \sys must consider record-level similarities to identify if records from different tables are related---rather than considering the similarities of specific column values to identify exact matches.
%By building off recent advances in Transformer-based encoders applied to records in structured datasets, we provide a general method to identify contextually similar entities. 
%At a high-level, \sys provides an interface for keyless joins by constructing an index that is populated with task-specific embeddings.
%To enable this functionality, we propose a three-step system architecture: preprocessing, representation learning, and joining.


%that we can simplify context enrichment by defining and and abstracting this new class of join: a \emph{keyless} join that performs a join based on record similarity. 
%Just as traditional database joins provide an abstraction layer for combining structured data sources given KFK relationships, we propose keyless joins as an abstraction layer for context enrichment (Figure~\ref{fig:categories}).


%In this paper, we evaluate how to develop a general context enrichment system that requires no code modification.  
%We show how abstracting keyless joins as a fundamental primitive for context enrichment can help achieve this goal.
%close the loop for developing simple, no-code ML pipelines over structured data. 
%The resulting research challenge is in exploring the design space to determine the architecture and abstractions required to enable general keyless joins. 
%In response, we propose \sys, a no-code context enrichment framework.


%As input to \sys's default architecture, users simply provide a base data source, an auxiliary data source, and a small set of examples of related records across the two sources (Figure~\ref{fig:overview}.
%For each record in the base data source, \sys then returns the most related records from the auxiliary data source.
%These outputs can then be processed for use in a downstream task (e.g., concatenated or averaged).

%We develop \sys as a no-code framework for context enrichment to demonstrate that keyless joins enable generalization to workloads spanning search, entity matching, fuzzy joins, question answering, and recommendation (as in Figure~\ref{fig:example}) by only changing a high-level configuration file. 
%When using \sys's default architecture and operators, users simply provide a base data source, an auxiliary data source, and a small set of examples of related records across the two sources.
%For each record in the base data source, \sys then returns the most related records from the auxiliary data source.
%These outputs can then be processed for use in a downstream task (e.g., concatenated or averaged).

%The key insight behind \sys is that new Transformer-based methods for embedding generation~\citep{transformers,bert} can serve as the building blocks for a no-code keyless join enrichment layer. 
%Keyless joins must operate at the record-level, unlike KFK joins that operate at the schema-level. 
%As a result, \sys must consider record-level similarities to identify if records from different tables are related---rather than considering the similarities of specific column values to identify exact matches.
%By building off recent advances in Transformer-based encoders applied to records in structured datasets, we provide a general method to identify contextually similar entities. 
%At a high-level, \sys provides an interface for keyless joins by constructing an index that is populated with task-specific embeddings.
%To enable this functionality, we propose a three-step system architecture: preprocessing, representation learning, and joining.
}

%We identify three elements that a system must provide to implement a general keyless join enrichment layer.
%First, the system must represent records from different data sources in a comparable format regardless of schema.
%Second, these representations must be automatically tuned to identify contextually similar records as defined by a downstream application. 
%Finally, similar records must be quickly retrieved using the tuned representations. 


\minihead{Preprocessing} \sys transforms records from different data sources to a common representation, which allows us to apply the same methods across tasks to enable generality (1). 
%We answer: how can we represent records from different sources in a comparable format?
Although classic means of representing structured data often focused on integer encoding, Transformer-based encoders such as BERT and GPT have demonstrated success across data types including structured data~\citep{tabert,neuraldb}.
Thus, by default, \sys represents each record as a natural language sentence for input to a Transformer-based encoder, which we optionally pretrain using self-supervision.
%Building off this recent success, by default, \sys represents each record as a natural language sentence consisting of the column names and values in key-value format for input to a Transformer-based encoder.
We demonstrate that depending on the data vocabulary, encoder pretraining to bootstrap the pipeline with domain knowledge can increase recall of retrieved relevant records by up to \red{24\%}. 

\begin{figure}
\includegraphics[width=\columnwidth]{figures/overview.pdf}
\caption{\sys's interface for context enrichment. \sys retrieves related auxiliary records for each base record.}
\label{fig:overview}
\vspace{-1em}
\end{figure}

\minihead{Representation Learning} \sys automatically tunes the representations from the first step to identify contextually similar records as defined by a downstream application to improve ease-of-use (3).
Learning this representation is task-dependent: we show that a natural first approach of using pretrained Transformer-based embeddings (e.g., BERT) with no fine-tuning performs up to three orders of magnitude worse than a fine-tuned approach, often returning less than \red{10\%} of relevant records.  
%orders of magnitude worse than standard information retrieval methods (i.e., BM25); learning a representation to reflect relatedness is task-dependent.
Domain-specific pretraining in the first step can increase recall by over \red{30\%}, but this is still insufficient in isolation.
Thus, \sys relies on supervised examples of related records and a contrastive triplet loss~\citep{tripletloss} to learn a representation that encourages similar records to be close while pushing away dissimilar records in the induced embedding space. 
We evaluate how many labeled examples are required to match the performance of using all provided examples, and find that at times, \red{1\%} of the labels is sufficient, and that operators for automatic hard negative sampling improve performance by up to \red{25\%} recall.
%\sys provides negative sampling utilities to sample unrelated records, should a user only provide examples of related records.

\minihead{Joining} \sys quickly retrieves related records using the tuned representations to perform the keyless join.
%We answer: how can we quickly compare and identify related records?
A na\"ive means of identifying similar records would require exhaustive pairwise comparison of potentially joinable records.
However, this procedure scales quadratically with the number of considered records. 
While similarity-based join techniques as in data blocking~\citep{blocking} also aim to identify related records for a given base record, we show that the best method with respect to recall is domain-specific.
As we learned an embedding space to capture record similarity in the second step, \sys can instead populate an index with the learned embeddings, and use optimized maximum inner product search (MIPS) to identify the nearest neighbors of a given record.
This procedure allows \sys to capture one-to-one and one-to-many join semantics across a variety of downstream applications with low query-time overhead.
We demonstrate that \sys meets or exceeds the performance of seven similarity-based join baselines including BM25~\citep{bm25}, jaccard-similarity-based joins, and Levenshtein distance-based joins with respect to recall and query runtime.   

%We answer: what architecture and supervision is required to learn a representation where contextually similar records are close together in embedding space?
%As previously noted, we rely on Transformer-based encoders.
%While a na\"ive encoder architecture may train independent encoders for each data source, we find that for our context enrichment tasks, using a single encoder performs best.
%With respect to supervision, we demonstrate the leveraging pretrained BERT embeddings with no supervised fine-tuning performs orders of magnitude worse than standard information retrieval methods (i.e., BM25); learning a representation to reflect relatedness is task-dependent.
%While domain-specific pretraining in the preprocessing step helps bridge this gap, it is still insufficient in isolation.
%Thus, \sys instead uses supervised examples of related and unrelated records in this step.
%By default, \sys uses a contrastive triplet loss~\citep{tripletloss} to learn a representation; the triplet loss encourages similar records to be close and pushes away dissimilar records under the induced embedding space. 
%\sys provides negative sampling utilities to sample unrelated records, should a user only provide examples of related records.

%In the joining step, we perform the keyless join.
%We answer: how can we quickly compare and identify related records?
%A classic means of identifying similar records would require exhaustive comparison between all pairs of potentially joinable records (either the entire dataset, or a set of candidate records or a data block)~\citep{}.
%However, this procedure scales quadratically with the number of records considered. 
%As we are working in embedding space that has been tuned to capture record similarity, \sys can instead push the similarity check to the final pipeline step. 
%\sys populates an index with the learned embeddings, and uses optimized maximum inner product search (MIPS) to identify the nearest neighbors of a given record in the embedding space.

Although conventional wisdom in data management often says to rely on domain-specific pipelines for context enrichment, we introduce no-code ML semantics to context enrichment and empirically show how a single system can generalize to heterogeneous downstream tasks, providing extensibility (2).
We report on our experiences in deploying \sys across five tasks: fuzzy joining, entity matching, question answering, search, and recommendation.
We demonstrate that \sys generalizes to each, requires as little as a single line configuration change, and extends to downstream similarity-based analyses for search, entity matching, and recommendation as in Figure~\ref{fig:example}. 

In summary, we present the following contributions in this paper:

\begin{itemize}
    \setlength\itemsep{.75em}
    \item We propose keyless joins as a new abstraction layer for context enrichment. To our knowledge, this is the first work to abstract and generalize similarity-based tasks across data integration, natural language processing, search, and recommendation as a data management problem.
    \item We design and develop \sys, the first no-code framework for context enrichment that implements keyless joins.
    \item We empirically demonstrate that \sys generalizes to five workloads by meeting or exceeding the recall of baselines with fewer than 5 lines of configuration changes, and evaluate the design of \sys's default architecture.
\end{itemize}












































%\red{[similarity search + downstream; too short and redundant with previous?]} \\
%Finally, given the fine-tuned model, \sys identifies data points that should be joined using an optimized routine for maximum inner product search~\citep{faiss}.
%By pushing the similarity check to the final step of the architecture, \sys eliminates the costly quadratic comparison needed by classic systems~\citep{}. 
%The outputs of \sys can either be directly used by a downstream task with similar records concatenated or averaged, or the representation in the original data sources can be directly used.

\eat{
%Methods for automated machine learning (AML) that integrate ML and data processing have become increasingly prevalent~\citep{seehamlet} as machine learning (ML) now powers a wide variety of data-driven applications such as search, ranking, and query answering~\citep{randomstuff}.
%These methods typically assume that data is obtained from a single source (e.g., a single database table, or an collection of text records), or that there exists a join key that connects multiple normalized data sources to one another either directly or via simple preprocessing (e.g., aggregation or interpolation)~\citep{hamlet,arda}. 
%However, when a single data source is not sufficiently informative for a given task, the sources that users may wish to augment their data with provide different, yet overlapping views of the same underlying information, where no explicit join key can be used to unite the data sources. 
}
\eat{
Rising data volumes in conjunction with human processing and labeling efforts have resulted in unprecedented amounts of task-specific, high-fidelity\eat{supervised and unsupervised} training data.
This data has enabled machine learning (ML) systems to power a wide array of critical applications spanning search, recommendation, and question answering~\citep{ml1, ml2, ml3}. 
However, as our demand for ML-powered applications grows, it becomes infeasible to develop and process task-specific datasets from scratch~\citep{snorkel,crossmodal}.
As a result, a single dataset may not be sufficient in isolation for a given task~\citep{arda}.
We must instead leverage a combination of heterogeneous, potentially overlapping datasets that have been generated and stored for other uses~\citep{lakehouse,gpt2}. For instance, consider the following scenario:
}
\eat{
%Great training data has enabled ML to power a huge array of cool things.  % maybe instead make a sell here about attention and training data/processing not meeting pace with it %todo: establigh the heterogeneity and overlappingness of these datasets
%As the space grows, we find that oftentimes a single dataset is not used in isolation---either due to collecting data to improve improve model performance by leveraging additional information to enrich the input training data or as a result of an increasing ecosystem of collected data that can be leveraged.  
}
\eat{
\vspace{5pt}
\emph{An e-commerce company operates a store that sources products from several vendors. Each vendor provides a unique product catalog, where catalogs may overlap and evolve based on supplier inventory.  
An ML engineer at this company wishes to display the most relevant shopping results for a user given their purchase history.
Catalogs have unique product representations (i.e., schema) ranging from free-form text to highly-structured tabular product descriptions. 
While the company has labeled a small number of product matches across the different catalogs, no global product identifier exists as a unifying join key.
Thus, the engineer must develop a system to join products across the catalogs, and display the most relevant products for a user's query.}\vspace{5pt}

We refer to the process of joining datasets that are heterogeneous yet overlapping in information as \emph{context enrichment}, where multiple auxiliary data sources (e.g., product catalogs) are combined to augment, or enrich, a base data source (e.g., the e-commerce company's global product list).
Although similar to existing problems in data augmentation~\citep{dataaug} or management~\citep{arda,hamlet,hamletpp,tableunion}, existing methods assume that practitioners operate over either a single data source, or can learn explicit join keys to unite multiple data sources.
In contrast, context enrichment is tailored to the rising class of data-intensive workloads that manage multiple data sources without such join keys, as present in data lakes~\citep{lakehouse}.
These workloads span both classic data management, (e.g., data integration, information retrieval, relational data augmentation, fuzzy joining) and machine learning (e.g., entity disambiguation, question answering, multi-hop question answering). 
As our data ecosystems and need for data-driven applications continue to grow, we require scalable systems for context enrichment to power the next generation of data analytics and ML platforms. 
}

\eat{
In response, we introduce the \enrich operator, a declarative relational operator that performs context enrichment.
Given a base and auxiliary data sources, the \enrich operator identifies data points in the auxiliary sources that share context with the base data source, and returns the joined result. 
Rather than relying on information solely present in each column to join datasets, \enrich instead learns a representation for each data point such that their distance in the induced embedding space reflects their similarity to one another \reword{for use in a downstream workload}. 
To enable scalable, generalizable context enrichment, the \enrich operator overcomes two key bottlenecks: human attention and computational resources. 
}
\eat{
First, as human attention is fundamentally limited compared to computational and storage capacity~\citep{mbcidr}, a system for general context enrichment cannot rely on excessive human supervision and processing for \emph{each} join that must be performed.
Typical automated means for identifying candidate matches across datasets require large amounts of supervised training data (i.e., examples of matching and not matching data points) to train an ML model~\citep{deepmatcher}.
The \enrich operator instead leverages recent advances in self-supervised learning and transformer models in natural language processing to alleviate this need.  
We first represent each data source's data points as natural language sentences, which enables us to represent heterogeneous textual and numeric data sources with a shared vocabulary.
We then automatically identify similar data points using unsupervised ranking from information retrieval (i.e., BM25), and use these data points to perform pre-training via masked language modeling to bootstrap a transformer model.
This pre-training step enables us to use a small subset of labeled examples to fine-tune our data representation.
}
\eat{
Second, as data volumes rapidly grow, a system for context enrichment must scale with an increasing number of large, heterogeneous datasets.
A na\"ive yet classic means of identifying similar data points would require exhaustive comparison between all pairs of potentially joinable data points (either the entire dataset, or a set of candidate data points or a data block).
However, this procedure scales quadratically with the number of data points considered. 
The \enrich operator instead scales to large data volumes by learning a representation over which maximum inner product search identifies related records across heterogeneous data sources.
We use a small subset of labeled data points to fine-tune the representation learned from the pre-training step using a contrastive loss~\citep{tripletloss}, so similar data points are close to one another in the embedding space induced by the representation.
Given this representation, we can identify data points that should be joined using an optimized routine for maximum inner product search~\citep{faiss}.
}
\eat{
%The \enrich operator addresses the scaling challenges across people, machine, and application as follows. 
%To realize this opportunity, a system for context enrichment must overcome three \reword{bottlenecks} in uniting heterogeneous datasets for an end-task: human attention, computational resources, and \reword{diversity of target application.} 
%First, as human attention is fundamentally limited compared to computational and storage capacity~\citep{mbcidr}, a system for context enrichment cannot rely on excessive human supervision for each join.
%Second, as data volumes rapidly grow, a system for context enrichment must scale with increasing number of heterogeneous datasets and their size.
%Finally, as target applications diversify, a system for context enrichment must provide a generalizable architecture and interface amenable for reuse.


%First, the \enrich operator reduces the need for human supervision by leveraging recent advances in self-supervised learning and attention in natural language processing. 
%We instead first represent each data point as a natural language sentence, and automatically identify candidate similar data points using unsupervised ranking from information retrieval (i.e., BM25). 
%We use these candidate data points to perform pre-training via masked language modeling to bootstrap a transformer model.
%This pre-training step enables us to then use a small subset of labeled examples to fine-tune our data representation.

%Second, the \enrich operator scales to large data volumes by learning a representation over which maximum inner product search identifies related records across heterogeneous data sources. 
%A na\"ive yet classic means of identifying similar data points would require exhaustive comparison between all pairs of potentially joinable data points (either the entire dataset, or set of candidate data points or a data block).
%However, this procedure scales quadratically with the number of data points considered. 
%Thus, we instead use the small subset of labeled data points to fine-tune the learned representation above using a contrastive loss~\citep{tripletloss}, where similar data points are close to one another.
%Given this representation, we can identify data points that should be joined using an optimized routine for maximum inner product search~\citep{faiss}.
}
\eat{
% We refer to this procedure as context enrichment, where multiple auxiliary data sources are combined to augment, or enrich, a base table.
%Context enrichment differs from more traditional means of data augmentation as they either operate over a  a single data source/table, or assume the presence of join keys to unite multiple data sources/tables together.
% In particular, these techniques do not address the case where heterogeneous data sources cannot be combined with an explicit join key, but instead consists of overlapping views of related information. 

% Unlike the canonical database join that links multiple data sources, where explicit join keys unite and augment data sources, context enrichment relies on  information that unites these tables are  


%Existing methods that integrate ML and data processing typically ignore this challenge, or assume 




% ML powers a bunch of stuff, so AML that integrates ML and data processing has become increasingly prevalent. 
% This work either only deals with single tables, or assumes the presence of a join key. 
% For example ....
% 


Different types of joins
\begin{enumerate}
    \item Joining because mentions are in different namespaces, but same things -- record linkage and dedupe
    \item Joining because you have different entities that have overlap in content or context -- retrieval, predictive, etc
\end{enumerate}


Traditional DB focuses on the first. However, the latter is also huge. But if you don't have primary-key/foreign-key, unfortunately, there is very limited tooling to join things together. 
 
This is a new type of joins that relies on embeddings. 

It appears in question answering, information retrieval, entity disambiguation, etc.


We present BLAH, a new operator that represents these embedding-based joins, and provides a unified interface for enabling such queries. 

bm25 is index creation for the join (can be anything you want; tfidf)

how to connect with traditional join with this 

join by random doesn't work. different columns for each, doesn't work. 
}

%Much of machine learning's success with unstructured data is a result of our ability to extract information relevant to a downstream task from large volumes of \emph{context-rich training data.} 
%For instance, a single image contains most of the context required to perform an image classification task---large supervised image datasets and efficient deep learning architectures to extract this context revolutionized computer vision~\citep{alexnet}. 
%Similarly, the ability to integrate and leverage context from unsupervised textual data sources via transformers~\citep{transformers} revolutionized natural language processing~\citep{bert,gpt2}. 
%On the other hand, structured data suffers from context being scattered across numerous, nonuniform datasets.
%\red{[Structured data's design --> fragmentation; we must overcome]}
%Structured datasets are typically in a form optimized for efficient querying and manipulation---e.g., in normalized form specialized to a single set of business needs. 
%Thus, context for a single data point is split across multiple data sources, which is at odds with ML models that thrive given an abundance of context-rich information.

%While classic solutions for context enrichment often do not apply, newer ML-based methods rely on humans for supervision and to develop custom systems for each enrichment task. 
%The classic data management approach is to denormalize datasets using primary key-foreign key (KFK) joins.
%However, for an increasing number of tasks, as the one above, KFK dependencies are not present.
%Practitioners may alternatively turn to ML-based approaches to join entities across datasets, but this requires large amounts of hand-labeled training data, which is often time-consuming and arduous to collect for each enrichment task~\citep{snorkel}. 
%Finally, even if a team is able to develop a method for effective context enrichment for a given task, they do so in an end-to-end manner~\citep{deepmatcher}.
%As a result, they start from scratch for each new enrichment domain---entity matching (as in the example), information retrieval, fuzzy joins, and even question answering and entity disambiguation.
%The lack of a unified approach to context enrichment leads to redundant solutions that waste human time: the ML engineer in the above example is unlikely to interface directly with the advertising team at the same company, who may encounter similar challenges. 
%\sys instead learns a representation for each data point such that their distance in the induced embedding space reflects their similarity to one another. 
%\sys proceeds in a three-step architecture: pre-training, fine-tuning, joining.





%The outputs of \sys can be configured to be directly used by a downstream task with related data points concatenated or averaged.

%utilizes optimized maximum inner product search (MIPS) to identify the nearest neighbors of a given record in the embedding space.
%By pushing the similarity check to the final step of the architecture, \sys eliminates the costly quadratic comparison needed by classic systems~\citep{}. 
%We show how the outputs of \sys can be used for general similarity-based analysis as in the e-commerce example. 



%The resulting research challenge when developing \sys is determining the architecture and abstractions required to enable no-code keyless joins. 
%In response, we introduce both \sys's high level architecture, as well as the implementation of \sys's default operator configuration. 

%We propose a three-step system architecture: preprocessing, representation learning, and joining.
%First we must process the input datasets of varying schema such that we can apply a general architecture — while the input schema is known, they are heterogenous.

%Performing a keyless join requires computing record similarity for a downstream task, and performing the join based on the computed similarity. 
%In response, we propose a three-step architecture when designing \sys: preprocessing, representation learning, and joining.  
%The goal of the first step is to learn a data representation such that similarity in the induced embedding space is proportional to the data points' relatedness, or similarity for the downstream task. 
%Given the learned representation, the joining step identifies and returns data points that are most similar to one another. 
%In effect, \sys provides an interface for keyless joins by constructing an index that is populated with task-specific embeddings.
%Developing the operators necessary to enable this two-step architecture requires answering three key technical questions. 

%First, how can we represent data points from different sources in a comparable format for the first step? 
%Although classic means of representing structured data has often remained limited to integer encoding, advances in pre-trained transformer-based encoders such as BERT have demonstrated success across many data types, including structured data~\citep{}.
%We \sys relies on these encoders to generate embeddings for each data point by forming sentences using each key-value pair in a data source. 
%While na\"ive approach to leveraging these encoders may seek to train independent encoders for each data source, we find that for our context enrichment tasks, using a single encoding source performs best in practice. 
%Thus, \sys's default configuration is a single BERT encoder, and we provide configuration options to use either multiple encoder modules as part of the first step. 
%We show that using a single encoder performs up to \red{XXX} better. 

%Second, what supervision is required to learn a representation where similar data points are close together in embedding space?
%Learning a representation to reflect relatedness is task dependent.
%As such, \sys requires a small amount of supervised examples of data points that are related and unrelated to a subset of query data points.
%\sys provides negative sampling utilities to sample unrelated data points, should a user be incapable of providing such supervision.
%By default, \sys uses a contrastive triplet loss~\citep{tripletloss} to learn a representation; the triplet loss encourages similar points to be close and pushes away dissimilar points under the induced embedding space. 
%While the loss function used is a configurable parameter, we find that the triplet loss performs well across our tasks, and is the default operator. 
%In addition, for tasks that may benefit from pre-training the encoder module, we provide operators that can leverage either fully supervised or self supervised methods to bootstrap representation learning. 
%We show that self-supervised pre-training can improve the performance of tasks by up to \red{XXX.} 


%Finally, how can we quickly compare data points to identify those that are related to one another in the second step?
%A na\"ive yet classic means of identifying similar data points would require exhaustive comparison between all pairs of potentially joinable data points (either the entire dataset, or a set of candidate data points or a data block).
%However, this procedure scales quadratically with the number of data points considered. 
%As we are working in embedding space that has been tuned to capture data point similarity, \sys instead utilizes optimized maximum inner product search (MIPS) to identify the nearest neighbors of a given data point in the embedding space.
%By pushing the similarity check to the final step of the architecture, \sys eliminates the costly quadratic comparison needed by classic systems~\citep{}. 
%The outputs of \sys can be configured to be directly used by a downstream task with related data points concatenated or averaged.
%We show how the outputs of \sys can be used for general similarity-based analysis as in the e-commerce example. 


%We report on our experiences in applying \sys across \reword{five} different domains. 
%We demonstrate how no-code context enrichment allows users to go from zero-to-one on a variety of target applications by abstracting away previously tedious procedures. In summary, we present the following contributions in this paper:


%Traditional data-intensive workloads that perform context enrichment as an inherent primitive are developed in isolation from one another, and fail to capitalize on advances made in each domain. 
%By developing a unified framework for context enrichment with limited supervision, we provide a system for solving for such tasks \reword{easier than before, with less supervision.} 
\eat{\begin{itemize}
    \setlength\itemsep{.75em}
    \item We propose keyless joins as a new abstraction layer to enable no-code context enrichment.
    \item We design and develop \sys, the first no-code framework that implements the keyless join abstraction layer for context enrichment.
    \item We evaluate \sys's default configuration, and demonstrate that \sys generalizes \reword{five} workloads across domains spanning data systems and natural language processing via a high-level configuration file.
\end{itemize}}


\eat{
%\red{[What's wrong with context enrichment in ML?]} \\
Practitioners may alternatively turn to ML-based approaches to join entities across datasets, but this requires large amounts of hand-labeled training data, which is often time-consuming and arduous to collect for each enrichment task~\citep{snorkel}. 
Even if a team is able to develop a method for effective context enrichment for a given task, they do so in an end-to-end manner~\citep{deepmatcher}.
As a result, they start from scratch for each new enrichment domain---entity matching (as in the example), information retrieval, fuzzy joins, and even question answering and entity disambiguation.
The lack of a unified approach leads to redundant solutions that waste human time: the ML engineer in the above example is unlikely to interface directly with the advertising team at the same company, who may encounter similar challenges. 
Context enrichment requires a generic, unifying operation that processes structured data for ML workloads.


%\red{[Main Idea]} \\
Our key insight to tackle context enrichment---and the need for a generic operator to perform keyless joins---is to leverage the context that we wish to unite to learn a common data representation across tables where data points' distance in the induced embedding space reflects their similarity to one another. 
We can then holistically evaluate and cluster related data points to join datasets rather than relying on information present in a small set of KFK dependencies.




%\red{[our proposal]} \\
To realize this, we propose \sys, a new context enrichment system  that generalizes and optimizes for keyless joins.
Given a base and auxiliary data sources, \sys identifies data points in the auxiliary sources that share context with the base data source, and returns the joined result. 
Just as databases created an abstraction layer for querying structured data, \sys provides an abstraction layer for context enrichment for downstream ML tasks. 
\sys consists of two components.
First, \sys learns a common data representation for the data sources. For generalizability, \sys must perform this step while reducing the amount of training data required compared to learning this representation from scratch.
Second, \sys identifies data points across the data sources that share context with one another.
For scalability, \sys must perform this step without without comparing all possible data points to see if they are a match. 
%\sys provides a \emph{generalizable architecture} that leverages recent advances in self-supervision in natural language processing to \emph{reduce human supervision} by up to \red{XXX} across \red{YYY} tasks.  using recent advances in self-supervision in natural language processing


%\red{[pre-training/fine-tuning to reduce supervision needed]} \\
In the first step, \sys performs self-supervised masked language modeling to pre-train its embedding using context from each data source, followed by a fine-tuning phase to learn the embedding. 
%As human attention is fundamentally limited compared to computational and storage capacity~\citep{mbcidr}, a system for general context enrichment cannot rely on excessive human supervision and processing for \emph{each} join that must be performed.
Typical automated means for identifying candidate matches across datasets require large amounts of supervised training data (i.e., examples of matching and not matching data points) to train an ML model~\citep{deepmatcher}.
\sys instead first represents each data source's data points as natural language sentences, which enables us to represent heterogeneous textual and numeric data sources with a shared vocabulary.
\sys then automatically identifies similar data points using unsupervised ranking from information retrieval (i.e., BM25), and uses these data points to perform pre-training via masked language modeling to bootstrap the parameters of a transformer model.
Finally, \sys fine-tunes the pre-trained transformer model given a set of labeled examples to learn a data representation where similar items are close in the induced embedding space.

%\red{[similarity search + downstream; scales]}
In the second step, \sys identifies data points that should be joined using an optimized routine for maximum inner product search~\citep{faiss} (MIPS).
A na\"ive yet classic means of identifying similar data points would require exhaustive comparison between all pairs of potentially joinable data points (either the entire dataset, or a set of candidate data points or a data block).
However, this procedure scales quadratically with the number of data points considered. 
The \sys instead scales to large data volumes by learning a representation over which maximum inner product search identifies related records across heterogeneous data sources.
We use a small subset of labeled data points to fine-tune a task-specific representation learned from the pre-training step using a contrastive loss~\citep{tripletloss}, so similar data points are close to one another in the embedding space induced by the representation, and can be retrieved via MIPS.
By pushing the similarity check to the final step of the architecture, \sys eliminates the costly quadratic comparison needed by classic systems~\citep{}. 
The outputs of \sys can either be directly used by a downstream task with similar records concatenated or averaged, or the representation in the original data sources can be directly used.

%\red{[results]}
\sys provides a flexible interface for a variety of target applications by providing a generalizable architecture and interface amenable for reuse. 
Context enrichment is a key primitive in several seemingly unrelated tasks spanning: entity matching, entity disambiguation, information retrieval, relational data augmentation, and question answering.
%Traditional data-intensive workloads that perform context enrichment as an inherent primitive are developed in isolation from one another, and fail to capitalize on advances made in each domain. 
By developing a unified framework for context enrichment with limited supervision, we provide a system for solving for such tasks \reword{easier than before, with less supervision.} 
In summary, we present the following contributions:
\begin{itemize}
    \setlength\itemsep{.75em}
    \item We introduce \sys, a system that performs context enrichment given two or more datasets.
    \item We demonstrate how \sys generalizes workloads across data systems and natural language processing to provide a unified interface for tasks relating multiple data sources.
    \item We empirically show that \sys reduces the number of training examples needed for downstream tasks by up to \red{XXX} to maintain performance.
\end{itemize}
}





\eat{



\minihead{Results} We report Retrieval@1, Retrieval@10, and MRR@10 of IMDb and IMDb-hard in Table~\ref{table:retrieval}, computed with the post-processing module described in Section~\ref{case:IR}. 
\sys outperforms BM25, and only drops at most 4 points (in Retrieval@1) in the IMDb versus IMDb-hard tasks, while BM25 degrades by over 20 points. 


\minihead{Results} We report our F1 score on the test set compared to several baselines in Table~\ref{table:dm_all}.
\sys@1 refers to retrieving the top match, and \sys@best refers to retrieving the number of \records that provides the best F1 score, set via validation. 

The first three results columns reflect the numbers reported from the four deep-learning-based solutions from the deepmatcher package, where DM$_\text{SIF}$ refers to their simple aggregate function model,
DM$_\text{RNN}$ refers to their sequence-aware bidirectional RNN model,
DM$_\text{att}$ refers to their sequence alignment model that uses decomposable attention, and DM$_\text{hyb}$ refers to their hybrid sequence-aware model with decomposable attention ~\citep{deepmatcher}, each of which is customized for EM.
DM$_\text{SIF}$ and DM$_\text{RNN}$ are comparable to the previous standard deep learning method for EM, DeepER~\citep{deeper}. 
The fourth results column reflects the numbers reported by the current state-of-the-art deep-learning-based system, Ditto~\citep{ditto}.
Ditto achieves these results using pre-trained language models, with custom optimizations that allow users to tag input text spans, perform sentence summarization for long records, and apply data augmentation to find hard examples.

Without any such optimizations, \sys@best provides results within 2 F1 points of Ditto in 3 tasks, outperforms at least one other custom deep-learning-based solution on 10 of the 13 tasks, and outperforms all but Ditto on 5 tasks  (underperforming compared to DM$_\text{hyb}$ by less than 1 F1 point on 4 others). 

As an added benefit of our MIPS-based approach, upon inspection of our returned results, we identified mislabeled examples in the training dataset. 
For instance, in the abt-buy dataset, we found a cluster of records in the specified right table that contain the same column values: rtable-id 799, 800, 801. 
However, ltable-id value 720 erroneously lists rtable-id 800 as not a match in the train set, when rtable-id 799 is a match in the test set.


\minihead{Results} We report our results in Table~\ref{table:retrieval} after training once over 10M of the 397M training examples, as training the full dataset for even one epoch requires over a week with our hardware. 
Notably, we obtain MRR@10 of 0.231 after just 250K training examples---which is just  0.07\% of the provided training dataset.
We report the official BM25 baseline solution, which we outperform by 1.49$\times$.
Our results are on par with K-NRM, a kernel based neural model, which achieves a dev set performance of 0.218~\cite{marcobert}, and slightly below the state-of-the-art from the time, IRNet, with 0.278 MRR@10~\citep{irnet}. 
For comparison, the first state-of-the-art BERT-based model uses BERT$_\text{large}$ to achieve MRR@10 of 0.365 after training on 12.8M examples~\cite{bertthing}, and current state-of-the-art achieves 0.439~\cite{rocketQA}. 
With further development and configuration of \sys \encoder aggregation method, \sys can implement ColBERT~\cite{colbert}, a previous state-of-the-art method that achieves 0.384 MRR@10 on the MS MARCO document ranking task, passage ranking's sister task that operates on larger input passages (i.e., "documents"). 


\minihead{Results} We report Retrieval@1, Retrieval@10, and MRR@10 of the modified SQuAD workload Table~\ref{table:retrieval}. In each case, we outperform BM25, where the gap between the two methods grows from  as \sys retrieves more records. 


\minihead{Results} We report Retrieval@1, Retrieval@10, and MRR@10 of the IMDb-wiki-join application Table~\ref{table:retrieval}. 
\sys significantly outperforms BM25 when retrieving the top \record. 
BM25 closes the gap when considering retrieval@10, but still lags far in MRR@10. 

In the IMDb-wiki-rec application, we report the mean squared error (MSE) between the rating estimates and the true rating when aggregating 1, 10, 20, and 30 nearest neighbors. The task is a fairly easy workload for which predicting the average training rating provides a MSE 1.19, and a gradient-boosted decision tree over the joined data returns 0.82 MSE.
We aim to meet or exceed the GBDT's performance. 
Both one- and two-hop approaches improve performance as the number of neighbors increase, until a plateau is reached. 
The two-hop approach attains MSE of 1.69, 0.92, 0.89, and 0.89 for 1, 10, 20, and 30 neighbors, respectively, while the one-hop approach performs better with 1.59, 0.89, 0.86, and 0.85. 
}

==> tables/baselines-k.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll|c|c|c|c|c|c|c|c|}
\cline{3-10}
\textbf{}                           & \textbf{}        & \multicolumn{8}{c|}{\textbf{k-to-90}}                                                                                                                                                                \\ \hline
\multicolumn{1}{|l|}{\textbf{Task}} & \textbf{Dataset} & \textbf{\textsc{ld}} & \textbf{\textsc{jk-ws}} & \textbf{\textsc{jk-2g}} & \textbf{\textsc{l-ws}} & \textbf{\textsc{J-2g}} & \textbf{\textsc{bert}} & \textbf{\textsc{bm25}} & \textbf{\textsc{emb}} \\ \hline
\multicolumn{1}{|l|}{FJ}            & IMDb-easy        &                      &                         & \textbf{}               &                        & \textbf{}              &                        &                        &                       \\ \hline
\multicolumn{1}{|l|}{FJ}            & IMDb-med         &                      &                         &                         &                        & \textbf{}              &                        &                        &                       \\ \hline
\multicolumn{1}{|l|}{QA}            & SQuAD            &                      &                         &                         &                        &                        &                        &                        & \textbf{}             \\ \hline
\multicolumn{1}{|l|}{S}             & MS MARCO         &                      &                         &                         &                        &                        &                        &                        & \textbf{}             \\ \hline
\multicolumn{1}{|l|}{R}             & IMDb-wiki-join   &                      &                         &                         & \textbf{}              &                        &                        &                        &                       \\ \hline
\multicolumn{1}{|l|}{EM-T}          & Abt-Buy          &                      &                         & \textbf{}               &                        &                        &                        &                        & \textbf{}             \\ \hline
\multicolumn{1}{|l|}{EM-T}          & Company          &                      &                         &                         &                        &                        &                        & \textbf{}              & \textbf{}             \\ \hline
\multicolumn{1}{|l|}{EM-S}          & Avg,  < 200 Test &                      &                         &                         &                        &                        &                        & \textbf{}              &                       \\ \hline
\multicolumn{1}{|l|}{EM-S}          & Avg, > 200 Test  &                      &                         &                         &                        & \textbf{}              &                        & \textbf{}              & \textbf{}             \\ \hline
\multicolumn{1}{|l|}{EM-D}          & Avg. < 200 Test  &                      &                         &                         &                        &                        &                        & \textbf{}              &                       \\ \hline
\multicolumn{1}{|l|}{EM-D}          & Avg. > 200 Test  &                      &                         &                         & \textbf{}              & \textbf{}              &                        & \textbf{}              & \textbf{}             \\ \hline
\end{tabular}%
}
\caption{Number of records retrieved to achieve a 90\% recall.}
\label{tab:kneeded}
\end{table}

==> tables/dm_micros.tex <==
\begin{table}[]
\small
\begin{tabular}{|c|lrrrr||r|}
\hline
\textbf{\textbf{Task}} & \textbf{\textbf{Dataset}} & \multicolumn{1}{l}{\textsc{all}} & \multicolumn{1}{l}{\textsc{-mlm,rl}} & \multicolumn{1}{l}{\textsc{-rl}} & \multicolumn{1}{l|}{\textsc{-mlm}} & \multicolumn{1}{|c|}{\textsc{te}} \\ \hline
EM-T                   & Abt-Buy                   & 87.45                            & 3.92                                 & 2.96                             & 1.08                               & 5.30                             \\ \hline
EM-T                   & Company                   & 86.38                            & 3.14                                 & 1.97                             & 1.02                               & 2.40                             \\ \hline
EM-S                   & BeerAdvo-RateBeer         & 89.99                            & 2.16                                 & 1.10                             & 1.52                               & 33.75                            \\ \hline
EM-S                   & iTunes-Amazon             & 75.77                            & 1.84                                 & 1.14                             & 1.43                               & inf                              \\ \hline
EM-S                   & Fodors-Zagat              & 86.42                            & 1.46                                 & 1.14                             & 1.33                               & 26.46                            \\ \hline
EM-S                   & DBLP-ACM                  & 98.51                            & 1.07                                 & 1.02                             & 1.01                               & 1.19                             \\ \hline
EM-S                   & amazon-google             & 69.83                            & 1.49                                 & 1.30                             & 1.01                               & 3.85                             \\ \hline
EM-S                   & DBLP-Scholar              & 81.50                            & 1.22                                 & 1.15                             & 0.94                               & 2.74                             \\ \hline
EM-S                   & Walmart-Amazon            & 73.11                            & 1.96                                 & 2.26                             & 1.02                               & 15.56                            \\ \hline
EM-D                   & DBLP-ACM                  & 98.00                            & 1.19                                 & 1.05                             & 1.00                               & 1.33                             \\ \hline
EM-D                   & DBLP-Scholar              & 81.16                            & 1.30                                 & 1.05                             & 0.94                               & 3.20                             \\ \hline
EM-D                   & iTunes-Amazon             & 67.63                            & 1.93                                 & 1.61                             & 1.73                               & 16.15                            \\ \hline
EM-D                   & Walmart-Amazon            & 69.27                            & 3.03                                 & 2.12                             & 1.04                               & 5.96                             \\ \hline
\end{tabular}
\caption{Microbenchmarks evaluating \sys's architecture, reflecting how many times better \sys is compared to: using a pretrained DistilBERT$_{\text{base}}$ model, without representation learning, without MLM pretraining, and when using one encoder for each dataset.}
\label{table:dm_micros}
\end{table}

==> tables/micros.tex <==
% \hhline{~~--------------}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|
>{\columncolor[HTML]{FFFFFF}}r rrr
>{\columncolor[HTML]{6FA8DC}}r |r|}
\hline
\multicolumn{8}{|c|}{\cellcolor[HTML]{EFEFEF}\textbf{Recall@1}}                                                                                                                                                                                                                                                                                                                                            \\ \hline
\cellcolor[HTML]{F3F3F3}\textbf{\textbf{Task}} & \cellcolor[HTML]{F3F3F3}\textbf{\textbf{Dataset}} & \cellcolor[HTML]{F3F3F3}\textbf{{\textsc{-mlm,rl}}} & \cellcolor[HTML]{F3F3F3}\textbf{{\textsc{-rl}}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-ft}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-mlm}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-ns}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{te}} \\ \hline
FJ                                             & IMDb                                              & -53.15\%                                            & \cellcolor[HTML]{A4C8E9}-19.78\%                & \cellcolor[HTML]{AACCEB}-22.25\%              & \cellcolor[HTML]{72AADD}-1.69\%                & -0.84\%                                       & \cellcolor[HTML]{BAD6EF}-28.02\%             \\ \hline
FJ                                             & IMDb-hard                                         & -90.19\%                                            & \cellcolor[HTML]{DCEAF7}-68.29\%                & \cellcolor[HTML]{D4E5F5}-63.31\%              & \cellcolor[HTML]{8EBBE4}-20.54\%               & -1.82\%                                       & \cellcolor[HTML]{AFCFEC}-41.02\%             \\ \hline
QA                                             & SQuAD                                             & \cellcolor[HTML]{FAFCFE}-78.5\%                     & \cellcolor[HTML]{FFFFFF}-81.88\%                   & \cellcolor[HTML]{E6F0F9}-67.09\%              & \cellcolor[HTML]{6FA8DC}3.2\%                  & \cellcolor[HTML]{8EBBE4}-14.72\%              & \cellcolor[HTML]{C6DDF2}-48.08\%             \\ \hline
S                                              & MS MARCO                                          & -99.91\%                                            & \cellcolor[HTML]{E2EEF8}-81.06\%                & \cellcolor[HTML]{DEEBF7}-78.26\%              & \cellcolor[HTML]{6FA8DC}-6.36\%                & \cellcolor[HTML]{94BFE5}-30.32\%              & \cellcolor[HTML]{ADCEEB}-46.34\%             \\ \hline
R                                              & IMDb-wiki                                         & -99.96\%                                            & \cellcolor[HTML]{FEFEFF}-98.79\%                & \cellcolor[HTML]{F8FBFE}-94.88\%              & \cellcolor[HTML]{78AEDF}-6.66\%                & -0.75\%                                       & \cellcolor[HTML]{FEFFFF}-99.\%               \\ \hline
EM-T                                           & Average All                                       & -90.43\%                                            & \cellcolor[HTML]{F0F6FC}-80.98\%                & \cellcolor[HTML]{EBF3FB}-78.25\%              & \cellcolor[HTML]{75ACDE}-7.75\%                & -4.59\%                                       & \cellcolor[HTML]{FBFDFE}-87.8\%              \\ \hline
EM-S                                           & Average All                                       & \cellcolor[HTML]{BFD9F0}-49.51\%                    & \cellcolor[HTML]{8FBBE4}-24.07\%                & \cellcolor[HTML]{92BEE5}-25.9\%               & \cellcolor[HTML]{6FA8DC}-7.47\%                & \cellcolor[HTML]{72AADD}-9.02\%               & \cellcolor[HTML]{FFFFFF}-83.47\%                \\ \hline
EM-D                                           & Average All                                       & \cellcolor[HTML]{D6E6F5}-54.01\%                    & \cellcolor[HTML]{A8CBEA}-34.46\%                & \cellcolor[HTML]{A5C9EA}-33.13\%              & \cellcolor[HTML]{6FA8DC}-10.18\%               & \cellcolor[HTML]{7AAFDF}-14.65\%              & \cellcolor[HTML]{FFFFFF}-71.74\%                \\ \hline \hline
\multicolumn{8}{|c|}{\cellcolor[HTML]{EFEFEF}\textbf{Recall@10}}                                                                                                                                                                                                                                                                                                                                           \\ \hline
\cellcolor[HTML]{F3F3F3}\textbf{Task}          & \cellcolor[HTML]{F3F3F3}\textbf{Dataset}          & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-mlm,rl}}   & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-rl}}   & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-ft}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-mlm}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{-ns}} & \cellcolor[HTML]{F3F3F3}\textbf{\textsc{te}} \\ \hline
FJ                                             & IMDb                                              & -30.02\%                                            & \cellcolor[HTML]{9EC4E8}-9.83\%                 & \cellcolor[HTML]{9EC4E8}-9.77\%               & \cellcolor[HTML]{70A9DD}-0.39\%                & -0.25\%                                       & \cellcolor[HTML]{84B5E2}-4.54\%              \\ \hline
FJ                                             & IMDb-hard                                         & -78.54\%                                            & \cellcolor[HTML]{D3E4F5}-54.26\%                & \cellcolor[HTML]{B9D5EE}-40.1\%               & \cellcolor[HTML]{78AEDF}-5.17\%                & -0.52\%                                       & \cellcolor[HTML]{80B3E1}-9.52\%              \\ \hline
QA                                             & SQuAD                                             & \cellcolor[HTML]{E9F2FA}-65.71\%                    & \cellcolor[HTML]{FFFFFF}-78.28\%                   & \cellcolor[HTML]{D6E6F5}-54.89\%              & \cellcolor[HTML]{6FA8DC}2.29\%                 & \cellcolor[HTML]{7CB0E0}-4.64\%               & \cellcolor[HTML]{A0C6E8}-24.6\%              \\ \hline
S                                              & MS MARCO                                          & -99.79\%                                            & \cellcolor[HTML]{DAE9F6}-75.02\%                & \cellcolor[HTML]{D5E6F5}-71.74\%              & \cellcolor[HTML]{6FA8DC}-4.85\%                & \cellcolor[HTML]{89B8E3}-21.8\%               & \cellcolor[HTML]{A1C6E9}-37.48\%             \\ \hline
R                                              & IMDb-wiki                                         & -99.74\%                                            & \cellcolor[HTML]{FAFCFE}-95.76\%                & \cellcolor[HTML]{E4EFF9}-80.58\%              & \cellcolor[HTML]{73ABDD}-2.54\%                & 0.03\%                                        & \cellcolor[HTML]{F7FAFD}-93.8\%              \\ \hline
EM-T                                           & Average All                                       & -74.24\%                                            & \cellcolor[HTML]{D6E7F6}-51.34\%                & \cellcolor[HTML]{D1E4F4}-48.41\%              & \cellcolor[HTML]{7FB2E0}-2.74\%                & 6.11\%                                        & \cellcolor[HTML]{E4EFF9}-58.91\%             \\ \hline
EM-S                                           & Average All                                       & \cellcolor[HTML]{C0D9F0}-42.73\%                    & \cellcolor[HTML]{89B8E3}-15.41\%                & \cellcolor[HTML]{8EBBE4}-17.89\%              & \cellcolor[HTML]{73ABDD}-4.77\%                & -2.9\%                                        & \cellcolor[HTML]{FFFFFF}-74.11\%                \\ \hline
EM-D                                           & Average All                                       & \cellcolor[HTML]{E6F0F9}-53.54\%                    & \cellcolor[HTML]{A1C6E8}-26.12\%                & \cellcolor[HTML]{A0C6E8}-26.04\%              & \cellcolor[HTML]{82B4E1}-13.93\%               & -6.7\%                                        & \cellcolor[HTML]{FFFFFF}-63.57\%                \\ \hline
\end{tabular}%
}
\caption{%Microbenchmarks evaluating \sys's architecture. 
Microbenchmarks reflecting the percent difference from the default architecture (Table~\ref{tab:baselines}) compared to: a pretrained DistilBERT$_{\text{base}}$ model without representation learning (\textsc{-mlm,rl}), MLM pretraining without RL (\textsc{-rl}), RL with no Transformer fine tuning (\textsc{-ft}), RL with no MLM pretraining (\textsc{-mlm}), no hard negative sampling (\textsc{-ns}), and one encoder per dataset (\textsc{te}). Better results within each row are darker.}
\label{table:micros}
\end{table}

==> tables/retrieval.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|l|cc|cc|cc|}
\hline
\textbf{Task}          & \textbf{Dataset} & \multicolumn{2}{c|}{Ret@1} & \multicolumn{2}{c|}{Ret@10} & \multicolumn{2}{c|}{MRR@10} \\ \cline{3-8} 
\multicolumn{1}{|l|}{} &                  & BM25         & \textsc{Emb}        & BM25         & \textsc{Emb}          & BM25         & \textsc{Emb}          \\ \hline
FJ                     & IMDb             &     86.35         &      95.06       &      91.27        &       99.02       &      0.879        &      0.965        \\ \hline
FJ                     & IMDb-hard        &     64.44         &      91.19       &      74.12        &       98.43       &      0.676        &      0.938        \\ \hline
QA                     & SQuAD            &     53.34         &      59.34      &      71.53        &       84.84       &      0.593        &       0.679      \\ \hline
S                      & MS MARCO         &     -             &     16.62        &     -             &      44.76        &     0.167        &      0.249        \\ \hline
R                      & IMDb-wiki-join   &     63.25         &     96.44        &      96.25        &      98.92        &      0.771        &      0.973        \\ \hline
\end{tabular}}
\caption{End-to-end performance of \sys compared to using BM25 after the preprocessing step.}
\label{table:retrieval}
\end{table}
